Firefly Neural Architecture Descent: a General Approach for Growing Neural Networks

We propose firefly neural architecture descent, a general framework for progressively and dynamically growing neural networks to jointly optimize the networks' parameters and architectures. Our method works in a steepest descent fashion, which iteratively finds the best network within a functional neighborhood of the original network that includes a diverse set of candidate network structures. By using Taylor approximation, the optimal network structure in the neighborhood can be found with a greedy selection procedure. We show that firefly descent can flexibly grow networks both wider and deeper, and can be applied to learn accurate but resource-efficient neural architectures that avoid catastrophic forgetting in continual learning. Empirically, firefly descent achieves promising results on both neural architecture search and continual learning. In particular, on a challenging continual image classification task, it learns networks that are smaller in size but have higher average accuracy than those learned by the state-of-the-art methods.

==> Firefly splitting/backup/backup.tex <==
% % the general goal of the Firefly Steepest Descent is to find a new $\theta$ within certain neighborhood of $\theta_0$, i.e. $\theta \in N(\theta_0, \epsilon)$, such that the loss decreases the most under a . Here, $\epsilon$ is a parameter that controls the size of $N(\theta_0, \epsilon)$
% % It is a general framework. For any architecture $\theta$, let $N(\theta; \epsilon)$ be a general neighorhood of $\theta$,
% % where $\epsilon$ is parameter that control the size of $N(\theta; \epsilon)$ (e.g., radius), such that when $\epsilon=0$, we have $N(\theta; \epsilon) = \theta$.  

% We consider a general procedure: 
% $$
% \theta_{t+1} \gets 
% \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~
%  \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) \leq \tau_t \right\},
% $$
% where $C(\theta)$ represents a measure of size or computational cost of the network represented by $\theta$. 

% \textcolor{red}{[Explain definition of $N(\theta,\epsilon)$ and $C(\theta)$]} 
% By choosing different $N(\theta)$, we derive a general class of growing mechanisms: 

% 1. Splitting 


% 2. Introducing New Neurons

% 3. Growing layers

% \textcolor{red}{[How to solve optimization?]} 
% A remaining question is how to solve the optimization in each step. The key idea is that when $\epsilon$ is small, the linear objective is closely linear and hence can be solved approximately. 

% Let $\theta = \theta_t \oplus \delta$ (define it in proper way).  What is the value space of $\delta$? 
% Then the optimization reduces to 
% $$
% \delta_{t+1}  
% = \arg\min_{\delta} L(\theta_{t} \oplus \delta) ~~~~s.t.~~~~
% %\delta \in N(0,\epsilon),
% \norm{\delta}_2\leq \epsilon, 
% ~~~~ ||{\delta}||_0 \leq \tau_t. 
% $$

% Our approach: 

% Step 1: Solve $\delta$ without the L0 constraint by running a small number of gradient descent. We this yields that constrainted optimization:
% $$
% \min_{\delta} L(\theta_{t} \oplus \delta) +  \lambda \norm{\delta}_2^2. $$

% Step 2: Select the one with the largest contribution (in terms of gradient norm). This can be motivated by Taylor expansion. We use \emph{integrated gradient}. 

% In practice, we find a small number of $N$ is sufficient (e.g., $N=3$), and outperforms $N=1$. 

% \textcolor{blue}{[Have a nice diagram for our method]}

% \section{Application to Continual Learning} 
% \red{[introduce the set up of continuous learning]}... 


% \section{Related works}
% \textcolor{red}{[Review related works on growing networks]} 

% 1. net morphism/net2net

% 2. growing networks in continous learning. 

% 3. autogrow (growing layers)
 


% \section{FireFly Splitting}
% In this section, we present the Firefly expansion, a first order method to gradually enlarge a network. In particular, Firefly aims to study two questions:
% % FireFly splitting is mainly studying two questions: 
% \begin{enumerate}
%     \item can we split without dealing with the splitting matrix and therefore get rid of the local convergence assumption?
%     \item can we allow not only splitting existing neurons, also allow emerging new neurons?
% \end{enumerate}
% % For 1), we can directly optimize the $\delta$s in the original optimization problem using SGD. So here I replace the 2-norm constraint by an infinite norm constraint to relatively enlarge the feasible sets (compared to 2-norm) and scale the constraints according to the original $\theta$ (we can use $\epsilon$ as well, there is no justification now for scaling):
% To begin with, we formulate the objective of Firefly as the following:
% \begin{flalign*}
% \text{minimize: } &  \mathcal{L}(\delta, w) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(\sum_{i=1}^m w_i \sigma(\theta + \delta_i, x) + \sum_{j=1}^k b_j \sigma(\delta_j, x) \bigg)\bigg]\\
% \text{subject to: }  &\sum_{i=1}^m w_i = 1\\
% &\forall i,\quad ||\delta_i||_2 \leq \epsilon\\
% &\forall j,\quad b_j \leq \epsilon\\
% \end{flalign*}
% % Due to above, we know if two copies of neurons have shared direction of improvement, it can be captured by the gradient anyway. Therefore, I force $\delta_1 = -\delta_2$, so I only need to optimize one of them. The problem then becomes:
% % \begin{flalign*}
% % \text{minimize: }&  \mathcal{L}(\delta) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(\frac{1}{2} ( \sigma(\theta + \delta, x) + \sigma(\theta - \delta, x) \bigg)\bigg]\\
% % &||\delta||_\infty \leq \epsilon ||\theta||_\infty\\
% % \end{flalign*}
% To estimate the loss decrease contribution of each neurons, here we use the line integral method. Assume we consider $n$ neurons, so by above, we will have $\delta = (\delta_1, \dots, \delta_k)$. Note that $\mathcal{L}(0) = \mathcal{L}(\theta)$, we have
% \begin{equation}
%     \mathcal{L}(\delta) - \mathcal{L}(0) = \int_{t=0}^1 \nabla \mathcal{L}(t\delta) \cdot \delta d_t \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta)\bigg) \cdot \delta.
% \end{equation}
% As a result, for each individual neuron that has perturbation $\delta_j$, its contribution to loss decrease can be estimated by:
% \begin{equation}
%     \text{contribution}(j) = \mathcal{L}(\delta_j) - \mathcal{L}(0) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_j)\bigg) \cdot \delta_j.
% \end{equation}


% %We can also define the contribution of each neuron by 
% %$$\text{contribution}(j) = \frac{\mathcal{L}(\delta) - \mathcal{L}(0)}{f_{\theta}(\delta) - f_{\theta}(0)}$$

% %Here $f_{\theta}$ represent the output of the current layer with weight $\theta$, so this contribution constraint the newly added neurons to have a larger loss decrease as well as a minor output change in its layers. 

% Then we can select the top-$m$ of those.
\\\\




% For 2), it is hard to determine the number of neurons to add. Imagine that we are allowed to add infinite number of neurons, then it is essentially possible to fit any function. Therefore, we restrict the number of newly added neurons to be less than a fix number $k$ (so we will have $m$ splitted neurons and fewer than $k$ newly added neurons after a single split operation). The resulting new optimization problem is therefore:

% I do not have much thought on this. The simplest thing to do is to treat all those $\delta_j$, $b_j$ the same as $\delta_i$ and use SGD to train them.
% \paragraph{side note:} some questions:
% \begin{itemize}
%     \item Empirically speaking, the perturbation direction matters less than which neuron to split (if you split certain neuron, you can get stuck). So ideally, we only need $\mathcal{O}(n)$ spaces to store each neurons importance. Since we are doing forward backward during training, can we estimate them on the fly and then split according to the stored info?
%     \item Following above, with firefly, I am thinking maybe it is also possible to train the perturbations on the fly (during training). Say, we add an l1 norm constraint on the perturbation and just let it train. And split according to the norm of the eventual perturbations. The benefit of doing this is that it is not ``local'' anymore, the loss indeed decrease by certain amount after we do this. One may ask then why don't we just double the hidden layer and train the neural network and then prune. I believe it's certainly doable. You start from a small hidden size, then you double the layer width, train, and then prune, and then double again. However, whenever you double the layer, if you nonetheless need to do the net-2-wider-net operation. Otherwise randomly initialized neurons might not do well. In contrast, perturbations are naturally orthogonal to the original parameter and also relies on original parameter. So this method both has a good start point and better descent direction.
% \end{itemize}

% \subsection{Expanding Multiple Layers Simultaneously}
% Assume we are at layer $l$, and have layer below $l-1$ with $n_{l-1}$ neurons and above $l+1$ with $n_{l+1}$ neurons originally. Following the above, if we add $K$ new neurons to each layer and also consider splitting existing $n$ neurons within this layer. Denote $x$ as the original input without expanding the previous layer, and $x'$ the $K$ dimensional new input induced from adding $K$ new neurons to the layer $l-1$. Denote $\Theta \in \mathbb{R}^{n_{l}\times n_{l-1}}$ the original weight matrix at layer $l$. Similarly, the perturbation on $\Theta$ is $\Delta \in \mathbb{R}^{n_{l}\times n_{l-1}}$ and the weights on $l$ layer for the newly added $K$ neurons is $\Delta_{o} \in \mathbb{R}^{K \times n_{l-1}}$. The weight that projects the previous $K$ neurons to the current layer is $\Delta_i \in \mathbb{R}^{(n_l+K) \times K}$. We further split $\Delta_i$ into $\Delta_{i1} \in \mathbb{R}^{n_l \times K}$ and $\Delta_{i2} \in \mathbb{R}^{K \times K}$. The problem can be formulated as:
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{diary/firefly.eps}
%     \caption{Illustration figure of the learnable perturbations.}
%     \label{fig:my_label}
% \end{figure}
% \begin{flalign*}
% \text{minimize: } &  \mathcal{L}(\Delta, \Delta_i, \Delta_o) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(
% \frac{1}{2}\bigg(\sigma((\Theta + \Delta)x + \Delta_{i1}x') + \sigma((\Theta - \Delta)x + \Delta_{i1}x')\bigg) + \epsilon \sigma(\Delta_ox + \Delta_{i2}x') 
% \bigg)\bigg]\\
% \text{subject to: }  & ||\Delta||^2_2 + ||\Delta_i||^2_2 + ||\Delta_o||^2_2 \leq c
% \end{flalign*}

% \begin{equation}
%     \text{contribution}(i_1) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_{i_1})\bigg) \cdot \delta_{i_1}, \quad\text{where $\delta_{i_1}$ is the $i_1$-th row of $\Delta$} 
% \end{equation}

% \begin{equation}
%     \text{contribution}(i_2) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_{i_2})\bigg) \cdot \delta_{i_2}, \quad\text{where $\delta_{i_2}$ is the $i_2$-th row of $\Delta_o$} 
% \end{equation}

% \begin{equation}
%     \text{contribution}(i_1) = \nabla \mathcal{L}(\theta_{i_1} + \delta_{i_1})||_{\delta_{i_1}= 0} \cdot \delta_{i_1}
% \end{equation}
% In fact, during practice, I still find the line integral methods gives better results. This probably because it considers the change beyond the local curvature as well. In practice, $N=3$ seems enough. Also, in the extreme case, the gradient can be taken at any single point along the line the perturbation moves. If we take at the gradient at the very beginning, i.e. $\lim_{t \rightarrow 0}\nabla \mathcal{L}(\theta + t \delta)$, then this should be equivalent as the ``minimum" eigenvector in the exact case. On the other hand, if we take the gradient at $t=1$, then it estimates each neuron's contribution using it's current gradient and how much it deviates from 0. In general, if the local curvature is more convex in the larger space (as if the network has splitted), then the estimation at $t=1$ should be more conservative. Similarly, if the local curvature is more concave, which means the further we move along the perturbation, the loss decreases more on average, then the estimation is more optimistic.
% \section{Firefly (with new neurons) splitting}
% \begin{algorithm*}
%     \caption{Firefly (with new neurons) neural architecture expansion algorithm} \label{alg:main}
%     \begin{algorithmic}
%     \State For each layer, initialize $\Delta \in \mathbb{R}^{n_l \times n_{l-1}}$, $\Delta_o \in \mathbb{R}^{K \times n_{l-1}}$ and $\Delta_i = [\Delta_{i1}; \Delta_{i2}] \in \mathbb{R}^{(n_l+K) \times K}$.
    
%     \While{not converging}\Comment{Optimize the perturbations}
%         \State Calculate $L = \mathcal{L}(\Delta, \Delta_i, \Delta_o) + \lambda(||\epsilon_1 \Delta||^2_F + \epsilon_2 ||\Delta_o||^2_F)$.
%         \State Update $\Delta, \Delta_i, \Delta_o$ according to their gradient of $L$.
%         \State Clip $\Delta_i$ such that $||\Delta_i||_\infty \leq \epsilon_2$
%     \EndWhile
%     \State For each layer, initialize $w = c = \bm{0} \in \mathbb{R}^{n_l\times 1}, w_o = c_o = \bm{0} \in \mathbb{R}^{K\times 1}$.
%     \For{$z = 1 : N$}\Comment{Determine whom to split or expand}
%         \State $t = (2z - 1) / (2N)$
%         \State Let $\tilde{L} = \mathcal{L}((t\Delta + c \odot \Delta), (t\Delta_o + c_o \odot \Delta_o), \Delta_i)$
%         \State $w = w + \pdv{\tilde{L}}{c} / N$
%         \State $w_o = w_o + \pdv{\tilde{L}}{c_o} / N$
%     \EndFor
%     \State Split and expand neurons with the top-$m$ largest weights in $w \oplus w_o$
%     \end{algorithmic}
% \end{algorithm*}
% Recall that
% $$
% \mathcal{L}(\Delta, \Delta_i, \Delta_o) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(
% \frac{1}{2}\bigg(\sigma((\Theta + \epsilon_1 \Delta)x + \Delta_{i1}x') + \sigma((\Theta - \epsilon_1 \Delta)x + \Delta_{i1}x')\bigg) + \epsilon_2 \sigma(\Delta_ox + \Delta_{i2}x') 
% \bigg)\bigg]
% $$
% In practice:
% $$\lambda = 0.01, \quad \epsilon_1 = \sqrt{\epsilon_2},\quad N=3$$

% \section{preliminary results}
% \subsection{Two-Layer RBF Network}
% One of the issues that exact and Rayleigh Quotient methods have is that they are more prone to be stuck at local minimas. This is because either method determines its splitting direction (the eigenvector direction corresponding to the minimum eigenvector) based on the local curvature at the original minimum point. By contrast, Firefly methods, by gradually optimizing the perturbation direction, can see further beyond the original minimum point. We confirm our hypothesis on a simple two-layer radial-basis function neural network, which is of the form:
% \begin{equation}
%     f^*(x) = \sum_{i=1}^{20} w_i^* \sigma((\theta_i^*)^T [x, 1]), \quad \forall \theta_i^*, w_i^* \sim \mathcal{N}(0, \bm{I})
% \end{equation}
% \begin{figure}
% \begin{subfigure}[h]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{diary/rbf_loss.png}
%   \caption{Train Loss v.s. Number of Neurons}
% \end{subfigure}%
% \begin{subfigure}[h]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{diary/13.png}
%     \caption{Example of Exact method Got Stuck}
% \end{subfigure}
% \caption{(a) shows the RBF neural network training loss of different growing methods at different number of neurons, the firefly with new neuron method avoids getting stuck locally by considering growing new neurons as well as splitting. (b) gives an example of how pure splitting methods can get stuck at a local minima.}
% \end{figure}


















%with 
%provides a powerful and  then  estimates each neuron's individual  contribution to the expansion via the integrated gradient method, greedily selects out those neurons that contribute the most and expand from there on. Our method is simple to use and can be flexibly extended to include various growing operations. We derive our method for both growing wider, deeper and continuous learning. 
%
%Since FG only uses gradient estimation, it is much simpler to use and allow us to extend the framework to allow not only splitting existing neurons, but also introducing new neurons or even new layers. 
%

%Empirically, our method demonstrates better performance against existing splitting and growing methods on neural architecture search problems. Empirically, our method is demonstrated to be a useful approach for learning accurate and small neural architectures. \qred{mention some good results here} By combining with DARTS, we achieve xxx and xxx. For continuous learning tasks, we achieve xxx. and significantly outperform existing state-of-the-art approaches. 
%
%To further illustrates the potential of the FG method, we apply it to a continual learning task where it is natural to expand network capacity on the fly. 
%
%As expected, the proposed method is able to keep learning multiple tasks continually with much less parameters but higher accuracy compared to the state-of-the-art.\qred{remove? does not read exciting}To summarize, our key contribution is two-folded: \begin{enumerate}
%    \item Introducing a general and flexible  framework for growing neural network, which allows us to progressively increasingly wider and deeper networks. 
    %; the framework includes locally splitting existing neurons, growing new neurons, and introducing new layers.
 %   \item Applying our method to both neural architecture search and continual learning problems and achieve the state-of-the-art results.
%\end{enumerate}



% \iffalse 
% Learning compact but effective neural architecture is important for real-world applications that suffer from computational constraints, i.e. applications on mobile devices. 
% %
% Network pruning tackles this problem by removing less important parameters from a large pretrained network so that the remaining subnetwork can roughly preserve the original  performance. 
% %
% Unlike pruning, growing methods aim to gradually enlarge the  network's capacity only when necessary and therefore can more flexibly adapt to the task of interest in an online fashion. 
% %
% While simple heuristics like uniformly expanding the width of a feed-forward neural network can work well in certain scenarios, they are still far from being efficient and it is often hard for these methods to outperform pruning methods. 

% %
% Recently, \citet{splitting2019} first frame the network growing problem from a functional steepest descent perspective and present a practical algorithm that greedily determines which neurons are to split and in what direction. 
% %
% By doing so, their method does not require a well pretrained large network, can flexibly adapt its learning capacity, and  demonstrates comparable or improved performance over pruning methods. 
% %
% Despite good performance, the method is limited to only splitting existing neurons and therefore can oftentimes get stuck at local minimums. 
% %
% In addition, the method relies on an  accurate estimation of a local second order splitting matrix, which makes it both hard to implement and computational inefficient.


% To address these issues, we introduce a universal framework of  greedy first-order methods, the Firefly Growing (FG). 
% %
% FG uses a small amount of data to train a local perturbation, i.e. the possible expansions, within the neighborhood  functional space of the given network. 
% %
% It then efficiently estimates each neuron's individual  contribution to the expansion via the integrated gradient method, greedily selects out those neurons that contribute the most and expand from there on. 
% %
% Since FG only uses gradient estimation, it is much simpler to use and allow us to extend the framework to allow not only splitting existing neurons, but also introducing new neurons or even new layers. 
% %
% With such flexibility, FG empirically demonstrates better performance against existing splitting and growing methods on neural architecture search problems. 
% %
% To further illustrates the potential of the FG method, we apply it to a continual learning task where it is natural to expand network capacity on the fly. 
% %
% As expected, the proposed method is able to keep learning multiple tasks continually with much less parameters but higher accuracy compared to the state-of-the-art.

% To summarize, the key contributions of this work are:
% \begin{enumerate}
%     \item Introducing a universal first-order framework, the Firefly Growing, to greedily expand a neural network; the framework includes locally splitting existing neurons, growing new neurons, and introducing new layers.
%     \item Applying the Firefly Growing method to both neural architecture search and continual learning problems and achieve the state-of-the-art results.
% \end{enumerate}

 

% \fi






 %The neighorhood in \eqref{equ:masterupdate} determines the candidate size of network growing and hence places an important role. It need to be designed 
%case by case but some general rules applies. In this section, we mainly consider the general neighborhoods that allows to grow wider.  
 %Note that in this framework, the choice of 
 %Note that 
 %the neighborhood 
  %neighorhood in \eqref{equ:masterupdate} 
%  plays a crucial role of determining 
 % the possible ways in which the network can grow.
% $\neib(f_t, ~\epsilon)$ %, which we discuss in sequel,  plays a critical role. 
 %It should include functions that are $\epsilon$-close to $f_t$ but  
 %with a rich set network structures that makes growing possible (e.g., growing wider or deeper), 
 %, and also need to be constructed to make the optimization in \eqref{equ:masterupdate} (approximately) solvable in practice. 
  %, that are functionally close $f_t$. 
 %may have 
%such that the output does changes smoothly. 
%We can view $\epsilon$ as a step size parameter. 
%where we search the best neural network in a neighborhood $\neib(f_t, ~\epsilon)$ around $f_t$, subject to that its size increases at most by $\eta_t$ over $f_t$.  Here the neighborhood  $\neib(f_t, ~\epsilon)$ is defined such that 
%is no longer than 
%where $\{\eta_{t}\}$ controls the size that we want to increase over $\vv \theta_t$ and $\neib(\vv\theta_t, ~\epsilon)$ is a neighborhood of $\vv \theta_t$ in $\Omega$ with a size parameter $\epsilon$ such that $f_{\vv\theta}(x)= f_{\vv\theta_t}(x) + O(\epsilon)$, such that the output does changes smoothly. We can view $\epsilon$ as a step size parameter. 
%The idea here is similar to typical parametric gradient descent, which can be viewed as taking $\neib(\vv\theta_t, ~\epsilon)$ be the a typical L2 ball in Euclidean space, corresponding to models of the same size. To achieve architecture descent, however, we need to  extend the definition of  $\neib(\vv\theta_t, ~\epsilon)$ to include networks with larger sizes.  And also address how to solve the optimization problem.
%
% In the sequel, we address two important problems: 1) how to define the neighborhood $\neib(\vv\theta_t, ~\epsilon)$ and 2) how to solve the optimization efficiently in practice.  \qred{fix}

%and 2) how to solve the optimization efficiently in practice.  \qred{fix}

%Motivated by \citet{splitting2019},  
%In this work,we approach the problem with a general progressive local descent method, in which we incrementally update the parameter and/or structure of $f$ in $\Omega$ to greedily descent the loss in a way similar to typical gradient descent. 
%growing neural networks in a \emph{local descent} fashion. 
%In progressive growing, See Algorithm XXXX for the general framework.  Starting from a relatively small network, we alternate between typical gradient-based \emph{parametric descent phase}   with fixed model structures, and novel \emph{architecture descent phase}  that grow the network structure to decrease the loss when it is impossible with pure parameter descent, lifting the parameter optimization into a higher dimensional space to escape local optima that can not be escaped in the lower dimensional space (of the smaller models). 



%\paragraph{Definition of $\neib(\vv\theta_t, ~\epsilon)$} 


==> Firefly splitting/backup/method.tex <==
\section{Firefly Steepest Descent}
In this section, we formalize the Firefly Steepest Descent method by first providing a general framework and then discussing three specific instantiations for different growing strategies.\\\\
%

Let $\Omega$ be the space of all possible models and architectures. 
Consider, for example,  the case of one-layer neural networks, 
we have $f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$, where $\vv \theta = [\theta_i]_{i=1}^n$. Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$. This is an infinite dimensional space. In general, $\Omega$ can be much more complex than this for the case of deep neural networks. 

We consider an abstract algorithm which performs steepest descent on $\Omega$. The idea is to equip each point $\theta$ in $\Omega$ a neighorhood $N(\theta, \epsilon)$, which $\epsilon$ is the size ...


Consider at the growing iteration $t$, the current neural network is parameterized by $\theta_t$ and denote $C(\theta_t)$ as the computational cost of the network, i.e. the total flops. The general objective of the Firefly Steepest Descent is therefore to find a new $\theta$ within a neighborhood of $\theta_t$ which decreases the loss the most under the constraint that $C(\theta)$ remains low. Formally, we consider the following iterative process:
%
\begin{equation}
    \label{eq:6}
    \theta_{t+1} \gets \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~ \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) - C(\theta_t) \leq \tau_t \right\}.
\end{equation}
%
Here $\tau_t$ is a predefined computational budget for the growth and $\epsilon$ is the parameter controlling the size of the neighborhood $N(\theta_t, \epsilon)$, i.e. $\epsilon$ can be the radius of the ball centered at $\theta_t$ in the $L_p$ space \red{this should be a neighorhood in the architecture space, not $L_p$ space}. Note that here we want to abuse the notations and allow $\theta_{t+1}$ to have higher dimension than $\theta_t$. In this case, we treat those dimensions that $\theta_t$ does not have as zeros.\\\\
%
During practice, since the computational cost is mainly associated with the number of channels for each layer, we might just pick $\tau_t$ such that the number of increased channels is limited by some constant $M$. For optimization convenience, we consider a formulation equivalent to Equation \ref{eq:6} by optimizing over the perturbations around $\theta_t$. We also simply pick the $\ell_2$ norm constraint, though extensions to other norms are straightforward. Namely, let $\theta = \theta_t \oplus \delta_t$ (again, the dimensions are matched in the same way as when we compare $\theta_t$ and $\theta_{t+1}$; \red{still $\oplus$ is not defined mathematically}), then above update rule becomes:
%
\begin{equation}
    \label{eq:7}
    \delta_t \gets \arg\min_{||\delta_t||_2 \leq \epsilon} \left \{ L(\theta_t \oplus \delta_t) ~~~~s.t.~~~~ ||\theta_t \oplus \delta_t||_0 - ||\theta_t||_0\leq M \right\} \quad \text{and} \quad \theta_{t+1} &\gets \theta_t \oplus \delta_t ~.    
\end{equation}
To solve the above optimization, we consider the following two-step algorithm:\\\\
\textbf{Step 1}: transform the hard norm constraint into a norm penalty in the objective and solve $\delta_t$ without the $\ell_0$ constraint by running a small number of gradient descent steps:
\begin{equation}
    \hat{\delta}_t = \arg\min_{\delta} L(\theta_t \oplus \delta) + \lambda ||\delta||^2_2
\end{equation}
\textbf{Step 2}: project $\hat{\delta}_t$ back to satisfy the $\ell_0$ constraint, i.e. selecting the top-$M$ neurons that contribute the most to the loss decrease. Formally, let $\delta_t = z \odot \hat{\delta}_t$, where $z\in \{0, 1\}^n$ and $n$ is the dimension of $\hat{\delta}_t$. The objective can be formulated as:
\begin{equation}
    \min_z L(\theta_t \oplus (z \odot \hat{\delta_t})) ~~~~s.t.~~~~ ||z||_0 \leq M
\end{equation}
The possible choices of $z$ explode combinatorially when the dimension of $\hat{\delta}$ is large. Therefore, in practice, we estimate each neuron's contribution with the integrated gradient method. Namely,
\begin{equation}
    \Delta L = L(\theta_t \oplus \hat{\delta_t}) - L(\theta_t) = \int_{\alpha=0}^1 \nabla L(\theta_t \oplus \alpha \hat{\delta}_t) \cdot \hat{\delta_t} ~d\alpha.
\end{equation}
Expanding the gradient for individual parameter $\hat{\delta}_t^{(i)}$, we can formally define the contribution of each neuron and use monte-carlo method to approximate the integral:
\begin{equation}
\text{contribution}(\hat{\delta}_t^{(i)}) = \int_{\alpha=0}^1 \pdv{L(\theta_t \oplus \alpha \hat{\delta}_t)}{\alpha \hat{\delta}_t^{(i)}} \pdv{\alpha \hat{\delta}_t^{(i)}}{\alpha} d\alpha \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\delta}_t^{(i)})\bigg) \cdot \hat{\delta}_t^{(i)}.
\end{equation}
In practice, we find that with as small the $N$ as 3, the sampling can approximate the integral well. After the $\delta_t$ is found, FG simply expands the network according to $\delta_t$ and then resume the learning process. The whole pipeline of FG is summarized in Algorithm \ref{alg:firefly}.\\\\
Next, we will discuss three different network growing strategies: 1) splitting existing neurons, 2) growing new neurons, and 3) introducing extra layers. For each of these strategies, we present their corresponding objective formulation under the above general framework.
\paragraph{Splitting Existing Neurons:}
\paragraph{Growing New Neurons:}
\paragraph{Introducing Extra Layers:}

\begin{algorithm*}[t] % enter the algorithm environment
\caption{Firefly for Progressive Training of Neural Networks} 
\begin{algorithmic} % enter the algorithmic environment
%\begin{emumerate} 
\STATE \textbf{Input} : Search Space $S$. Initial small network $A_0$
\STATE Start from $A_0$.
%with random initialization, set the maximum neuron grow number $m^{*}_{total}$ or energy growth constraint $e^*_{total}$ each iteration and a threshold $|\lambda^*| > 0$ to stop. Repeat the following 4 steps below until the stop criterion is met:
\STATE \textbf{Repeat} Until the stop criterion is met
\STATE At step $t$
\STATE \textbf{1.} Train $A_t$ for several epochs to decrease the loss. 
    \vspace{.3\baselineskip} 
    \STATE \textbf{2.} Expand $A_t$ to a larger neighbor network $A_t'$ by adding a set of neurons $n_t$ in the search space $D$
    \vspace{.3\baselineskip} 
    \STATE \textbf{3.} Train $A_t'$ for several iterations, select the best subset of neurons in $n_t$ using our method. Keep these neurons in the network and drop the rest of the neurons in $n_t$ to get the new network $A_{t+1}$
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}


==> Firefly splitting/backup/method2.tex <==
\section{Firefly Steepest Descent}
In this section, we first provide a general functional steepest descent perspective for growing neural architectures and briefly review the existing splitting steepest descent as a special case.
%
Then we introduce the more general Firefly Growing framework that uses first-order method to approximate the steepest descent.
%
In addition, we will discuss three particular growing strategies under the general framework.


\section{Main Idea}
To illustrate the idea, 
let us consider a simple one layer neural network: 
$f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$,
where $\vv \theta = [\theta_i]_{i=1}^n$.
Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$.
This is an infinite dimensional space. The problem of learning then reduces to 
\begin{align*} 
\min_{\vv\theta\in\vv \Omega} L(\vv\theta)\overset{def}{=} \E_{x\sim \D}[\Phi(f(x; \vv\theta))] ~~~~s.t.~~~~  C(\theta) \leq \eta, 
\end{align*}
where $C(\theta)$ is some complexity cost such as the size of the network and $\eta$ is a budget constraint, and $\Phi(\cdot)$ denotes the loss function, e.g., $\Phi(f(x)) = (f(x)-f^*(x))^2$ where $f^*$ is the underlying true function. 

%In \citet{splitting2019}, a steepest descent approach is proposed. It alternates between: 

In progressive growing,
we start from a small network and gradually improve its performance by growing in a monotonic fashion. Our procedure alternates between 
parametric descent within a fixed subregion $\Omega_{m}$  and architecture descent across the regions: 

1. \emph{Parametric Descent}  
We perform typical parametric updates with a fixed model structures, 
corresponding to travel inside a subregion $\Omega_{m}.$ 
The parametric descent can continue until no further improvement can be made inside $\Omega_m$, i.e., local optima is reached.  %within the fixed region $\P$
%(corresponding )
%Fixing the structure and optimizing the parameters, this corresponds to optimizing $\vv\theta$ within a fixed subspace $\Omega_{\vv m}.$ 

2. \emph{Architecture Descent} We grow the neural network architecture by jointly updating the parameter and model architecture, 
which corresponds to jumping from one subregion to a higher region with higher complexity. 
%If $\vv\theta$ is not 
%network parameter
%In general, $\Omega$ can be much more complex for deep neural networks.
%Although $\Omega$ is an infinite dimensional space which includes neural networks with varying sizes, it still possible to perform steepest descent in the space of $\vv\Omega$. 


%Starting from an initial network $\vv\theta_0$, at each iteration $t$, we perform a decent on the loss via
Let $\vv \theta_t$ be the neural network at the $t$-th growing phase, we propose to grow the network via the following formulation: 
\begin{align} \label{equ:masterupdate}
\vv \theta_{t+1} = \argmin_{\vv\theta\in \vv \Omega_\infty} L(f(\cdot, \vv\theta)) ~~~~s.t.~~~  \vv\theta \in \neib(\vv\theta_t, ~\epsilon),~~~~~~ 
C(\vv\theta) \leq C(\vv\theta_t)+\eta_{t+1}, 
\end{align}
where $\{\eta_{t}\}$ controls the size that we want to increase over $\vv \theta_t$ and $\neib(\vv\theta_t, ~\epsilon)$ is a neighborhood of $\vv \theta_t$ in $\Omega$ with a size parameter $\epsilon$ such that $f_{\vv\theta}(x)= f_{\vv\theta_t}(x) + O(\epsilon)$, such that the output does changes smoothly. We can view $\epsilon$ as a step size parameter. 

The idea here is similar to typical parametric gradient descent, which can be viewed as taking $\neib(\vv\theta_t, ~\epsilon)$ be the a typical L2 ball in Euclidean space, corresponding to models of the same size. 
To achieve architecture descent, however, we need to  extend the definition of  $\neib(\vv\theta_t, ~\epsilon)$ to include networks with larger sizes.  And also address how to solve the optimization problem.
In the sequel, we address two important problems: 1) how to define the neighorhood $\neib(\vv\theta_t, ~\epsilon)$ and 2) how to solve the optimization efficiently in practice. 

\paragraph{Definition of $\neib(\vv\theta_t, ~\epsilon)$} 
The neighorhood in \eqref{equ:masterupdate} determines 
the candidate size of network growing and hence places an important role. It need to be designed case by case but some general rules applies. In this section, 
we mainly consider the general neighborhoods that allows to grow wider. 

It is useful to illustrate the idea with one-layer networks. 
Consider $f_\theta(x) = \sum_{i=1}^{m} w_i \sigma(x, \theta_i)$. We augmented it by two types of operators: 

\emph{Splitting Neurons (local).} 
We may consider the local updates turns a neuron into multiple similar neurons (intutively viewed as splitting). 
Splitting a neuron $w_i \sigma(x, \theta_i)$ amounts to replace it with a set of neurons $w_{i\ell} \sigma(x, \theta_{i\ell})$, 
where $|\theta_{i\ell} - \theta| \leq \epsilon$ and $\sum_{i\ell} w_{i} =1$. This ensures that the network output after splitting remains similar to the original network when $\epsilon$ is small.
 As argued in \citet{splitting2019}, it is sufficient to consider splitting to two copies $m=2$ and $w_{i1} =w_{i2} = 1/2$ and $\delta_{i1} = -\delta_{i2} = \delta_i$. In this case, it splits into two copies with equal weights, following opposite directions. 

\emph{Growing New Neurons.} 
We introduce a new neuron  $\epsilon w_i' \sigma(\theta', x)$ with a small output weight. that is, we replace $f_\theta$ with $f_\theta(x) + \epsilon w_i'\sigma(\theta_i', x)$ which introduces small change if $\epsilon$ is small. 
Because $\theta'$ can be choosen arbitrarily, this update is non-local and hence may help jump out of local optima. 
%with a small output weight. This amounts to replace $f_\theta$ with $f_\theta(x) + w_i' \sigma$
%Motivated by \citep{splitting2019}, we re
%$$f_{\vv\vartheta'}(x) =\sum_{i=1}^{m'} w_i \sigma(x,\theta'_i).$$Such that for each $j$, we need 

Overall, the augmented neural networks in $\neib(f_t, \epsilon)$
can have a form of 
$$
f(x; ~ \epsilon, \delta) = \sum_{i=1}^m \frac{1}{2}(\sigma(x, \theta_i +\epsilon_i\delta_i)  
+ \sigma(x, \theta_i - \epsilon_i \delta_i)) + \sum_{i=m+1}^{m'} \epsilon_i \sigma(x, \vartheta_i),
$$
where $\epsilon_i$ denotes a step size parameter associated with the $i$-th split or grown neuron and satisfies $\epsilon_i \in [0, \epsilon]$. If $\epsilon_i$ it means the corresponding splitting/growing is turned off,
the $\delta_i$ and $\vartheta_i$ are the splitting direction. 
Therefore, the size of each $f \in \neib(f_t, \epsilon)$  is $C(f ) \leq \norm{\epsilon}_0.$
The weights of the new neurons and satisfies $\norm{\delta_i}_2\leq 1, \norm{\vartheta_i}_2
\leq 1$. 

\paragraph{Optimization}
Now the optimization reduces to 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot; ~\vv\epsilon, \vv\delta)) ~~~s.t.~~~ \norm{\vv \epsilon}_0 \leq \eta_{t+1},~~~\epsilon_i \in [0,\epsilon],~~~
\norm{\delta_i}_2 \leq 1.
$$
This amounts to a joint optimization of the $\delta_i$ vectors, and a combinatorial optimization of which $\epsilon$ should be turned off. 

Although this yields a combinatorial optimization due to the L0 constraint on $\epsilon$, we solve it with two simple steps: 

1) Optimizing $\vv \delta$ with that the sparsity constraint, that is $[\hat{\vv\epsilon}_0, \hat{\vv\delta}]=\argmin_{\vv \epsilon, \vv \delta} L(f(\cdot; ~\vv \epsilon, \vv\delta)) ~~~s.t.~~~ \epsilon_i \in [0,\epsilon],~~~\norm{\delta_i}_2 \leq 1$.

2) Optimizing $\vv \epsilon$. To do so, note that when $\epsilon$ is small, we have by Taylor expansion: 
$$
L_{f_t}(\vv\epsilon, \hat{\vv\delta})  = L_{f_t}(0,0)
+ \sum_{i=1}^{M}\epsilon_i g_i,~~~~~~~ \text{where}~~~ 
g_i = \nabla_{\epsilon_i }L_{f_t}(\hat{\vv\epsilon}_0, \hat{\vv\delta}).
$$
Therefore, we find the optimal $\epsilon $ by 
$$
\min_{ \vv\epsilon } \sum_{i=1}^M \epsilon_i g_i ~~~~s.t.~~~ \norm{\epsilon}_0 \leq \eta_{t},
$$
whose optimal solution amounts to select the neurons with the the most negative $g_i$. Precisely, we have 
%which amounts a solution of 
$$
\hat{\epsilon}_i = \ind(g_i \leq \min(0, g_{(\eta_t)})), 
$$
where $g_{(1)} \leq g_{(2)} \leq \cdots$ is the reordering of $\{g_i\}$ \qred{switch to integral gradient.} 

\paragraph{Growing New Layers}
Our framework is highly flexible, as it just need to define the candidate set of growing operators. 
We introduce how to grow new layers. 

Assume $f$ is a deep neural network of form $f = f_T \circ \cdots \circ f_{1}$. 
We consider 
\begin{align*} 
f' = f_T \circ (I +  h_{T-1}) \cdots  (I + h_2)\circ  f_2\circ (I+  h_1) \circ f_{1}, &&\text{with}&& h_{t}(x)= \sum_{i=1}^{m'} \epsilon_{i\ell} \sigma(x, \delta_{ti}).
\end{align*}
where  we insert new residual layers of form $I+ h_{t}$, 
with $\epsilon_{it} \in [0,\epsilon]$ controlling if the $i$-th neuron is turned on. For growing layers, we may want to ensure that the increase of both new layers and new neurons are controlled. %Formally, we can define $C(f) = \max(d)$
Note that $\norm{\vv\epsilon}_{0} = \sum_{i\ell} \ind(\epsilon_{i\ell}\neq 0)$ denotes the number new neurons introduced and 
$\norm{\vv\epsilon}_{0,\infty}=\sum_{\ell} \ind(\norm{\vv\epsilon_{i}}_{\infty} \neq 0)$ the number of new layers introduced. 
The optimizatoin can be framed into 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot~;~ \vv\epsilon, \vv\delta))  ~~~s.t.~~~ \norm{\vv\epsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\epsilon}_{0,\infty} \leq \eta_{t,1},~~ \norm{\delta_{it}} \leq 1. 
$$
The optimization can be solved similar the case of going wider in Section XXX. 
Similar to that case, we can first solve the optimal $\vv\delta$, and then using Taylor expansion 
the optimal $\vv\epsilon$ can be approximately found by 
$$
\min_{\vv\epsilon} \sum_{ti} \epsilon_{ti} g_{ti}~~~~~s.t.~~~~ \norm{\vv\epsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\epsilon}_{0,\infty} \leq \eta_{t,1},
$$
where $\epsilon_{ti} = \nabla_{\epsilon_{ti}} L(f(\cdot ~;~\vv \epsilon, \vv \delta))$. This solution of this can be obtained by sorting $g_{ti}$ in ascending order and select the neurons until $\norm{\vv\epsilon}_{0} \leq \eta_{t,0}$ or  $\norm{\vv\epsilon}_{0,\infty}$ is satisfied, or when the gradient becomes positive. \qred{but positive is not a problem; fix}

\paragraph{Remark} In practice, we can jointly apply any combinations of the above growing strategies to enlarge the network. As illustrated in the above examples, since Firefly Growing only requires an estimation of the gradient, it can be conveniently apply to different growing scenarios.
%Therefore, the complexity function can be defined as $C(f) - C(f_t) = $
%(x)= \sum_{i=1}^{m'} \sigma(x, \delta_{ti})$. 
%Let f


\subsection{Continual Learning} 
Continual learning (CL) studies the problem of learning a sequence of different tasks (datasets) $\mathcal D_t$ that arrive in a temporal order,
%
so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks $\{\mathcal D_k\}_{k=1}^t$. 
%
The major difficulty of CL is to avoid the \emph{catastrophic forgetting} problem, which means learning the new task will severely interfere with the knowledge learned previously and make the agent ``forget'' about how to do previous tasks.
Network growing provides a natural framework to address this problem because it allows to argument the network while keeping the previous neurons from the previous tasks unchanged. 

Inspired by [XXX], 
our approach is to keep track of a master network $f_{t}$
and a mask $m_s$ for each task $s \leq t$, such that $f_{t}$ applied with mask $m_s$ works for task $s$. 
When a new task $\D_{t+1}$ arrives, 
we grow the network to address the new task. 
The new neural network includes three types of neurons: 

1. The old neurons from the existing network, which does not introduce additional storage. 

2. Neurons inherited from neurons from $f_t$, but adjust copied to fit with the new task. This creates a new neuron and hence increases the storage demand. It is similar to splitting but the original copy is kept (except kept off for the new task).

3. Newly introduced neurons with small output weights. 

%To do so, 
For $f_t(x)=\sum_{i=1}^m \sigma(x; \theta_i^t)$, the growing region is 
$$
f(x; ~ \vv\epsilon, \vv\delta) = 
\sum_{i=1}^m \sigma(x; \theta_i^t + \epsilon_i \delta_i) + 
\sum_{i=m+1}^{m'} \epsilon_i \sigma(x; \delta_i). 
%\sigma(x; \theta_i^t + \epsilon \delta) 
$$
The new neurons introduced is $\norm{\vv\epsilon}_0$, including the relaxed neurons, and the newly introduced neurons. 
Therefore, the optimization reduces to 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot; ~\vv\epsilon, \vv\delta)) ~~~~s.t.~~~~ \norm{\vv\epsilon}_0\leq \eta_t, ~~ \norm{\vv\epsilon}_\infty \leq \epsilon, ~~~ \norm{\vv\delta}\leq 1. 
$$
It can be solved using the same method as before. 
After $f_{t+1}$ is constructed, the masks of the previous tasks are updated accordingly. 
%complexity
%is $C(f(\cdot; ~\vv\epsilon, \vv\delta)) = C(f_t) + $

%the 
%we selectively grow the network to 
%Let $f_t$ be the network for the $t$-th task. 
%
%
%
%
%

%
The performance of CL is evaluated in the end on all the tasks the agent has seen before. So when the $t$-th task arrives, for a parameterized learner, the general objective is to find the parameter $\theta_t$ that minimize the loss over all datasets:
\begin{equation}
    \theta_t = \arg\min_{\theta} \sum_{k=1}^t \mathcal{L}(\theta, \mathcal{D}_k).
\end{equation}
However, since the agent no longer has access to previous datasets, a popular surrogate objective is:
\begin{equation}
    \theta_t = \arg\min_{\theta} \mathcal{L}(\theta, \mathcal{D}_t) + D(\theta_t || \theta_{t-1}),
\end{equation}
where $\theta_t$ denotes the best parameter learned up to task $t-1$ and $D$ is some divergence measuring the similarity between $\theta_t$ and $\theta_{t-1}$. So the ideal $\theta_t$ should minimize the loss on current task while being close to the previous $\theta_{t-1}$ to preserve the performance on old tasks. Consider all $\theta_t \in \Omega$, then a common approach is to fix $\theta_{t-1}$ while growing some new neurons $\theta_{\text{new}}$ so that $\theta_t = \theta_{t-1} \oplus \theta_{\text{new}}$. Meanwhile, we can record a binary mask $m_t$ for task $t-1$ so that $\theta_{t-1} = m_t \odot \theta_t$. Clearly, it follows that $\theta_i = m_{i+1} \odot m_{i+2} \dots \odot m_t \odot \theta_t$, for all $i < t$. As one may have noticed, the key of success for this type of methods is to efficiently grow a small group of new neurons to achieve loss decreases as most as possible, which coincides with what FSD is designed for. Hence, we also consider using FSD as a novel growing method to solve CL.

% One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.

\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}

%%CL is a natural application of the FG method. \qred{write about our own methods first before listing the baselines}%
%To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.%
%We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. 
To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}

%\subsection{}
%$\epsilon_i \in [0, \epsilon]$ and $\norm{\delta}\leq 1 $ and $\vartheta_i\in \RR^d$. 
%$$f_{\vv\vartheta'}(x) =\underbrace{\sum_{i=1}^m \sum_{\ell=1}^k w_{i\ell} \sigma(x, \theta_{i\ell})}_{splitting} + \underbrace{\sum_{j=1}^{m'- k m} w_{j} \sigma(x, \theta_j)}_{growing~~new}$$
%$$\neib(f_{t}; \epsilon) = \{ f \colon ~~ f(x) =\underbrace{\sum_{i=1}^m \sum_{\ell=1}^{k_i} w_{i\ell} \sigma(x, \theta_{i}^t + \epsilon \delta_{i\ell})}_{splitting} +  \underbrace{\epsilon \sum_{j=1}^{k_0} w_{j} \sigma(x, \theta_j)}_{growing~~new} 
%(w_i , \theta_i) \colon ~~ \}$$
%\sum_{i\ell}\ind( \epsilon_i \neq 0) + \sum_j \ind(ep=0).$ 
%$C(f ) = \sum_{i\ell}\ind( w_{i\ell}\norm{\delta_{i\ell}}\neq 0) + \sum_j \ind(w_j=0).$
%k_i + k_0$. 

%It remains to solve the problem. To do so, we first solve $\tilde f_{t+1} = \argmin_{f} L(f)~~s.t.~~ f \in \neib(f_t, \epsilon),$ and then note that we $\epsilon$ is very small, we have $$f(x) = \sum_{i=1}^m \frac{1}{2}(\sigma(x, \theta_i +\epsilon_i\delta_i)  + \sigma(x, \theta_i - \epsilon_i \delta_i)) + \sum_{i=m+1}^{m'} \epsilon_i \sigma(x, \vartheta_i),
%$$where $\epsilon_i \in \{0,\epsilon\}$ and $\norm{\delta}\leq 1 $Minimizing $f$ in $\neib(f_t, \epsilon)$

%is an increasing sequence of  budget constraints \leq \cdots \leq \eta_t \leq \cdots \leq \eta_{\infty}=\eta$ is an increasing sequence ofand 
%$\vv\theta$
%Starting from a network $\vv\theta_t$ with $n$ neurons (which has already reached parametric optimum), our question is how to optimally grow it in an optimal, incremental way. 
%We consider growing wider first. 
%We want to grow the network with continous changes of the neuron. 
%There are two essential ways to grow the network. 
%1. Splitting neurons, in which we replace an existing neural $w_i\sigma(\theta_i, x)$  into $\sum_{k} w_i \sigma(\theta_{i}+\delta_{ik}, x).$2. Growing new neurons, in which we introduce new neurons with $w_{i,new}\sigma(\theta_{i,new}, x)$. 

%This is framed as augmenting the network to 
%$$f(x; \vv \theta, [\delta,\epsilon]) = \sum_{i=1}^m\sum_{i=1}^n w_{ik}\sigma(\theta_i + \delta_{ik}, x)  + \sum_{j=1}^{m'} w_{i}'\sigma(\theta_{i}', x)$$And then we want to optimize it 
%$$\min_{\delta, \epsilon \in N } L(\theta, [\delta], \epsilon).$$The idea is that when $\epsilon$ is sufficiently small, we can approximate it by first growing a lot and then prune?

%$$\min_{\theta'} L(\theta, \theta') s.t.~~~ \norm{\theta}_0\leq \eta, ~~~~ \norm{\theta'} \in N(0).  $$
%We solve this problem bycan approximate it by first growing a lot and then prune?

%$$\tilde \theta'=\argmin_{\theta'} L(\theta, \theta') s.t.~~~ \norm{\theta}_0\leq \eta, ~~~~ \norm{\theta'} \in N(0).  $$
%and then 
%$$\theta' = \arg\min L(\theta, \theta') + \lambda \norm{\theta'}_0\leq \eta. $$

%To formulate the problem of progressively growing a neural network, we can first equip each point $\theta_0 \in \Omega$ with a neighborhood $N(\theta_0, \epsilon)$, where $\epsilon$ describes the size of this neighborhood, and then look within this neighborhood for a new parameter $\theta$ such that the training loss mostly decreases. As a result, this procedure corresponds well to the idea of functional gradient descent. %\bo{I will try to add more to this part, but the transition to next section is still difficult.}


%
\subsection{Growing as Functional Steepest Descent}
Let $\Omega$ be the space of all possible models, i.e. models that have different parameters and architectures.
%
Consider, for example, the case of one-layer neural networks, 
we have $f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$, where $\vv \theta = [\theta_i]_{i=1}^n$.
%
Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$. This is an infinite dimensional space. In general, $\Omega$ can be much more complex for deep neural networks. To formulate the problem of progressively growing a neural network, we can first equip each point $\theta_0 \in \Omega$ with a neighborhood $N(\theta_0, \epsilon)$, where $\epsilon$ describes the size of this neighborhood, and then look within this neighborhood for a new parameter $\theta$ such that the training loss mostly decreases. As a result, this procedure corresponds well to the idea of functional gradient descent. \bo{I will try to add more to this part, but the transition to next section is still difficult.}
%
\subsection{Firefly Growing Framework}
Consider at the growing iteration $t$, the current neural network is parameterized by $\theta_t$ and denote $C(\theta_t)$ as the computational cost of the network, i.e. the total flops. The general objective of the Firefly Steepest Descent is therefore to find a new $\theta$ within a neighborhood of $\theta_t$ which decreases the loss the most under the constraint that $C(\theta)$ remains low. Formally, we consider the following iterative process:
%
\begin{equation}
    \label{eq:6}
    \theta_{t+1} \gets \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~ \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) - C(\theta_t) \leq \tau_t \right\}.
\end{equation}
%
Here $\tau_t$ is a predefined computational budget for the growth and $\epsilon$ is the parameter controlling the size of the neighborhood $N(\theta_t, \epsilon)$, i.e. $\epsilon$ can be the radius of the ball centered at $\theta_t$ in $\Omega$. Note that $\theta_{t+1}$ can have higher dimension than $\theta_t$. During practice, since the computational cost is mainly associated with the number of channels for each layer, we might just pick $\tau_t$ such that the number of increased channels is limited by a certain constant $M$. For optimization convenience, we consider a formulation equivalent to Equation \ref{eq:6} by optimizing over the perturbations around $\theta_t$. We also simply pick the $\ell_2$ norm constraint, though extensions to other norms are straightforward. Namely, let $\theta = \theta_t \oplus \delta_t$ (again, the dimensions are matched in the same way as when we compare $\theta_t$ and $\theta_{t+1}$; \red{still $\oplus$ is not defined mathematically}), then above update rule becomes:
%
\begin{equation}
    \label{eq:7}
    \delta_t \gets \arg\min_{||\delta_t||_2 \leq \epsilon} \left \{ L(\theta_t \oplus \delta_t) ~~~~s.t.~~~~ ||\theta_t \oplus \delta_t||_0 - ||\theta_t||_0\leq M \right\} \quad \text{and} \quad \theta_{t+1} &\gets \theta_t \oplus \delta_t ~.    
\end{equation}
To solve the above optimization, we consider the following two-step algorithm:\\\\
\textbf{Step 1}: transform the hard norm constraint into a norm penalty in the objective and solve $\delta_t$ without the $\ell_0$ constraint by running a small number of gradient descent steps:
\begin{equation}
    \hat{\delta}_t = \arg\min_{\delta} L(\theta_t \oplus \delta) + \lambda ||\delta||^2_2
\end{equation}
\textbf{Step 2}: project $\hat{\delta}_t$ back to satisfy the $\ell_0$ constraint, i.e. selecting the top-$M$ neurons that contribute the most to the loss decrease. Formally, let $\delta_t = z \odot \hat{\delta}_t$, where $z\in \{0, 1\}^n$ and $n$ is the dimension of $\hat{\delta}_t$. The objective can be formulated as:
\begin{equation}
    \min_z L(\theta_t \oplus (z \odot \hat{\delta_t})) ~~~~s.t.~~~~ ||z||_0 \leq M
\end{equation}
The possible choices of $z$ explode combinatorially when the dimension of $\hat{\delta}$ is large. Therefore, in practice, we estimate each neuron's contribution with the integrated gradient method. Namely,
\begin{equation}
    \Delta L = L(\theta_t \oplus \hat{\delta_t}) - L(\theta_t) = \int_{\alpha=0}^1 \nabla L(\theta_t \oplus \alpha \hat{\delta}_t) \cdot \hat{\delta_t} ~d\alpha.
\end{equation}
Expanding the gradient for individual parameter $\hat{\delta}_t^{(i)}$, we can formally define the contribution of each neuron and use monte-carlo method to approximate the integral:
\begin{equation}
\ref{eq:score}
\text{contribution}(\hat{\delta}_t^{(i)}) = \int_{\alpha=0}^1 \pdv{L(\theta_t \oplus \alpha \hat{\delta}_t)}{\alpha \hat{\delta}_t^{(i)}} \pdv{\alpha \hat{\delta}_t^{(i)}}{\alpha} d\alpha \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\delta}_t^{(i)})\bigg) \cdot \hat{\delta}_t^{(i)}.
\end{equation}
In practice, we find that with as small the $N$ as 3, the sampling can approximate the integral well. After the $\delta_t$ is found, FG simply expands the network according to $\delta_t$ and then resume the learning process. The whole pipeline of FG is summarized in Algorithm \ref{alg:firefly}.
\subsection{Three Growing Strategies}
\label{sec:str}
Next, we will discuss three different network growing strategies: 1) splitting existing neurons, 2) growing new neurons, and 3) introducing extra layers. For each of these strategies, we present its specific objective function as in step 1 of the FG framework. For illustration purpose, we will consider a neural network like $\Phi(\sigma(\theta, x))$, where $\theta$ is the neuron, $x$ is the input, $\sigma$ is the activation function, and $\Phi$ the mapping that maps the output of the neuron to the final output.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/firefly.pdf}
    \caption{Visual illustration of the three splitting methods. In all cases, FSD first expands the network as illustrated in the visualization and then train the corresponding $\delta$/$\bm{\Delta}$.}
    \label{fig:firefly_method}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Splitting Existing Neurons:} From Theorem 2.3 of \cite{splitting2019}, the optimal solution of greedily splitting existing neurons is to split them into two copies that have the opposite local updates. Formally, if a neuron $\theta$ were to be splitted, the optimal way is to split it into
$\Phi(\frac{1}{2}\sigma(\theta+\delta, x) + \frac{1}{2}\sigma(\theta-\delta, x))$,
where $\delta$ ideally should be along the direction of the mininum eigenvector of the splitting matrix, and the loss decrease are estimated by the corresponding minimum eigenvalue. Instead of solving the eigenvalues/eigenvectors exactly, FG trains the local perturbation $\delta$ with data to approximate the steepest descent direction, and then select the neurons based on the integrated gradient estimation. To summarize, for each neuron $\theta$ in the network, FG creates a corresponding $\delta$ that shares the same size as $\theta$, and then minimize the following:
\begin{equation}
\label{eq:split}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\frac{1}{2}\sigma(\theta+\delta, x) + \frac{1}{2}\sigma(\theta-\delta, x)\bigg) \bigg] + \lambda ||\delta||^2_2.
\end{equation}
After a few gradient steps, FG uses Equation \ref{eq:6} to select the $M$ neurons with the most contribution and only split these neurons according to their learned $\hat{\delta}$.
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/continual-learning.pdf}
    \caption{Illustration of how FSD performs continual learning. When the $t$-th task comes, FSD will iteratively grow the network until it solves the task and then record the corresponding network mask to reproduce the performance on task $t$ in the future.}
    \label{fig:my_label}
\end{figure}
\paragraph{Growing New Neurons:} As we will show in the experiment section, adding new neurons can be essential for FG to escape local minimums compared to pure splitting methods. Since we constrain the computation growth, we limit the algorithm to grow at most $M$ neurons. To make the functional gradient descent update continuous at the current architecture, when introducing these neurons, we initialize them around $0$ and give them a very small weight $\epsilon$. Formally, denote a new neuron as $\theta_{\text{new}} = \bm{0} + \delta$, we consider the following objective:
\begin{equation}
\label{eq:new}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta, x)  + \epsilon \cdot \sigma(\delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.
\end{equation}


\paragraph{Introducing Extra Layers:}
Denote the output of a layer as $\bm{h} = \sigma(\bm{W}\bm{x})$, where $\bm{W}$ is the weight matrix of the layer of interest. To introduce an extra layer, we can insert an identity mapping~\citep{chen2015net2net} layer on top of the current layer, i.e. $\bm{h} = \sigma(\bm{I}\sigma(\bm{W}\bm{x}))$\footnote{Note that this requires $\sigma$ satisfying $\sigma(\bm{I}\sigma(\bm{v})) = \sigma(\bm{v}),\forall \bm{v}$. ReLU is one example of this type of activations.}. Then the objective of finding new layers becomes:
\begin{equation}
    \hat{\bm{\Delta}} = \min_{\bm{\Delta}} \mathbb{E}_{\bm{x} \in \mathcal{D}} \bigg[
        \Phi \bigg(
            \sigma\big((\bm{I} + \bm{\Delta})\sigma(\bm{W}\bm{x})\big)
            \bigg)
    \bigg] + \lambda ||\bm{\Delta}||_F.
\end{equation}
After $\hat{\bm{\Delta}}$ is determined, we can similarly apply Equation~\ref{eq:6} to calculate the contribution of the entire layer by replacing every $\hat{\delta}$ with $\hat{\bm{\Delta}}$. On the other hand, since the contribution of the entire layer is just the sum of the contributions of each neuron, we could alternatively use that summation to approximate the contribution of the layer. Denote the $k$-th row of $\hat{\bm{\Delta}}$ as $\delta_k$ and assume $\hat{\bm{\Delta}}$ has $K$ rows in total ($K$ neurons at this layer), we then have:
\begin{equation}
\label{eq:score}
    \text{contribution}(\hat{\bm{\Delta}}) \approx  \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\bm{\Delta}}) \bigg) \cdot \hat{\bm{\Delta}} = \frac{1}{N}\bigg(\sum_{z=1}^N \sum_{k=1}^K \nabla L(\frac{2z-1}{2N}\delta_k) \bigg) \cdot \delta_k.
\end{equation}

\paragraph{Remark} In practice, we can jointly apply any combinations of the above growing strategies to enlarge the network. As illustrated in the above examples, since Firefly Growing only requires an estimation of the gradient, it can be conveniently apply to different growing scenarios.

\begin{algorithm*}[t] % enter the algorithm environment
\label{alg:main}
\caption{Firefly for Progressive Training of Neural Networks} 
\begin{algorithmic} % enter the algorithmic environment
%\begin{emumerate} 
\STATE \textbf{Input} : Search Space $S$. Initial small network $A_0$
\STATE Start from $A_0$.
%with random initialization, set the maximum neuron grow number $m^{*}_{total}$ or energy growth constraint $e^*_{total}$ each iteration and a threshold $|\lambda^*| > 0$ to stop. Repeat the following 4 steps below until the stop criterion is met:
\STATE \textbf{Repeat} Until the stop criterion is met
\STATE At step $t$
\STATE \textbf{1.} Train $A_t$ for several epochs to decrease the loss. 
    \vspace{.3\baselineskip} 
    \STATE \textbf{2.} Expand $A_t$ to a larger neighbor network $A_t'$ by adding a set of neurons $n_t$ in the search space $D$
    \vspace{.3\baselineskip} 
    \STATE \textbf{3.} Train $A_t'$ for several iterations, select the best subset of neurons in $n_t$ using our method. Keep these neurons in the network and drop the rest of the neurons in $n_t$ to get the new network $A_{t+1}$
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}

\begin{algorithm*}[t] % enter the algorithm environment
\caption{Firefly Steepest Descent for Continual Learning} 
\begin{algorithmic} % enter the algorithmic environment
    \STATE \textbf{Input} : a stream of datasets $\{\mathcal{D}_1, \mathcal{D}_2, \dots, \mathcal{D}_K\}$, an initial network $A_0$.
    \FOR{task $k=1:K$}
        \STATE Denote $A_k = A_{k-1}$.
        \IF{$k = 1$}
            \STATE Train $A_1$ for several epochs until convergence.
        \ENDIF
        \WHILE{$A_k$ cannot solve task $k$}
            \IF{$k = 1$}
                \STATE Grow $A_k$ with the \textbf{split}-existing-neuron and grow-new-neuron strategies.
            \ELSE
                \STATE Grow $A_k$ with the \textbf{duplicate}-existing-neuron and grow-new-neuron strategies.
            \ENDIF 
            \STATE minimize $L(\mathcal{D}_k, A_k)$ for several epochs until convergence.
        \ENDWHILE
        \STATE Record the network mask $m_k$ for $A_k$.
    \ENDFOR
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}

\subsection{Continual Learning} 
Continual learning (CL) studies the problem of learning a sequence of different tasks (datasets) $\mathcal D_t$ that arrive in a temporal order,
%
so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks $\{\mathcal D_k\}_{k=1}^t$. 
%
The major difficulty of CL is to avoid the \emph{catastrophic forgetting} problem, which means learning the new task will severely interfere with the knowledge learned previously and make the agent ``forget'' about how to do previous tasks.
%
The performance of CL is evaluated in the end on all the tasks the agent has seen before. So when the $t$-th task arrives, for a parameterized learner, the general objective is to find the parameter $\theta_t$ that minimize the loss over all datasets:
\begin{equation}
    \theta_t = \arg\min_{\theta} \sum_{k=1}^t \mathcal{L}(\theta, \mathcal{D}_k).
\end{equation}
However, since the agent no longer has access to previous datasets, a popular surrogate objective is:
\begin{equation}
    \theta_t = \arg\min_{\theta} \mathcal{L}(\theta, \mathcal{D}_t) + D(\theta_t || \theta_{t-1}),
\end{equation}
where $\theta_t$ denotes the best parameter learned up to task $t-1$ and $D$ is some divergence measuring the similarity between $\theta_t$ and $\theta_{t-1}$. So the ideal $\theta_t$ should minimize the loss on current task while being close to the previous $\theta_{t-1}$ to preserve the performance on old tasks. Consider all $\theta_t \in \Omega$, then a common approach is to fix $\theta_{t-1}$ while growing some new neurons $\theta_{\text{new}}$ so that $\theta_t = \theta_{t-1} \oplus \theta_{\text{new}}$. Meanwhile, we can record a binary mask $m_t$ for task $t-1$ so that $\theta_{t-1} = m_t \odot \theta_t$. Clearly, it follows that $\theta_i = m_{i+1} \odot m_{i+2} \dots \odot m_t \odot \theta_t$, for all $i < t$. As one may have noticed, the key of success for this type of methods is to efficiently grow a small group of new neurons to achieve loss decreases as most as possible, which coincides with what FSD is designed for. Hence, we also consider using FSD as a novel growing method to solve CL.

% One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.

\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}

%%CL is a natural application of the FG method. \qred{write about our own methods first before listing the baselines}%
%To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.%
%We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. 
To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}


==> Firefly splitting/content/abstract.tex <==
\begin{abstract}
We propose \emph{firefly neural architecture descent}, a general framework for progressively and dynamically growing neural networks to jointly optimize the networks' parameters and architectures. 
%
Our method works in a steepest descent fashion, which iteratively finds the best network within a functional neighborhood of the original network 
that includes a diverse set of candidate network structures. 
%
By using Taylor approximation, the optimal network structure in the neighborhood can be found with a greedy selection procedure.
%
We show that firefly descent can flexibly grow networks both wider and deeper, and can be applied to learn accurate but resource-efficient neural architectures that avoid catastrophic forgetting in continual learning.
%
Empirically, firefly descent achieves promising results on both neural architecture search and continual learning. In particular, on a challenging continual image classification task, it learns networks that are smaller in size but have higher average accuracy than those learned by the state-of-the-art methods.
\end{abstract}

==> Firefly splitting/content/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we present a simple but highly flexible framework for progressively growing neural networks in a principled steepest descent fashion. 
%
Our framework allows us to incorporate various mechanisms for growing networks (both in width and depth).
%
Furthermore, we demonstrate the effectiveness of our method on both growing networks on both single tasks and continual learning problems, in which our method consistently achieves the best results. Future work can investigate various other growing methods for specific applications under the general framework.  

==> Firefly splitting/content/experiment.tex <==
\section{Experiment}\label{sec:experiments}
In this section, we present three sets of experiments to showcase the power of FG for both neural architecture optimization and continuous learning. 
Across various tasks, we find our method tends to much smaller and computationally efficient architecture with higher performance than existing methods. 
In particular, we find method singificantly outperforms the state-of-the-art m continuous learning methods, including xXX and XXX, all of which also progressively grow neural networks to adapt to new tasks.  

We start with a toy RBF network experiment  in Section XXX 
to demonstrate the advantage of FG over the splitting steepest descent \citep{splitting2019, wu2020signed}, 
%, compared with the second-order splitting method, is less likely to get stuck at local minimums. 
%
and then evaluate our 
FG on neural architecture search (NAS) for 
image classification, in terms of both growing wider and deeper.  
We apply our method to continual learning (CL) 
and compare it against the state-of-the-art method \qred{(name some methods?)} that also continuously grow a network. 

\subsection{Toy RBF Network} \label{sec:toy}
%One problem with the second-order splitting method is that it is more likely to get stuck at local minimums. Because the method considers only the local curvature around the origininal minimum, and more importantly, it can only split existing neurons. To illustrate this problem, 
For the purpose of illustration, 
we start with testing our methods on growing an one-dimensional two-layer radial-basis function (RBF) neural network with one-dimensional inputs, %which is of the form: 
\begin{equation} 
\label{equ:rbf}
f(x) = \sum_{i=1}^{m} w_i \sigma(\theta_{i1} x + \theta_{i2}), \quad \text{where } ~~\sigma(t) = \exp (-\frac{t^2}{2}), ~~~~~x \in \RR, 
\end{equation}
\qred{how do you generate the parameters?}
where $w_i \in \mathbb R$ and $\theta_i = [\theta_{1i},\theta_{2i}]$ are the input and output weights of the $i$-th neuron, respectively. We generate our true function by drawing $m = 15$ neurons with $w_i$ and $\theta_i$ i.i.d. from  $\normal(0,3)$. 
For dataset $\{x^{(\ell)}, y^{(\ell)}\}_{\ell=1}^{1000}$, we generate them
with $x^{(\ell)}$ drawing from $\mathrm{Uniform}([-5,5])$ and let $y^{(\ell)} = f(x^{(\ell)})$.
We apply various growing methods to grow the network from one single neuron all the way up to 12 neurons. 

\emph{Random Splitting} ({\tt Random (Splitting)}): When growing the network, we randomly select one of the existing neurons from the network, split it into two copies, set the output weight to be half value of the original one and give each of them a small random perturbation.

\emph{Random Splitting+New} ({\tt Random (Splitting+New)}): \red{Should not also have as baseline as well?} We introduce 5 newly initialized neurons drawn from $\mathcal{N}(0, 0.1)$ with a small output weights and list them as well as the existing neurons in the network as the candidate set. We randomly choose one neuron from the candidate set, if we choose the newly initialized neuron, we directly add them in the network. And if we select the existing neurons, we split it using the same operation as the {\tt Random Splitting} case.

\emph{Splitting steepest descent} ({\tt Steepest Splitting}):  We following the algorithm of \cite{splitting2019}. We choose one neuron to split and set the perturbation step size $\epsilon = 0.01$.

\emph{Firefly steepest descent} ({\tt Firefly (Splitting only)}): 
\qred{Some key parameters are missing, such as how many neurons we split and add before pruning. We need to do an ablation study on it...} We only apply splitting existing neurons operation described in Section \ref{sec:str} here. After expand the network, we train for 5 iterations and choose the neuron with the highest contribution score defined in \ref{eq:score}. 


\emph{Firefly steepest descent} ({\tt Firefly (Splitting+New)}): 
We apply our algorithm \ref{alg:main}, and deploy 
the splitting and introducing-new-neuron strategies defined in \ref{eq:split} and \ref{eq:new}.   
We add 5 new neurons which are initialized from $\mathcal{N}(0, 0.1)$ and split the existing neurons in the network into two copies. After expanding the network, we will select the neuron with best score after training for 5 iterations.

\emph{Training from scratch} ({\tt Scratch)}): We also train networks of different sizes directly, without progressive growing. 

All the growing methods above add one neuron at each step. We update 10,000 iterations between two consecutive growing. Furthermore, to make sure the results are consistent, we generate one fixed true function, run the experiments 20 times with different generated datasets and report the averaged training loss of the network at each stage of growing in Figure~\ref{fig:toy} \qred{are models randomized everytime as well?}.

Figure \ref{fig:toy}a shows the \red{training loss} as we grow the network size. We can see that 
%w.r.t. the size of the learned network 
{\tt Firefly (Splitting+New)} tends to achieve nearly-zero loss, suggesting that it can efficiently escape local optimum via growing. 
\red{{\tt Random (Splitting+New)}  considers the same space of growing operations, but is clearly less efficient.}
In contrast, methods that only include splitting operators are more likely to get stuck, domenstrating the benefit of adding \red{new random neurons (need fix the name)}. 
%tends to find minimize the training loss 
\red{all splitting methods can get stuck} (never make such absolute claim, and it is your own method.......) at a local minimum and the training loss will no longer decrease from there on. By contrast, FG can more easily escape local minimums and achieve near zero training loss with as few as 6 neurons.



 To study the contribution scores and the integral approximation method described in \ref{eq:score}, we choose one case when the network has $m = 3$ neurons. We expand the network by applying {\tt Firefly (Splitting+New)}, which will split the three existing neurons and introduce 5 new neurons in. After training the expanded network for 5 iterations, we sort the neurons using contribution score, select one of them adding into the network and fintune the network for 10,000 iterations.  Figrue \ref{fig:toy}b shows the relationship between the score rank and the loss after fintuneing when applying different integral steps. We can see from the figure that adding the neuron with a high contribution score will help the network converge better. In addition, more integral steps will lead a better approximation, and as a result, the score rank will 
have a better correlation with the loss after finetune.

%which randomly chooses a neuron to split, and the train from scratch (scratch) method which trains a network of the same size from sctach. For all of the growing methods, we apply them to grow the RBF network from $1$ neuron all the way up to $12$ neurons and draw the corresponding loss curves. 


%In this section, we present three sets of experiments to showcase the strength of FG. Firstly, we adopt a toy RBF network experiment to demonstrate that FG, compared with the second-order splitting method, is less likely to get stuck at local minimums. Then we evaluate FG's performance on Neural Architecture Search (NAS) problems with standard image classification datasets. To further illustrate potential usage of the FG method, we apply it to a continual learning problem and compare it against the state-of-the-art method that also iteratively grow a network. As we will show, FG can learn a much smaller architecture with less computation resource and achieve even higher performance.

%\subsection{Toy RBF Network}
%One problem with the second-order splitting method is that it is more likely to get stuck at local minimums. Because the method considers only the local curvature around the origininal minimum, and more importantly, it can only split existing neurons. To illustrate this problem, we consider growing a two-layer radial-basis function (RBF) neural network with one-dimensional inputs, which is of the form:
%\begin{equation} 
%\label{equ:rbf}
%f(x) = \sum_{i=1}^{m} w_i \sigma(\theta_{i1} x + \theta_{i2}), \quad \text{where } ~~\sigma(t) = \exp (-\frac{t^2}{2}).
%\end{equation}
%Here, $w_i \in \mathbb R$ are the weights of each neuron, and $\theta_{i1}$ and $\theta_{i2}$ are the first layer weights and biases. Specifically, we consider baselines including the steepest descent splitting method (splitting), the random splitting method (random splitting) which randomly chooses a neuron to split, and the train from scratch (scratch) method which trains a network of the same size from sctach. For all of the growing methods, we apply them to grow the RBF network from $1$ neuron all the way up to $12$ neurons and draw the corresponding loss curves. For FG, we apply the splitting and introducing-new-neuron strategies. When introducing new neurons, the neurons are initialized from $\mathcal{N}(0, 0.1)$. At each growing iteration, FG uses one epoch of training to estimate the steepest descent gradient as well as determining which neurons to expand. For all methods, we update 10,000 iterations between two consecutive growing. Furthermore, to make sure the results are consistent, we run the experiments 20 times and report the averaged training loss of the network at each stage of growing in Figure~\ref{fig:toy}.

\begin{figure}[ht!]
    \centering
    \begin{tabular}{cc}
    \raisebox{3.0em}{\rotatebox{90}{{ Loss}}}~\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png} &
    \raisebox{3.0em}{\rotatebox{90}{{ Loss after training}}}~\includegraphics[width=0.45\textwidth]{figures/rbf/score.png}\\
         Number of neurons & Score Rank
         \\
         (a) & (b)\\
    \end{tabular}
    
    \caption{
    \qred{[shorter]}
    \red{TODO: Add random splitting + new baseline here}
    (a) Average loss under 20 runs. 
    (b) The relationship between the contribution score and loss after finetuning when applying different $N$ when $m = 3$.
    }
    \label{fig:toy}
\end{figure}



\subsection{Growing Wider and Deeper Networks}\label{sec:expwider}
We test the effectiveness of our method for growing network width and growing depth, respectively. We use standard image classification tasks on MINST and CIFAR10 as benchmark.  
%of networks for standard image classification tasks. 
\paragraph{Growing width} \qred{result feels not strong with a single figure?}
We compare our method with Splitting Steepest Descent \citep{splitting2019} and Net2Net uniform grow baselines on CIFAR-10 using VGG19 to test FG's performance on widening a deep network. \qred{use bullet like earlier}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{1\baselineskip}
    
    \begin{tabular}{c}
     %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
     \hspace{-1.5em}\raisebox{3.0em}{\rotatebox{90}{{ Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/VGG/percent.pdf}\\
         %Number of neurons & 
         Parameter size ratio
    \end{tabular}
    
    \caption{Widening \qred{wider? more information} VGG19 on CIFAR10 \qred{turn to a wrapfigure}
    }
    \label{fig:cifar}
\end{wrapfigure}

For Net2Net, which uniform grow network by randomly choose the existing neurons to split in each layer. \qred{better to have an independent sentence explain "we compare with Net2Net, which uniform grow network by xx and xx (do they have both splitting and new?) " } Start with a small VGG19 network with a $0.125\times$ multiplier applies on each layer, we grow $30\%$ of the neurons in each layers each time.

For Splitting Steepest Descent and our method, we start with a small VGG19 network with 16 channels in each layer. When applying Splitting Steepest Descent, we follow the setting in \citep{splitting2019} and split $30\%$ neurons in the network each time.

For Firefly steepest descent, we apply splitting and introducting new neurons together. When expanding the network we split all the neurons in the network and additionally add $50$ new neurons in each layer. In the selecting phase, we train the network with new neurons for 1 epoch and select the top $30\%$ of the new neurons based on the contribution score. 

In addition, between two grow steps using the methods above, the network will be finetuned with 160 epochs.

From Figure \ref{fig:cifar}, we can see our Firefly performance outperform the other two growing method and outperform the Full size VGG19's performance using less than 10\% parameters. 


\paragraph{Growing depth} To evaluate FG's performance on deepening a network, we compare against AutoGrow \cite{wen2019autogrow} and Uniform Network Morphsim \citep{wei2016network} that can also introduce new layers. We follow the AutoGrow's experiment setting and choose the same MNIST and CIFAR-10 dataset. For AutoGrow, we build 3 blocks with 1 layer in each block as the initial network. The first layer in each block are set with stride = 2 to decrease the feature map's resolution. For Network Morphsim and FG, we start with a network having one layer with 16 channels in each blocks. Each step, for Network Morphsim, we randomly add one layer in a block.  For AutoGrow, we follow the setting in the paper and grow the layer with pre-defined layer width. And for FG, we pre-define 10 identity layers in each blocks and grow the depths.


\begin{table}[ht!]
\centering
\begin{tabular}{c|c|ccc}

\hline
  \multicolumn{2}{c|}{ }&Structure& Param (M) & Accuracy\\
\hline

\multirow{3}*{MNIST} & AutoGrow & 20-20-20 & 212 & 99.66 \\

& Firefly & 16-15-16 & \textbf{154} &99.66 \\
& Network Morphsim & 23-22-18 & 253 &99.64 \\

\hline
\multirow{2}*{CIFAR10} & AutoGrow & 23-22-22 & 342 & 90.84 \\

& Firefly & - & - &- \\

\hline

\end{tabular}
\caption{Growing Depth }
\end{table}






\subsection{Application on Neural Architecture Search}
\label{sec:expDarts}
We apply our method to improve cell-based Neural Architecture Search (NAS)\citep[e.g.][]{ zoph2018learning, liu2018progressive, real2019regularized}. The idea of cell-based NAS is to learn an optimal neural network module (called cell), from a predefined search space, such that networks constructed from multiple cells can achieve good performance. A cell is a directed graph with $N$ nodes as $N$ latent space. There are several edges between the nodes that can be assigned with the operations in the predefined search space. 



%\qred{improve. need a full course explaination of cell-based. "The idea of cell-based NAS is to learn an optimal neural network module (called cell), from a predefined search space, such that networks constructed from the cell can achieve good performance. The search space of the cells consists of xxxx."}


Following the cell's setting in DARTS \citep{liu2018darts}, we search the structure on the cell with 7 nodes. Our targets is to search the best choice of the operations between each node pairs. We specially modify the operations choice into SepConv$3 \times 3$, SepConv$5 \times 5$, DilConv $3 \times 3$, DilConv $5 \times 5$ and Identity to better formulate our growing strategy. When build up the cell, SepConv$3 \times 3$, SepConv$5 \times 5$, DilConv $3 \times 3$, Dil Conv $5 \times 5$ will be add as operations between each Nodes in the cell and their output result will be sum up as the state of the Node on the output direction.


% \qred{without setting up what we want to do with NAS, i do not know what is going on here.}
% Comparing with other growing method, FG is capable of determining the importance of each layer \qred{(of what?)} globally \qred{what do you mean?}. In addition, FG can more efficiently determine the layer type in each cells by jointly growing all the layer types in the search space and keep only the layer with the most contribution. As a result, FG also achieves very good search efficiency, which is a major bottleneck of contemporary splitting methods. \qred{tell me what you do before saying that FG is good.}

 
To apply our method to cell-based NAS, we first build our search network with 5 stacked cell at the beginning. Among these 5 cells, the second and the fourth one is placed with a special cell called the reduction cell, which contains the operation with stride two to decrease the resolution of the feature map. At beginning, the operations' channels are set to be ${4, 8, 8, 16, 16}$ in each cells. We then progressively train and grow the network. Between every 10 epochs' training on the whole network, we choose one cel and grow all the operations using our Firefly splitting and adding new neurons strategy. Each time when expand the network, we introduce 16 new neurons and split all the existing neurons. In the selection phase, we keep $25\%$ new neurons with the highest contribution score. We totally train the network for 100 epochs with the cell grow order 1-2-3-4-5-1-2-3-4-5 which means each cell will be grow for twice. The overall training setting keep the same as DARTS.

After we finish the search, We select the widest layer as the final search result between each nodes. In addition, if all the layers between two nodes are grow less than $50\%$ comparing with the initial width, we select the identity operation as the search result.


\begin{table}[ht!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c|ccc}
    \hline
        Method & Search Time (GPU Days) & Param (M) & Error  \\
        \hline
        DenseNet-BC \citep{huang2018condensenet} & - & 25.6 & $3.46$
         \\
         \hline
         PNAS \citep{liu2018progressive}& 225 & 3.2 & $3.41$
         \\
         ENAS \citep{pham2018efficient} & 4 & 4.2 & $2.91$
         \\
         Random Search & 4 & 3.2 & $3.29 \pm 0.15$
         \\
      
          DARTS (first order) \citep{liu2018darts} & 1.5 & 3.3 & $3.00 \pm 0.14 $ \\

          DARTS (second order) \citep{liu2018darts}  & 4 & 3.3 & $ 2.76 \pm 0.09$ \\

          Firefly & 1.5 & 3.3 & $ 2.78 \pm 0.05 $  \\
          \hline
    \end{tabular}
    }
    \caption{Performance compared with several NAS baseline}
    \label{tab:nas}
\end{table}

\subsection{Continual Learning}\label{sec:expCL}
%Continual learning (CL) studies the problem of learning a sequence of different tasks in an online fashion so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks. The performance of CL is evaluated in the end on all the tasks the agent has seen before. As a result, the major difficulty of CL is to avoid the catastrophic forgetting problem, which is prominent on rich function approximators like the neural networks. One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.
%\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}
We test our method for continuous learning.  
%CL is a natural application of the FG method.
\qred{write about our own methods first before listing the baselines} 
%
To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.
%
We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}

During implementation, we apply both the copy-exist-neuron and grow-new-neuron strategies to tackle the CL problem. During each growing iteration, we add $15$ new neurons for each layer as candidates for growing. During the selection phase, we select out the top 256 neurons among all the copied neurons and new neurons, for learning the new task. Following the setup in CPG, we finetune 50 epochs for each sub-task.
% Continual learning is another task that perfectly suitable for a growing network. When the new data stream comes, the original network may lack the capacity to remember the new knowledge. Using a large network or separately use several individual model to learn the task may solve the question, however it will be super expensive when we face a large number of tasks situation. So we want to gradually grow the network to meet the growing demand of the network capacity when the new task comes. Moreover, we can better select and use the knowledge from the previous 
% task to support the newly grow network to fit the new task.


% When the training start, the tasks will come one by one as a data stream, the previous task's training data can not be retrieved after it is passed. To prevent the previous task from forgetting when training the new task data, we train the network start from a small network and gradually grow the network while keeping the previous learned neurons' weight fixed. 

% \bo{maybe we can introduce copying as another growing strategy.}
% Specifically saying, suppose we are training the network with task i. When task i is finished and task i + 1 comes, we first use a mask i to fix the weight for task i and prevent it from further update and grow the network using our firefly method. While growing, we keep the original output weight unchanged to prevent the forgetting on the original data. Each time, we add 15 new neurons as well as the splitting neurons copy from the original network at the expansion phase in each layer. Note that to keep the performance of the original network, we set the output weight of the splitting neurons to 1 instead of 0.5. In the selection phase, we train the expanded network for 50 epochs to better fit the new tasks and keep the top 256 neurons as the candidate neurons for the new task.
% After the Firefly operation is done for task i + 1, we together finetune these newly added neurons for task i + 1 with the previous fixed neurons as the parameter for task i + 1. 

Start from a small VGG16 with 32 channels in each layer, we repeat the procedure above and gradually grow our network capacity to adapt the new tasks while keep the old task's performance unchanged. After the training, we can retrieve the task i's model according to the corresponding mask i.

We randomly split CIFAR-100 into 10 and 20 random tasks and compare with some recent baselines including learn-to-grow \citep{li2019learn} and CPG \citep{hung2019compacting} which is the state of the art method on continuous learning tasks. Figure \ref{fig:cl}, Table \ref{tab:cl10} and Tabel \ref{tab:cl20} shows the result.

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|ccc}
    \hline
        Method &  Param (M) & Accuracy  \\
        \hline
          EWC & 6.55  & 74.23
         \\
           HAT & 6.83 & 74.52
         \\
          Learn-to-grow  & 6.86 & 76.21
         \\
          Firefly & 5.63 & \textbf{82.43} \\

          \hline
    \end{tabular}
    \caption{\red{TODO: Add param vs accuracy plot here} 10 random split CIFAR-100}
    \label{tab:cl10}
\end{table}

% \begin{table}[ht!]
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \scalebox{0.8}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%         Method&1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 &  9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 &  19&  20 & avg  \\
%         \hline
%          Individual & 86.8 &	83.2 &	91.6&	93.6 &	89.0&	94.0&	92.4&	79.6&	89.6&	88.6&	94.6&	80.6&	90.6&	88.2&	87.4&	90.8&	88.6&	93.8&	91.6&	82.6&  88.85 \\
%         \hline
%          CPG& 87.0 &	84.0 &	91.4&	95.6 &	91.2&	96.6&	93.0&	80.0&	90.0&	90.8&	95.6&	85.8&	92.4&	89.8&	89.4&	91.8&	89.6&	93.8&	92.8&	83.2&  90.19 \\
%          \hline
%          Firefly & 87.8 & 90.8 & 94.6 & 89.2 & 94.2 & 96.2 & 91.4 & 92.8 & 92.8 & 90.4 & 93.4 & 88.0 & 90.0 & 91.0 & 90.4 & 86.4 & 89.8 & 94.2 & 84.6 & 82.8 &  \textbf{90.53}


\begin{figure}
    \centering
    \begin{tabular}{c}
     %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
     \raisebox{3.0em}{\rotatebox{90}{{ Average Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/cl/cl_20.png}\\
         %Number of neurons & 
         Task ID
    \end{tabular}
    
    \caption{Average accuracy on 20 random split CIFAR-100 dataset over 3 runs. Individual means train each task from scratch using the Full VGG16.
    }
    \label{fig:cl}
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|ccccc}
    \hline
        Method &  Model Size (M) & Avg. Training epochs & Avg. Selecting epochs & Avg. Accuracy  \\
        \hline
          Individual &2565 & 100 & 0& 88.85
         \\
           CPG & 289 & 100 & 420 &90.75
         \\
           CPG w/o FC & 28 & 100 & 420 &90.58
         \\
          Firefly & 26 & 100 & 50 & \textbf{91.03} \\

          \hline
    \end{tabular}
    \caption{Cost of time and space on different method. CPG w/o FC means remove the fully connection layers before the classification layers in CPG to align the model size with Firefly. The average training epoch represents the average epochs taken in fitting the new tasks. The selecting epoch means iteratively pruning and training piggymasks for CPG, means expansion and selection phase for Firefly.   }
    \label{tab:cl20}
\end{table}










==> Firefly splitting/content/experimentshort.tex <==
\section{Empirical Results}\label{sec:experiments}
We conduct four sets of experiments to verify the effectiveness of firefly neural architecture descent.  
%
In particular, we first demonstrate the importance of introducing additional growing operations beyond neuron splitting \citep{splitting2019} 
%
and then apply the firefly descent to both neural architecture search and continual learning problems. In both applications, firefly descent finds competitive but more compact networks in a relatively shorter time compared to state-of-the-art approaches.

\paragraph{Toy RBF Network} \label{sec:toy} We start with growing a toy single-layer network to demonstrate the importance of introducing brand new neurons over pure neuron splitting. In addition, we show the local greedy selection in firefly descent is efficient by comparing it against random search.
%
Specifically, we adopt a simple two-layer radial-basis function (RBF) network with one-dimensional input and compare various methods that grow the network gradually from 1 to 10 neurons. 
%
The training data consists of 1000 data points from a randomly generated RBF network. 
%
We consider the following methods: 
%
{\tt Firefly}:  firefly descent for growing wider by splitting neuron and adding upto $m'=5$ brand new neurons; 
{\tt Firefly (split)}:  
 firefly descent for growing wider with only neuron splitting (e.g., $m'=0$);  
 {\tt Splitting}: the steepest splitting descent of \citet{splitting2019}; 
%
{\tt RandSearch (split)}: randomly selecting one neuron and splitting in a random direction, repeated $k$ times to pick the best as the actual split; we take $k=3$ to match the time cost with our method;
%
{\tt 
RandSearch (split+new)}: the same as  {\tt RandSearch (split)} but with 5 randomly initialized brand new neurons in the candidate during the random selecting;
%
{\tt Scratch}: training networks with fixed structures starting from scratch. 
%
We repeat each experiment 20 times with different ground-truth RBF networks and report the mean training loss in Figure~\ref{fig:toy}(a).

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/rbf/rbf.pdf}
    \caption{(a) Average training loss of different growing methods versus the number of grown neurons. (b) Firefly descent with different numbers of new neuron candidates.}
    \label{fig:toy}
    \vspace{-10pt}
\end{figure}

As shown in Figure~\ref{fig:toy}~(a), the methods with pure neuron splitting (without adding brand new neurons) can easily get stuck at a relatively large training loss and splitting further does not help escape the local minimum.  
%
In comparison, all methods that introduce additional brand new neurons can optimize the training loss to zero. Moreover, {\tt Firefly} grows neural network the better than random search under the same candidate set of growing operations.

We also conduct a parameter sensitivity analysis on $m'$ in Figure~\ref{fig:toy}(b), which shows the result of {\tt Firefly} as we change the number $m'$ of the brand new neurons. We can see that the performance improves significantly by even just adding one brand new neuron in this case, and the improvement saturates when $m'$ is sufficiently large ($m'=5$ in this case).

\paragraph{Growing Wider and Deeper Networks}\label{sec:expwider} We test the effectiveness of firefly descent for both growing network width and depth.
%
We use VGG-19~\citep{simonyan2014very} as the backbone network structure and compare our method with splitting steepest descent \citep{splitting2019}, 
%
Net2Net \citep{chen2015net2net} which grows networks uniformly by randomly selecting the existing neurons in each layer,
%
and neural architecture search by hill-climbing (NASH) \citep{elsken2017simple}, which is a random sampling search method using network morphism on CIFAR-10. 
%
For Net2Net, the network is initialized as a thinner version of VGG-19,  
whose layers are
$0.125\times$ the original sizes. 
%
For splitting steepest descent, NASH, and our method,  
we initialize the VGG-19 with 16 channels in each layer.  
%
%
For firefly descent,  we grow a network by both splitting  existing neurons and adding brand new neurons for widening the  network;  
we add $m'=50$ brand new neurons  
and set the budget to grow the size by $30\%$ at each step of  our method. 
See Appendix \ref{app:grow} for more information on the setting. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/VGG/cifar.pdf}
    \caption{(a) Results of growing increasingly wider networks on CIFAR-10; VGG-19 is used as the backbone. (b) Computation time spent on growing for different methods.
    }
    \label{fig:cifar}
\end{figure}
%new neurons 
%


% \begin{figure}[ht]
%     \centering
%     \vspace{-0.5\baselineskip}
%     \renewcommand\arraystretch{1.3}
%     \scalebox{0.85}{
    
%     \begin{tabular}{cc}
%       \raisebox{3.5em}{\rotatebox{90}{{\small Accuracy}}}~\includegraphics[width=0.37\textwidth]{figures/VGG/cifar10.pdf} & \hspace{5em}\raisebox{3.5em}{\rotatebox{90}{{\small Time (s)}}}~\includegraphics[width=0.37\textwidth]{figures/VGG/cifar10_time.pdf} \\
%         Model ratio &\hspace{5em} Method \\
%         (a) & \hspace{5em} (b)
%     \end{tabular}
%     }
%     \caption{Widening VGG19 on CIFAR10\qq{Results when growing increasingly wider networks on CIFAR10; VGG19 is used as the backbone.}
%     }
%     \label{fig:cifar}
%     \vspace{-1\baselineskip}
% \end{figure}

Figure~\ref{fig:cifar} (a) shows the test accuracy, where the x-axis is the percentage of the grown model's size over the standard VGG-19.
We can see that 
%
the proposed method clearly outperforms the \emph{splittting steepest descent} and  Net2Net.
In particular, we %it can also quickly 
achieve comparable test accuracy as the full model with only $4\%$ of the full model's size. Figure~\ref{fig:cifar}(b) shows the average time cost of each growing method for one step, we can see that {\tt Firefly} performs much faster than splitting the steepest descent and NASH. 
%
We also applied our method 
to gradually grow new layers in neural networks, 
we compare our method with NASH \citep{elsken2017simple} and AutoGrow \citep{wen2019autogrow}.
%
Due to the page limit, we defer the detailed results to Appendix \ref{app:grow}.

\paragraph{Cell-Based Neural Architecture Search}
\label{sec:expDarts} Next, we apply our method as a new way for improving cell-based Neural Architecture Search (NAS) \citep[e.g.][]{  zoph2018learning, liu2018progressive, real2019regularized}. 
%
The idea of cell-based NAS is to learn optimal neural network modules (called cells), from a predefined search space, 
such that they serve as good building blocks 
to composite complex neural networks. Previous works mainly focus on using reinforcement learning or gradient based methods to learn a sparse cell structure from a predefined parametric template. Our method instead gradually grows a small parametric template during training and obtains the final network structure according to the growing pattern.

Following the setting in DARTS \citep{liu2018darts}, 
we build up the cells as computational graphs whose structure is the directed DAG with 7 nodes.
% in which the cells %are computational graphs  
% the computational graph whose structure is the directed DAG with 7 nodes.\bo{fix this sentence?}
%
The edges between the nodes
are linear combinations of different computational operations (SepConv and DilConv of different sizes) and the identity map. 
%
To grow the cells, 
we apply firefly descent to grow 
the number of channels in each operation by both splitting existing neurons and adding brand new neurons. 
%If all the operations on each edge grow very slow, we choose the identity map as the final choice. 
%we the candidate operations is added as layers between nodes in the cell and their output results are summed up as output. 
%
%We stack 5 cells sequentially as a network for searching the best operation choice. 
%At the beginning, the number of channels in each operation is set to be a small one.We train the network and apply firefly descent to gradually grow the channels for all the operations in the cells by both splitting existing neurons and adding brand new neurons. 
%After several rounds of training and growing, we select the operation with the largest channels between each node as our final choice. In addition, if all the operations between each two nodes pair grow very slow, we choose the Identity map as the final choice. More details of the experiment setup can be found in Appendix \ref{app:nas}
%When growing cells, we composite a network by stacking 5 networks ....to evaluate the loss of the cells \qq{[get my original sentence back..]} 
%Then we apply the search result on a 20 sequentially stacked cells network  for the final training.
During search, we compose a network by 
stacking 5 cells sequentially to evaluate the quality of the cell structures. We train 100 epochs in total for searching, and grow the cells every 10 epochs. After training, the operation with the largest number of channels on edge is selected into the final cell structure. In addition, if the operations on the same edge all only grow a small amount of channels compared with the initial setting, we select the Identity operation instead. The network that we use in the final evaluation is a larger network consisting of 20 sequentially stacked cells.  %trained on the 
More details of the experimental setup can be found in Appendix \ref{app:nas}. 

%During testing, 
%
%
% ======


% ==== old merge to appendix===
% Following the setting in DARTS  \citep{liu2018darts}, 
% %
% we search the structure on cells\qq{remove and change to ", in which the cells are computational graphs .." }, 
% the computational graph whose structure is the directed DAG \qq{a fully connected directed  acyclic  graph (DAG)} with 7 nodes. 
% %
% The edges between each nodes\qq{between the nodes} represent the operations that transfer one nodes to another\qq{computation operators that process the nodes}.
% %
% Our targets\qq{target} is to find the best operation choice between each node pairs. We keep the operation choices SepConv$3 \times 3$,  SepConv$5 \times 5$, DilConv $3 \times 3$, DilConv $5 \times 5$ 
% and Identity map same as DARTS configure and remove AvegPooling3x3 and MaxPooling3x3 and Zero because they do not have parameters.

% When building up the cell, 
% the candidate operations is added as layers between nodes in the cell and their output results are summed up as output. 
% %
% We stack 5 cells sequentially as a network for searching the best operation choice. At the beginning, the number of channels in each operation is set to be a small one. We train the network and apply firefly descent to gradually grow the channels for all the operations in the cells by both splitting existing neurons and adding brand new neurons. After several rounds of training and growing, we select the operation with the largest channels between each node as our final choice. In addition, if all the operations between each two nodes pair grow very slow, we choose the Identity map as the final choice. More details of the experiment setup can be found in Appendix \ref{app:nas}

% Then we apply the search result on a 20 sequentially stacked cells network  for the final training.
% \qq{during search, we compose a network by 
% stacking 5 cells sequentially to evaluate the quality of the cell structures. 
% The network that we use in the final evaluation is a larger network consisting of 20 sequentially stacked cells.  %trained on the 
% }
%During testing, 
%
%
% ======



Table \ref{tab:nas} reports the results 
comparing {\tt Firefly} with several NAS baselines. 
%
Our method achieves a similar or better performance comparing with those RL-based and gradient-based methods like ENAS or DARTS, but with higher computational efficiency in terms of the total search time.
\begin{table}[h]
\parbox{1.0\linewidth}{
\renewcommand\arraystretch{1.0}
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c|c cc}
    \hlineB{2.5}
        Method & Search Time (GPU Days) & Param (M) & Error  \\
        % DenseNet-BC \citep{huang2018condensenet} & - & 25.6 & $3.46$
        %  \\
         \hline
         NASNet-A \citep{zoph2018learning}& 2000 & 3.1 & $2.83$
         \\
         ENAS \citep{pham2018efficient} & 4 & 4.2 & $2.91$
         \\
         Random Search & 4 & 3.2 & $3.29 \pm 0.15$
         \\
      
          DARTS (first order) \citep{liu2018darts} & 1.5 & 3.3 & $3.00 \pm 0.14 $ \\

          DARTS (second order) \citep{liu2018darts}  & 4 & 3.3 & $ 2.76 \pm 0.09$ \\

          {\tt Firefly} & 1.5 & 3.3 & $ 2.78 \pm 0.05 $  \\
    \hlineB{2.5}
    \end{tabular}
    }
    \vspace{5pt}
    \caption{Performance compared with several NAS baseline}
    \label{tab:nas}
   }
   \vspace{-15pt}
\end{table}


\begin{figure}[t!]
    \centering
    \begin{tabular}{c}
         \includegraphics[width=0.95\textwidth]{figures/cl/cl.pdf}
    \end{tabular}
    \caption{(a) Average accuracy on 10-way split of CIFAR-100 under different model size. We compare against Elastic Weight Consolidation (EWC)~\citep{kirkpatrick2017overcoming}, Dynamic Expandable Network (DEN)~\citep{yoon2017lifelong}, Reinforced Continual Learning (RCL)~\citep{xu2018reinforced} and Compact-Pick-Grow (CPG)~\citep{hung2019compacting}. (b) Average accuracy on 20-way split of CIFAR-100 dataset over 3 runs. Individual means train each task from scratch using the Full VGG-16.}
    \label{fig:cl}
    \vspace{-10pt}
\end{figure}

\textbf{Continual Learning}
\label{sec:expCL}~~
Finally, we apply our method to grow networks  for  continual learning (CL), and compare with two state-of-the-art methods,  Compact-Pick-Grow (CPG) \citep{hung2019compacting} and  Learn-to-grow~\citep{li2019learn},  
both of which also progressively grow neural networks for learning  new tasks.
%
For our method, we grow the networks starting from a thin variant of the original VGG-16 without fully connected layers. 

Following the setting in Learn-to-Grow, we construct 10 tasks by randomly partitioning CIFAR-100 into 10 subsets. 
Figure~\ref{fig:cl}(a) shows the average accuracy and size of models at the end of the 10 tasks learned by firefly descent, Learn-to-Grow, CPG and other CL baselines.
We can see that firefly descent learns smaller networks with higher accuracy. 
%
%
%
%
To further compare with CPG, we follow the setting of their original paper \citep{hung2019compacting} and randomly partition CIFAR-100 to 20 subsets of 5 classes to construct 20 tasks.
Table~\ref{tab:cl20} shows the average accuracy and size learned at the end of 20 tasks. Extra growing epochs refers to the epochs used for selecting the neurons for the next upcoming tasks, and {\tt Individual} refers to training a different model for each task. We can see that firefly descent learns the smallest network that achieves the best performance among all methods. Moreover, it is more 
computationally efficient than CPG when growing and picking the neurons for the new tasks. 
Figure~\ref{fig:cl}(b) shows the average accuracy over seen tasks on the fly. Again, firefly descent outperforms CPG by a significant margin.



















%,  and 
%of models 
%\citet{}, 
%shows model size vs. accuracy 
%As shown 
%We split\qq{use partition, splitting has special meaning in this paper} CIFAR-100 into 10 random tasks for comparing with Learn-to-Grow as well as other baselines and  adaptively change our grow ratio to control the size of the final model. 
%
%We also split\qq{parttion} CIFAR-100 into 20 random tasks to compare with CPG and Individual model which means train each task separately use an Full size VGG16.
%\qq{it feels strange. why compare different baselines with different parition. need an explaination }
%
%We let each method learn\qq{do not use phrases like "let your algorithm learn.."  } on the stream of those tasks and report the average accuracy across tasks on the fly in Figure~\ref{fig:cl}. \qq{we report in figurexx 
%the average accuracy across tasks of different methods. 
%}
%
%In addition, we also report the average accuracy and  the model size of the final model in Table~\ref{tab:cl20}. 
%
%We provide more details about the experiment setup in Appendix \ref{app:cl}.
%
%We can see from Figure 5 (a)\qq{space or not?} that we achieve a higher performance on 20-way split of CIFAR-100 comparing with Individually training each task from scratch and the state-of-the-art method CPG. 
%
%Table \ref{tab:cl20} further compare the model size and the extra epochs for expanding and picking neurons with Individual training, 
%CPG and CPG without fully connected layers that align the size with {\tt Firefly}. 
%
%We show our method get a higher performance with a much efficient space and time consumption.

% \begin{figure}
%     \centering
%     \renewcommand\arraystretch{1.3}
%     \begin{tabular}{cc}
%      %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
%      \raisebox{3.0em}{\rotatebox{90}{{ Average Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/cl/cl.pdf} & \raisebox{3.0em}{\rotatebox{90}{{ Average Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/cl/cl10.pdf}\\
%          %Number of neurons & 
%          \vspace{-3pt} Task ID & Param (M)\\
%          (a) & (b)
%     \end{tabular}
%     \caption{(a) Average accuracy on 20-way split of CIFAR-100 dataset over 3 runs. Individual means train each task from scratch using the Full VGG16. (b) Average accuracy on 10-way split of CIFAR-100 under different model size. 
%     }
%     \label{fig:cl}
% \end{figure}

% \begin{figure}
%  \centering
%  \hspace{-1.0em}\parbox{0.6\textwidth}{
%     \scalebox{0.85}{
%     \begin{tabular}{cc}
%      %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
%      \hspace{-1em} \raisebox{1.5em}{\rotatebox{90}{{ \small Average Accuracy}}}~\includegraphics[width=0.3\textwidth]{figures/cl/cl.pdf} & 
%      \hspace{-1em}
%      \raisebox{1.5em}{\rotatebox{90}{{ \small Average Accuracy}}}~\includegraphics[width=0.3\textwidth]{figures/cl/cl10.pdf}
%      \vspace{-1em}\\
%          %Number of neurons & 
%          { Task ID} & \hspace{-.5em}{ Param (M)}\vspace{-1em}\\
%           (a) &\hspace{-.5em}(b) \vspace{-1em}\\
%     \end{tabular}}
%     \caption{(Average accuracy on (a) 20-way split of CIFAR-100 over 3 runs.  (b) 10-way split of CIFAR-100 under different model size.
%     }}
%     \vspace{-0.7em}
%         \parbox{0.35\linewidth}{

% \centering
% \renewcommand\arraystretch{1.0}
% \vspace{1em}
% \scalebox{0.7}{
%     \hspace{-1.5em}
%     \begin{tabular}{c|cp{1cm}<{\centering}c}
%     \toprule
%           Method     &  Param(M)   & Extra Epochs & Accuracy \\
%     \midrule
%           Individual  & 2565        & 0            & 88.85 \\
%           CPG        & 289         & 420          & 90.75 \\
%           CPG w/o FC & 28          & 420          & 90.58 \\
%           {\tt Firefly}     & \textbf{26} & \textbf{50}  & \textbf{91.03} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:cl20}
% \caption{20-way split of CIFAR-100, CPG w/o FC is to align the model structure and model size with {\tt Firefly}}
% }
% \vspace{-1.5em}
% \label{fig:cl}
% \end{figure}


























% \begin{table}[ht!]
% \renewcommand\arraystretch{1.0}
%     \centering
%     \begin{tabular}{c|ccc}
%     \toprule
%         Method &  Param (M) & Accuracy  \\
%     \midrule
%           EWC & 6.55  & 74.23
%          \\
%           HAT & 6.83 & 74.52
%          \\
%           Learn-to-grow  & 6.86 & 76.21
%          \\
%           Firefly & 5.63 & \textbf{82.43} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\red{TODO: Add param vs accuracy plot here} 10 random split CIFAR-100}
%     \label{tab:cl10}
% \end{table}

\begin{table}[h]
\renewcommand\arraystretch{1.0}
    \centering
    \begin{tabular}{c|ccc}
    \hlineB{2.5}
        Method &  Param (M) & Extra Growing Epochs & Avg. Accuracy (20 tasks) \\
    \hline
          Individual  & 2565  & -   & 88.85
         \\
          CPG        & 289   & 420 & 90.75
         \\
          CPG w/o FC \footnotemark  & 28    & 420 & 90.58
         \\
          Firefly     & \textbf{26}    & \textbf{80}  & \textbf{91.03} \\
    \hlineB{2.5}
    \end{tabular}
    \vspace{5pt}
    \caption{20-way split continual image classification on CIFAR-100.} 
    \label{tab:cl20}
\end{table}
\footnotetext[4]{CPG without fully connected layers is to align the model structure and model size with {\tt Firefly}.}

% \begin{table}[ht!]
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \scalebox{0.8}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%         Method&1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 &  9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 &  19&  20 & avg  \\
%         \hline
%          Individual & 86.8 &	83.2 &	91.6&	93.6 &	89.0&	94.0&	92.4&	79.6&	89.6&	88.6&	94.6&	80.6&	90.6&	88.2&	87.4&	90.8&	88.6&	93.8&	91.6&	82.6&  88.85 \\
%         \hline
%          CPG& 87.0 &	84.0 &	91.4&	95.6 &	91.2&	96.6&	93.0&	80.0&	90.0&	90.8&	95.6&	85.8&	92.4&	89.8&	89.4&	91.8&	89.6&	93.8&	92.8&	83.2&  90.19 \\
%          \hline
%          Firefly & 87.8 & 90.8 & 94.6 & 89.2 & 94.2 & 96.2 & 91.4 & 92.8 & 92.8 & 90.4 & 93.4 & 88.0 & 90.0 & 91.0 & 90.4 & 86.4 & 89.8 & 94.2 & 84.6 & 82.8 &  \textbf{90.53}











==> Firefly splitting/content/funding.tex <==
\section*{Funding Transparency Statement}
\textbf{Funding Disclosure:} NSF
(CPS-1739964, IIS-1724157, NRI-1925082, CAREER-1846421, SenSE-2037267, EAGER-2041327), ONR (N00014-18-2243), FLI (RFP2-000), ARO (W911NF-19-2-0333), DARPA, Lockheed Martin, GM, and Bosch.

Peter Stone serves as the Executive Director of Sony AI America and receives financial compensation for this work.  The terms of this
arrangement have been reviewed and approved by the University of Texas
at Austin in accordance with its policy on objectivity in research.

==> Firefly splitting/content/impact.tex <==
\section*{Broader Impact}
This work develops a new framework that can grow neural networks simply and efficiently, which can be generally used in various applications that using neural networks and positively enhance their capacity and performance. In particular, we anticipate it can be applied on devices which have hard memory/computation constraint, i.e. mobile devices or robots. Our work does not have any negative societal impacts.

==> Firefly splitting/content/intro.tex <==
\section{Introduction}
Although biological brains are developed and shaped by complex progressive growing processes, most existing artificial deep neural networks are trained under fixed network structures (or architectures).
%
Efficient techniques that can progressively grow neural network structures can allow us to jointly optimize the network parameters and structures to achieve higher accuracy and computational efficiency, especially in dynamically changing environments.
%
% For example,
% recent works \citep[e.g.,][]{splitting2019, wang2019energy} 
% show that accurate and energy-efficient neural architectures can be learned by progressively growing network structures starting from a relatively small network.
% Moreover, both Net2Net~\citep{chen2015net2net} and the Network Morphism~\citep{wei2016network} argue that knowledge learned from previous tasks can be transferred to new and more complex tasks by expanding the network trained on previous tasks to a functionally-equivalent larger network to initialize the new tasks.
For instance, it has been shown that accurate and energy-efficient neural network can be learned by progressively growing the network architecture starting from a relatively small network~\citep{splitting2019, wang2019energy}. Moreover, previous works also indicate that knowledge acquired from previous tasks can be transferred to new and more complex tasks by expanding the network trained on previous tasks to a functionally-equivalent larger network to initialize the new tasks~\citep{chen2015net2net, wei2016network}.
%

In addition, dynamically growing neural network has also been proposed as a promising approach for preventing the challenging \emph{catastrophic forgetting} problem in continual learning~\citep{rusu2016progressive, yoon2017lifelong, rosenfeld2018incremental, li2019learn}.

Unfortunately, searching for the optimal way to grow a network 
leads to a challenging combinatorial optimization problem. 
Most existing works use simple heuristics  \citep{chen2015net2net, wei2016network}, or  
 random search \citep{elsken2017simple, elsken2018efficient} to grow networks and may not fully unlock the power of network growing. 
%
An exception is  splitting steepest descent~\citep{splitting2019},
which considers growing networks by splitting the existing neurons into multiple copies, and derives a principled functional steepest-descent approach for 
determining which neurons to split and how to split them.
%
However, the method is restricted to neuron splitting, and can not incorporate more flexible ways for growing networks, including adding brand new neurons and introducing new layers. 


In this work, we propose \emph{firefly neural architecture descent}, % (Firefly), 
 a general and flexible framework for progressively growing neural networks.  
%
Our method is a local descent algorithm 
inspired by the typical gradient descent and  splitting steepest descent. 
%
It grows a network by  
 finding the best larger networks 
 in a \emph{functional neighborhood} of the original network whose size is controlled by a step size $\epsilon$, 
 which contains a rich set of networks that have various (more complex) structures, but are $\epsilon$-close to the original network in terms of the function that they represent.
 The key idea is that, when $\epsilon$ is small,  
 the combinatorial optimization on the
 functional neighborhood 
 can be simplified to a greedy selection, and therefore can be solved efficiently in practice.
%

The firefly neural architecture descent framework is highly flexible and practical
and allows us to derive general approaches for growing wider and deeper networks (Section~\ref{sec:grow-width}-\ref{sec:grow_layers}).  
%
It can be easily customized to address specific problems. For example, our method 
provides a powerful approach for dynamic network growing in continual learning (Section~\ref{sec:cl}), and 
can be applied to optimize cell structures in cell-based neural architecture search (NAS) such as DARTS \citep{liu2018darts} (Section~\ref{sec:expDarts}). Experiments show that Firefly  efficiently learns accurate and resource-efficient networks in various settings.
In particular, for continual learning, 
our method learns more accurate and smaller networks  
that can better prevent catastrophic forgetting, 
outperforming state-of-the-art methods such as Learn-to-Grow~\citep{li2019learn} and Compact-Pick-Grow~\citep{hung2019compacting}. 

==> Firefly splitting/content/method.tex <==
\section{Firefly Neural Architecture Descent}
In this section, we start with introducing the general framework (Section~\ref{sec:general}) of firefly neural architecture descent. % (Firefly).
Then we discuss how the framework can be applied to grow a network both wider and deeper  (Section~\ref{sec:grow-width}-\ref{sec:grow_layers}). To illustrate the flexibility of the framework, 
we demonstrate how it can help tackle catastrophic forgetting in continual learning  (Section~\ref{sec:cl}). 
%
\subsection{The General Framework}
\label{sec:general} 
We start with the general problem of jointly optimizing neural network parameters and model structures.  
Let $\Omega$ be a space of neural networks with different parameters and structures (e.g., networks of various widths and depths). Our goal is to solve
\begin{align} \label{equ:Lf}
\argmin_{f}
\Big \{ L(f) ~~~s.t. ~~~ f\in \Omega,  ~~~ C(f) \leq \eta \Big\}, 
\end{align}
where $L(f)$ is the training loss function and $C(f)$ is a complexity measure of the network structure that reflects the computational or memory cost. This formulation poses a highly challenging optimization problem in a complex, hierarchically  structured space. 
%\bo{from Peter: what does it mean by heuristically structured space.}


We approach \eqref{equ:Lf} 
with a steepest descent type algorithm that generalizes typical parametric gradient descent and the splitting steepest descent of \citet{splitting2019}, 
with an iterative update of the form
\begin{align} \label{equ:masterupdate}
f_{t+1} = \argmin_{f} \Big \{ L(f) ~~~~s.t.~~~  f \in \neib(f_t, ~\epsilon),~~~~~~ 
C(f) \leq C(f_t)+\eta_{t} \Big\}, 
\end{align}
where we find the best network $f_{t+1}$ in 
neighborhood set $\neib(f_t, ~\epsilon)$ of the current network $f_t$ in $\Omega$, whose complexity cannot exceed that of $f_t$ by more than a threshold $\eta_t$. 
%
Here $\neib(f_t, ~\epsilon)$ denotes a neighborhood of  $f_t$ of ``radius'' $\epsilon$ such that $f(x) = f_t(x) +O(\epsilon)$ for $\forall f\in \neib(f_t, ~\epsilon)$. $\epsilon$ can be viewed as a small step size, which ensures that the network changes smoothly across iterations, and importantly, 
 allows us to use Taylor expansion to significantly simplify the optimization \eqref{equ:masterupdate} to yield practically efficient algorithms.  
%
 
The update rule in \eqref{equ:masterupdate} is highly flexible and reduces to different algorithms with different choices of $\eta_t$ and $\neib(f_t, \epsilon)$.
%
In particular, when $\epsilon$ is infinitesimal, by taking $\eta_t = 0$ and $\neib(f_t, \epsilon)$ the typical Euclidean ball on the parameters, \eqref{equ:masterupdate} reduces to standard gradient descent which updates the network parameters with architecture fixed.
%
However, by taking $\eta_t > 0$ and $\neib(f_t, \epsilon)$ a rich set of neural networks with different, larger network structures than $f_t$, we obtain novel \emph{architecture descent} rules that allow us to incrementally grow networks. 
   
   In practice, we alternate between parametric descent and architecture descent according to a user-defined schedule (see Algorithm~\ref{alg:main}). Because architecture descent increases the network size, it is called less frequently (e.g., only when a parametric local optimum is reached). From the optimization perspective, 
   performing architecture descent allows us to lift the optimization into a higher dimensional space with more parameters, and hence escape local optima that cannot be escaped in the lower dimensional space (of the smaller models). 
   
   In the sequel, we instantiate the neighborhood $\neib(f_t, ~\epsilon)$ for growing wider and deeper networks, and for continual learning, and discuss how to solve the optimization in \eqref{equ:masterupdate} efficiently in practice. 
 
\begin{algorithm*}[t] % enter the algorithm environment
    \label{alg:main}
    \caption{Firefly Neural Architecture Descent}  %\qred{improve}}  
    \begin{algorithmic} % enter the algorithmic environment
        \STATE \textbf{Input}: 
        %Search Space $\Omega$. 
        Loss function $L(f)$; 
        initial small network $f_0$; 
        search neighborhood $\neib(f, \epsilon)$; 
        maximum increase of size $\{\eta_t\}$. 
        \STATE \textbf{Repeat:} At the $t$-th growing phase:
            \STATE \textbf{1.} Optimize the parameter of $f_t$ with fixed structure using a typical optimizer for several epochs.
            \STATE \textbf{2.} Minimize $L(f)$ in $f \in \neib(f, \epsilon)$ without the complexity constraint (see e.g., \eqref{equ:wideroptwithno}) to get a large ``over-grown'' network $\tilde f_{t+1}$ by performing gradient descent.
            \STATE \textbf{3.}  Select the top $\eta_t$ neurons in $\tilde f_{t+1}$ with the highest importance measures to get $f_{t+1}$ (see \eqref{equ:epsilonoptwide}).  
    \end{algorithmic}
    \label{alg:firefly}  
\end{algorithm*}





\subsection{Growing Network Width}
\label{sec:grow-width} 
We discuss how to define $\neib(f_t, \epsilon)$ to progressively build increasingly wider networks, and then introduce how to efficiently solve the optimization in practice.   
%
We illustrate the idea with two-layer networks, but extension to multiple layers works straightforwardly. 
%
Assume $f_t$ is a two-layer neural network (with one hidden layer) of the form  $f_t(x) = \sum_{i=1}^{m} \sigma(x, \theta_i)$, 
where $\sigma(x, \theta_i)$ denotes its $i$-th neuron with parameter $\theta_i$ and $m$ is the number of neurons (a.k.a. width).
There are two ways to introduce new neurons 
to build a wider network, 
including splitting existing neurons in $f_t$ and introducing brand new neurons; see Figure~\ref{fig:firefly_method}. 
%
\paragraph{Splitting Existing Neurons} Following \citet{splitting2019},
an essential approach to growing neural networks is to 
split the neurons into a linear combination of multiple similar neurons. 
Formally, 
splitting a neuron $\theta_i$\footnote{A neuron is determined by both $\sigma$ and $\theta$. But since $\sigma$ is fixed under our discussion, we abuse the notation and use $\theta$ to represent a neuron.} into a set of neurons $\{\theta_{i\ell}\}$ with weights $\{w_{i\ell}\}$ 
amounts to replacing $\sigma(x, \theta_i)$ in $f_t$ with $\sum_{\ell } w_{i\ell} \sigma(x, \theta_{i\ell})$. 
We shall require that 
$\sum_{\ell} w_{i\ell} =1$ and $\norm{\theta_{i\ell} - \theta}_2 \leq \epsilon,$ $\forall \ell$ so that the new network is $\epsilon$-close to the original network. 
%This ensures that the network output after splitting remains similar to the original network when $\epsilon$ is small.
As argued in \citet{splitting2019}, when $f_t$ reaches a parametric local optimum and $w_{i\ell} \geq 0$, 
it is sufficient to consider a simple binary splitting scheme, which splits a neuron $\theta_i$ into two equally weighted copies along opposite update directions, that is, 
$\sigma(x, \theta_i) 
\Rightarrow 
 \frac{1}{2} \big ( \sigma(x, \theta_i + \epsilon \delta_{i}) 
 + \sigma(x, \theta_i -  \epsilon \delta_i)     
\big )
$, where $\delta_i$ denotes the update direction.

\paragraph{Growing New Neurons}  Splitting the existing neurons yields a ``local'' change 
because the parameters of the new neurons are close to that of the original neurons. 
%
A way to introduce ``non-local'' updates is to add brand new neurons with arbitrary parameters far away from the existing neurons. 
%
This is achieved by replacing $f_t$ with 
$f_t(x) + \epsilon\sigma(x, \delta)$, 
where $\delta$ now denotes a trainable parameter of the new neuron and the neuron is multiplied by $\epsilon$ to ensure the new network is close to $f_t$ in function. 
%This introduces new ``non-local'' information that can not be achieved by splitting neurons. 
%, this update is non-local and hence may help jump out of local optima. 
%with a small output weight. This amounts to replace $f_\theta$ with $f_\theta(x) + w_i' \sigma$
%Motivated by \citep{splitting2019}, we re
%$$f_{\vv\vartheta'}(x) =\sum_{i=1}^{m'} w_i \sigma(x,\theta'_i).$$Such that for each $j$, we need 

Overall, 
to grow $f_t(x) = \sum_i \sigma(x; \theta_i)$ wider, 
the neighborhood set $\neib(f_t, \epsilon)$ can include functions of the form
%\qq{here it is possible to }
%inclue a  %\eqref{equ:masterupdate} can be defined to include a combination of possible neuron splitting and growing. Formally, 
%for $f_t(x) = \sum_i \sigma(x; \theta_i)$, 
%we let $\neib(f_t, \epsilon)$ to consist of functions of form 
%we define 
%the augmented neural networks in $\neib(f_t, \epsilon)$
%can have a form of 
$$
f_{\vv\varepsilon,\vv\delta}(x) = \sum_{i=1}^m \frac{1}{2}\Big (\sigma(x, \theta_i +\varepsilon_i\delta_i)  
+ \sigma(x, \theta_i - \varepsilon_i \delta_i) \Big ) + \sum_{i=m+1}^{m+m'} \varepsilon_i \sigma(x, \delta_i),
$$
where we can potentially split all the neurons in $f_t$ and add upto $m'$ new non-local neurons ($m'$ is a hyperparameter). 
Whether each new neuron will eventually be added is  controlled by an individual step-size $\varepsilon_i$ that satisfies $|\varepsilon_i| \leq \epsilon$. If $\varepsilon_i = 0$, it means the corresponding new neuron is not introduced. 
%splitting/growing is turned off,
%the $\delta_i$ and $\vartheta_i$ are the splitting direction. 
Therefore, the number of new neurons introduced in  $f_{\vv\varepsilon, \vv\delta}$  equals the $\ell_0$ norm 
$\norm{\vv\varepsilon}_0 := \sum_{i=1}^{m+m'} \ind(\varepsilon_i = 0)$. % of $\vv\varepsilon$.
Here  $\vv\varepsilon = [\varepsilon_i]_{i=1}^{m+m'}$ and $\vv\delta = [\delta_i]_{i=1}^{m+m'}$. 
%= [\varepsilon_i]_{i=1}^{m+m'}.$  
%Overall, the 

Under this setting, the optimization in \eqref{equ:masterupdate} can be framed as 
\begin{align} \label{equ:wideropt}
\min_{\vv\varepsilon, \vv\delta}\Big\{  L(f_{\vv\varepsilon, \vv\delta}) ~~~s.t.~~~ \norm{\vv\varepsilon}_0 \leq \eta_{t},~~~\norm{\vv\varepsilon}_\infty \leq \epsilon,~~~
\norm{\vv\delta}_{2,\infty} \leq 1 \Big\},
\end{align}
where $\norm{\vv\delta}_{2,\infty}=\max_i \norm{\delta_i}_2$, which is constructed to prevent $\norm{\delta_i}_2$ from becoming arbitrarily large. 
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/firefly.pdf}
    \caption{An illustration of three different growing methods within firefly neural architecture descent. Both $\delta$ and $h$ are trainable perturbations.}
    \label{fig:firefly_method}
\end{figure}
\paragraph{Optimization} It remains to solve the optimization in \eqref{equ:wideropt}, 
which is challenging due to the $\ell_0$ constraint on $\vv\varepsilon$. 
%Now the optimization reduces to 
%$$\min_{\vv\varepsilon, \vv\delta} L(f(\cdot; ~\vv\varepsilon, \vv\delta)) ~~~s.t.~~~ \norm{\vv\varepsilon}_0 \leq \eta_{t+1},~~~\varepsilon_i \in [0,\epsilon],~~~\norm{\delta_i}_2 \leq \lambda .$$%This amounts to a joint optimization of the $\delta_i$ vectors, and a combinatorial optimization of which $\epsilon$ should be turned off. 
%Although this yields a combinatorial optimization due to the L0 constraint on $\epsilon$, 
%By exploiting that the 
However, when the step size $\epsilon$ is small,  
we can solve it approximately with a simple two-step method: we first optimize $\vv \delta$ and $\vv\varepsilon$ while dropping the $\ell_0$ constraint, and then re-optimize $\vv\varepsilon$ with Taylor approximation on the loss, which amounts to simply picking the new neurons with the largest contribution to the decrease of loss, measured by the  gradient magnitude. 

\emph{Step One.} Optimizing $\vv \delta$ and $\vv\varepsilon$ without the sparsity constraint $\norm{\vv\varepsilon}_0
\leq \eta_t$, that is,  
\begin{align} \label{equ:wideroptwithno}
[\tilde{\vv\varepsilon}, \tilde{\vv\delta}]=\argmin_{\vv\varepsilon, \vv\delta} \Big \{ L(f_{\vv\varepsilon, \vv\delta})
~~~s.t.~~~ 
%\norm{\vv\varepsilon}_0 \leq \eta_{t},~~~
\norm{\vv\varepsilon}_\infty \leq \epsilon,~~~
\norm{\vv\delta}_{2,\infty} \leq 1 \Big\}.%~~~s.t.~~~|\varepsilon_i| \leq \epsilon,~~~\norm{\delta_i}_2 \leq 1, ~~~\forall i \in [m+m'] \bigg\},
\end{align} 
In practice, we solve the optimization with gradient descent by 
turning the constraint into a penalty. 
Because $\epsilon$ is small, we only need to perform a small number of gradient descent steps.  

\emph{Step Two.} Re-optimizing $\vv\varepsilon$ with Taylor approximation on the loss. To do so, note that when $\epsilon$ is small, we have by Taylor expansion: 
$$
L(f_{\vv\varepsilon, \tilde{\vv\delta}})  = L(f)
 ~+~ \sum_{i=1}^{m+m'}\varepsilon_i s_i ~+~ O(\epsilon^2),~~~~~~~ %\text{where}~~~ 
s_i = \frac{1}{\tilde\varepsilon_i}\int_{0}^{\tilde \varepsilon_i}\nabla_{\zeta_i} L(f_{[\tilde{\vv\varepsilon}_{\neg i}, \zeta_i], \tilde{\vv\delta}}) d \zeta_i,
$$
where $[\tilde{\vv\varepsilon}_{\neg i}, \zeta_i]$ denotes 
replacing the $i$-th element of $\tilde{\vv\varepsilon}$ with $\zeta_i$, and $s_i$ is an integrated gradient that measures the contribution of turning on the $i$-th new neuron. In practice, we approximate the integration in $s_i$ by discrete sampling:  %\red{XXXXX} \qred{Or simplify to the typical gradient?}.
 $s_i \approx \frac{1}{n} \sum_{z=1}^{n} \nabla_{c_z} L(f_{[\tilde{\vv\varepsilon}_{\neg i}, c_z], \tilde{\vv\delta}})$ with $c_z =({2z-1})/{2n} \tilde{\varepsilon}_i$ and $n$ a small integer (e.g., $3$). 
%$s_i \approx \frac{1}{n} \sum_{z=1}^{n} \nabla_{c_z} L(f_{[\tilde{\vv\varepsilon}_{\neg i}, c_z], \tilde{\vv\delta}}), ~~~~~~ \text{where}~~~~ c_z = \frac{2z-1}{2n} \tilde{\varepsilon}_i.$
Therefore, optimizing $\vv\varepsilon $ with fixed $\vv\delta = \tilde{\vv\delta}$ can be approximated by 
\begin{align} \label{equ:epsilonoptwide}
\hat{\vv\varepsilon} =\argmin_{ \vv\varepsilon } \Big\{ \sum_{i=1}^{m+m'} \varepsilon_i s_i  ~~~~s.t.~~~ \norm{\vv\varepsilon}_0 \leq \eta_{t},~~~ 
\norm{\vv\varepsilon}_\infty \leq \epsilon%|\varepsilon_i|\leq \epsilon,~~~\forall i \in [m+m']  
\Big\}. 
\end{align}
It is easy to see that finding the optimal solution reduces to selecting the neurons with the largest gradient magnitude $|s_i|$. Precisely, we have $
\hat{\varepsilon}_i = -\epsilon~\ind(|s_i| \geq|s_{(\eta_t)}|)~ \sign(s_i)$, where $|s_{(1)}| \leq |s_{(2)}| \leq \cdots$ is the increasing ordering of $\{|s_i|\}$. 
Finally, we take $f_{t+1} = f_{\hat{\vv\varepsilon},\tilde{\vv\delta}}.$ 

It is possible to further re-optimize $\vv\delta$ with fixed $\vv \varepsilon $ and repeat the alternating optimization iteratively. However, performing the two steps above is computationally efficient and already solves the problem reasonably well as we observe in practice. 

%Note that 
\paragraph{Remark} When we include only neural splitting in $\neib(f_t, \epsilon)$, our method is equivalent to  
splitting steepest descent~\citep{splitting2019}, but with a simpler and more direct gradient-based optimization rather than solving the eigen-problem in~\citet{splitting2019, wang2019energy}. 

\subsection{Growing New Layers}
\label{sec:grow_layers}
We now introduce how to grow new layers under our framework. 
The idea is to include in $\neib(f_t, \epsilon)$ 
deeper networks with extra trainable residual layers 
and to select the layers (and their neurons) that contribute the most to decreasing the loss using the similar two-step method described in Section~\ref{sec:grow-width}.

Assume $f_t$ is a $d$-layer deep neural network of form $f_t = g_d \circ \cdots \circ g_{1}$, where $\circ$ denotes function composition. 
In order to grow new layers, 
we include in $\neib(f_t, \epsilon)$ functions of the form 
\begin{align*} 
f_{\vv\varepsilon, \vv\delta} = g_d \circ (I +  h_{d-1}) \cdots  (I + h_2)\circ  g_2\circ (I+  h_1) \circ g_{1}, &&\text{with}&& h_{\ell}(\cdot)= \sum_{i=1}^{m'} \varepsilon_{\ell i} \sigma(\cdot, \delta_{\ell i}),
\end{align*} 
in which we insert new residual layers of form $I + h_{\ell}$; here $I$ is the identity map,  and $h_{\ell}$ is a layer that can consist of upto $m'$ newly introduced neurons. 
Each neuron in 
$h_\ell$ is associated with a trainable parameter $\delta_{\ell i}$ and multiplied by $\varepsilon_{\ell i} \in [-\epsilon,\epsilon]$. 
As before,
the $(\ell i)$-th neuron is turned off if  $\varepsilon_{\ell i} = 0$,  and 
the whole layer $h_\ell$ is turned off if $\varepsilon_{\ell i} =0$ for all $i\in [1,m']$.  
Therefore, 
the number of new neurons introduced in $f_{\vv\varepsilon, \vv\delta}$ equals $\norm{\vv\varepsilon}_{0} := \sum_{i\ell} \ind(\epsilon_{i\ell}\neq 0)$, and the number of new layers added equals 
$\norm{\vv\varepsilon}_{\infty,0}: =\sum_{\ell} \ind(\max_i |\varepsilon_{\ell i}| \neq 0)$. 
Because adding new neurons and new layers 
have different costs, they can be controlled by two separate budget constraints (denoted by $\eta_{\eta_{t,0}}$ and $\eta_{t,1}$, respectively). 
% the number of new layers introduced. 
%For growing layers, we may want to ensure that the increase of both new layers and new neurons are controlled. %Formally, we can define $C(f) = \max(d)$
Then the optimization of the new network can be framed as 
$$
\min_{\vv\varepsilon, \vv\delta} \Big\{ L(f_{\vv\varepsilon, \vv\delta})  ~~~s.t.~~~ \norm{\vv\varepsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\varepsilon}_{\infty,0} \leq \eta_{t,1},~~~
\norm{\vv\varepsilon}_\infty\leq \epsilon, ~~~
\norm{\vv\delta}_{2,\infty} \leq 1\Big\}, 
$$
where $\norm{\vv\delta}_{2,\infty} = \max_{\ell,i}\norm{\delta_{\ell i}}_2$. 
This optimization can be solved with a similar two-step method to the one for growing width, as described in Section \ref{sec:grow-width}: 
%
we first find the optimal $[\tilde{\vv\epsilon},\tilde{\vv\delta}]$ without the 
complexity constraints (including $\norm{\vv\varepsilon}_{0} \leq \eta_{t,0},$  $\norm{\vv\varepsilon}_{0,\infty} \leq \eta_{t,1}$), and then re-optimize $\vv\varepsilon$ with a Taylor approximation of the objective: 
\begin{align*} 
\min_{\vv\varepsilon} \bigg\{\sum_{\ell i} \epsilon_{\ell i} s_{\ell i}~~~s.t.~~~ \norm{\vv\varepsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\varepsilon}_{\infty,0} \leq \eta_{t,1}\bigg\}, ~
\text{where}~ s_{\ell i} = \frac{1}{\tilde\varepsilon_{\ell  i}}\int_{0}^{\tilde \varepsilon_{\ell i}} \!\!\!\!\!\nabla_{\zeta_{\ell i}} L(f_{[\tilde{\vv\varepsilon}_{\neg \ell i}, \zeta_{\ell i}], \tilde{\vv\delta}}) d \zeta_{\ell i}. 
\end{align*}
%$\epsilon_{ti} = \nabla_{\epsilon_{ti}} L(f(\cdot ~;~\vv\varepsilon, \vv \delta))$. 
The solution can be obtained by sorting $|s_{ti}|$ in descending  order and selecting the top-ranked neurons until the complexity constraint is violated. % or when the gradient becomes positive. \qred{but positive is not a problem; fix}
%In practice, we can conveniently combine the strategies above to simultaneously grow the network wider and deeper. Moreover, the general method can be flexibly extended for specific application use, as will be demonstrated in the following section.

\paragraph{Remark} In practice, we can apply all methods above to simultaneously grow the network wider and deeper. Firefly descent can also be extended to various other growing settings without case-by-case mathematical derivation. Moreover, the space complexity to store all the intermediate variables is $\mathcal{O}(N+m')$, where $N$ is the size of the sub-network we consider expanding and $m'$ is the number of new neuron candidates.\footnote{Because all we need to store is the gradient, which is of the same size as the original parameters.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Growing Networks in Continual Learning} 
\label{sec:cl}
Continual learning (CL) studies the problem of learning a sequence of different tasks (datasets) that arrive in a temporal order,
%
so that whenever the agent is presented with a new task, it no longer has access to the previous tasks.
%
As a result, one major difficulty of CL is to avoid \emph{catastrophic forgetting}, in that learning the new tasks severely interferes with the knowledge learned previously and causes the agent to ``forget'' how to do previous tasks. One branch of approaches in CL consider dynamically growing networks to avoid \emph{catastrophic forgetting}~\citep{rusu2016progressive,li2017learning,yoon2017lifelong,li2019learn,hung2019compacting}. However, most existing growing-based CL methods 
use hand-crafted rules to expand the networks (e.g. uniformly expanding each layer) and do not explicitly seek for the best growing approach under a principled optimization framework.
%
We address this challenge with the Firefly architecture descent framework. 


Let $\D_t$ be the dataset appearing at time $t$ and $f_t$ be the network trained for $\D_t$. 
At each step $t$, we maintain a master network $f_{1:t}$ consisting of the union of all the previous networks $\{f_{s}\}_{s=1}^t$, such that each $f_s$ can be retrieved by applying a proper binary mask. 
%
When a new task $\D_{t+1}$ arrives, 
we construct $f_{t+1}$ by leveraging the existing neurons in $f_{1:t}$ as much as possible, 
while adding a controlled number of new neurons 
to capture the new information in $\D_{t+1}.$


Specifically, we design 
$f_{t+1}$ to include three types of neurons 
(see Figure~\ref{fig:cl_grow}): \textbf{1)} \emph{Old neurons from $f_{1:t}$}, whose parameters are \emph{locked} during the training of $f_{t+1}$ on the new task $\D_{t+1}$. This does not introduce extra memory cost.
%
\textbf{2)} \emph{Old neurons from $f_t$}, whose parameters are \emph{unlocked and updated} during the training of $f_{t+1}$ on $\D_{t+1}$. This introduces new neurons and hence increases the memory size. It is similar to network splitting in Section~\ref{sec:grow-width} in that the new neurons are evolved from an old neuron, but only one copy is generated and the original neuron is not discarded. 
%
\textbf{3)} \emph{New neurons} introduced in the same way as in Section~\ref{sec:grow-width},\footnote{It is also possible to introduce new layers for continual learning, which we leave as an interesting direction for future work.} which also increases the memory cost.
%
Overall, assuming $f_{1:t}(x)=\sum_{i=1}^m \sigma(x; \theta_i)$, possible candidates of $f_{t+1}$ indexed by $\vv\varepsilon,\vv\delta$ are of the form:
$$
f_{\vv\varepsilon, \vv\delta} (x)= 
\sum_{i=1}^m \sigma(x; \theta_i + \varepsilon_i \delta_i) + 
\sum_{i=m+1}^{m+m'} \varepsilon_i \sigma(x; \delta_i), 
%\sigma(x; \theta_i^t + \epsilon \delta) 
$$
where $\varepsilon_i \in [-\epsilon, \epsilon]$ again 
controls if the corresponding neuron is locked or unlocked (for $i\in [m]$), or if the new neuron should be introduced (for $i>m$). The new neurons introduced into the memory are $\norm{\vv\varepsilon}_0 = \sum_{i=1}^{m+m'} \ind(\varepsilon \neq 0)$.
%
The optimization of $f_{t+1}$ can be framed as 
$$
f_{t+1}=\argmin_{\vv\varepsilon, \vv\delta}\Big\{ L(f_{\vv\varepsilon, \vv\delta}; ~ \D_{t+1}) ~~~~s.t.~~~~ \norm{\vv\varepsilon}_0\leq \eta_t, ~~ \norm{\vv\varepsilon}_\infty \leq \epsilon, ~~~ \norm{\vv\delta}_{2,\infty}\leq 1\Big\},
%~~\forall i \in [m+m'] \Big\},
$$
where $L(f; \mathcal D_{t+1})$ denotes the training loss on dataset $\D_{t+1}$. 
The same two-step method  in Section \ref{sec:grow-width} can be applied to solve the optimization. After $f_{t+1}$ is constructed, the new master network $f_{1:t+1}$ is constructed by merging $f_{1:t}$ and $f_{t+1}$ and the binary masks of the previous tasks are updated accordingly. 
See Appendix \ref{app:firefly} for the detailed algorithm.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/continual-learning.pdf}
    \caption{Illustration of how Firefly grows networks in 
     continual learning.}
    \label{fig:cl_grow}
    \vspace{-10pt}
\end{figure}


==> Firefly splitting/content/related.tex <==
\vspace{-15pt}
\section{Related Works}\label{sec:related}
In this section, we briefly review previous works that grow neural networks in a general purpose and then discuss existing works that apply network growing to tackle continual learning.

\paragraph{Growing for general purpose}
Previous works have investigated ways of knowledge transfer by expanding the network architecture. One of the approaches, called Net2Net \citep{wei2016network}, provides growing operations for widening and deepening the network with the same output. So whenever the network is applied to learn a new task, it will be initialized as a functional equivalent but larger network for more learning capacity. Network Morphism \citep{wei2016network} extends the Net2Net to a broader concept, which defines more operations that change a network's architecture but maintains its functional representation. Although the growing methods are similar to ours, in these works, they randomly or adopt simple heuristic to select which neurons to grow and in what direction. As a result, they failed to guarantee that the growing procedure can finally reach a better architecture every time. \citep{elsken2017simple} solve this problem by growing several neighboring networks and choose the best one after some training and evaluation on them. However, this requires comparing multiple candidate networks simultaneously.

On the other hand, recently, \citet{splitting2019} introduces the Splitting Steepest Descent, the first principled approach that determines which neurons to split and to where. By forming the splitting procedure into an optimization problem, the method finds the eigen direction of a local second-order approximation as the optimal splitting direction. However, the method is restricted to only splitting neurons. Generalizing it to special network structure requires case-by-case derivation and it is in general hard to directly apply it on other ways of growing. Moreover, since the method evaluates the second-order information at each splitting step, it is both time and space inefficient.

\citet{hu2019efficient} proposes an efficient path selection method by jointly training all the possible path, select the best subset and add to the network. However, it only discusses the situation in the cell-based network. Our adding strategy treats the general single neuron as the basic unit, thus, firefly can greatly extend the growing scheme into various of scenarios. 

\paragraph{Growing for continual learning} continual learning is a natural downstream application of growing neural networks. ProgressiveNet~\citep{rusu2016progressive} was one of the earliest to expand the neural network for learning new tasks while fixing the weights learned from previous tasks to avoid forgetting. LwF~\citep{li2017learning} divides the network into the shared and the task-specific parts, where the latter keeps branching for new tasks. Dynamic-expansion Net~\citep{yoon2017lifelong} further applies sparse regularization to make each expansion compact. Along this direction, \cite{hung2019increasingly,hung2019compacting} adopt pruning methods to better ensure the compactness of the grown model. All of these works use heuristics to expand the networks. By contrast, {\tt Firefly} is developed as a more principled growing approach. We believe future works can build theoretical analysis on top of the {\tt Firefly} framework.


==> backup/backup.tex <==
% % the general goal of the Firefly Steepest Descent is to find a new $\theta$ within certain neighborhood of $\theta_0$, i.e. $\theta \in N(\theta_0, \epsilon)$, such that the loss decreases the most under a . Here, $\epsilon$ is a parameter that controls the size of $N(\theta_0, \epsilon)$
% % It is a general framework. For any architecture $\theta$, let $N(\theta; \epsilon)$ be a general neighorhood of $\theta$,
% % where $\epsilon$ is parameter that control the size of $N(\theta; \epsilon)$ (e.g., radius), such that when $\epsilon=0$, we have $N(\theta; \epsilon) = \theta$.  

% We consider a general procedure: 
% $$
% \theta_{t+1} \gets 
% \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~
%  \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) \leq \tau_t \right\},
% $$
% where $C(\theta)$ represents a measure of size or computational cost of the network represented by $\theta$. 

% \textcolor{red}{[Explain definition of $N(\theta,\epsilon)$ and $C(\theta)$]} 
% By choosing different $N(\theta)$, we derive a general class of growing mechanisms: 

% 1. Splitting 


% 2. Introducing New Neurons

% 3. Growing layers

% \textcolor{red}{[How to solve optimization?]} 
% A remaining question is how to solve the optimization in each step. The key idea is that when $\epsilon$ is small, the linear objective is closely linear and hence can be solved approximately. 

% Let $\theta = \theta_t \oplus \delta$ (define it in proper way).  What is the value space of $\delta$? 
% Then the optimization reduces to 
% $$
% \delta_{t+1}  
% = \arg\min_{\delta} L(\theta_{t} \oplus \delta) ~~~~s.t.~~~~
% %\delta \in N(0,\epsilon),
% \norm{\delta}_2\leq \epsilon, 
% ~~~~ ||{\delta}||_0 \leq \tau_t. 
% $$

% Our approach: 

% Step 1: Solve $\delta$ without the L0 constraint by running a small number of gradient descent. We this yields that constrainted optimization:
% $$
% \min_{\delta} L(\theta_{t} \oplus \delta) +  \lambda \norm{\delta}_2^2. $$

% Step 2: Select the one with the largest contribution (in terms of gradient norm). This can be motivated by Taylor expansion. We use \emph{integrated gradient}. 

% In practice, we find a small number of $N$ is sufficient (e.g., $N=3$), and outperforms $N=1$. 

% \textcolor{blue}{[Have a nice diagram for our method]}

% \section{Application to Continual Learning} 
% \red{[introduce the set up of continuous learning]}... 


% \section{Related works}
% \textcolor{red}{[Review related works on growing networks]} 

% 1. net morphism/net2net

% 2. growing networks in continous learning. 

% 3. autogrow (growing layers)
 


% \section{FireFly Splitting}
% In this section, we present the Firefly expansion, a first order method to gradually enlarge a network. In particular, Firefly aims to study two questions:
% % FireFly splitting is mainly studying two questions: 
% \begin{enumerate}
%     \item can we split without dealing with the splitting matrix and therefore get rid of the local convergence assumption?
%     \item can we allow not only splitting existing neurons, also allow emerging new neurons?
% \end{enumerate}
% % For 1), we can directly optimize the $\delta$s in the original optimization problem using SGD. So here I replace the 2-norm constraint by an infinite norm constraint to relatively enlarge the feasible sets (compared to 2-norm) and scale the constraints according to the original $\theta$ (we can use $\epsilon$ as well, there is no justification now for scaling):
% To begin with, we formulate the objective of Firefly as the following:
% \begin{flalign*}
% \text{minimize: } &  \mathcal{L}(\delta, w) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(\sum_{i=1}^m w_i \sigma(\theta + \delta_i, x) + \sum_{j=1}^k b_j \sigma(\delta_j, x) \bigg)\bigg]\\
% \text{subject to: }  &\sum_{i=1}^m w_i = 1\\
% &\forall i,\quad ||\delta_i||_2 \leq \epsilon\\
% &\forall j,\quad b_j \leq \epsilon\\
% \end{flalign*}
% % Due to above, we know if two copies of neurons have shared direction of improvement, it can be captured by the gradient anyway. Therefore, I force $\delta_1 = -\delta_2$, so I only need to optimize one of them. The problem then becomes:
% % \begin{flalign*}
% % \text{minimize: }&  \mathcal{L}(\delta) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(\frac{1}{2} ( \sigma(\theta + \delta, x) + \sigma(\theta - \delta, x) \bigg)\bigg]\\
% % &||\delta||_\infty \leq \epsilon ||\theta||_\infty\\
% % \end{flalign*}
% To estimate the loss decrease contribution of each neurons, here we use the line integral method. Assume we consider $n$ neurons, so by above, we will have $\delta = (\delta_1, \dots, \delta_k)$. Note that $\mathcal{L}(0) = \mathcal{L}(\theta)$, we have
% \begin{equation}
%     \mathcal{L}(\delta) - \mathcal{L}(0) = \int_{t=0}^1 \nabla \mathcal{L}(t\delta) \cdot \delta d_t \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta)\bigg) \cdot \delta.
% \end{equation}
% As a result, for each individual neuron that has perturbation $\delta_j$, its contribution to loss decrease can be estimated by:
% \begin{equation}
%     \text{contribution}(j) = \mathcal{L}(\delta_j) - \mathcal{L}(0) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_j)\bigg) \cdot \delta_j.
% \end{equation}


% %We can also define the contribution of each neuron by 
% %$$\text{contribution}(j) = \frac{\mathcal{L}(\delta) - \mathcal{L}(0)}{f_{\theta}(\delta) - f_{\theta}(0)}$$

% %Here $f_{\theta}$ represent the output of the current layer with weight $\theta$, so this contribution constraint the newly added neurons to have a larger loss decrease as well as a minor output change in its layers. 

% Then we can select the top-$m$ of those.
\\\\




% For 2), it is hard to determine the number of neurons to add. Imagine that we are allowed to add infinite number of neurons, then it is essentially possible to fit any function. Therefore, we restrict the number of newly added neurons to be less than a fix number $k$ (so we will have $m$ splitted neurons and fewer than $k$ newly added neurons after a single split operation). The resulting new optimization problem is therefore:

% I do not have much thought on this. The simplest thing to do is to treat all those $\delta_j$, $b_j$ the same as $\delta_i$ and use SGD to train them.
% \paragraph{side note:} some questions:
% \begin{itemize}
%     \item Empirically speaking, the perturbation direction matters less than which neuron to split (if you split certain neuron, you can get stuck). So ideally, we only need $\mathcal{O}(n)$ spaces to store each neurons importance. Since we are doing forward backward during training, can we estimate them on the fly and then split according to the stored info?
%     \item Following above, with firefly, I am thinking maybe it is also possible to train the perturbations on the fly (during training). Say, we add an l1 norm constraint on the perturbation and just let it train. And split according to the norm of the eventual perturbations. The benefit of doing this is that it is not ``local'' anymore, the loss indeed decrease by certain amount after we do this. One may ask then why don't we just double the hidden layer and train the neural network and then prune. I believe it's certainly doable. You start from a small hidden size, then you double the layer width, train, and then prune, and then double again. However, whenever you double the layer, if you nonetheless need to do the net-2-wider-net operation. Otherwise randomly initialized neurons might not do well. In contrast, perturbations are naturally orthogonal to the original parameter and also relies on original parameter. So this method both has a good start point and better descent direction.
% \end{itemize}

% \subsection{Expanding Multiple Layers Simultaneously}
% Assume we are at layer $l$, and have layer below $l-1$ with $n_{l-1}$ neurons and above $l+1$ with $n_{l+1}$ neurons originally. Following the above, if we add $K$ new neurons to each layer and also consider splitting existing $n$ neurons within this layer. Denote $x$ as the original input without expanding the previous layer, and $x'$ the $K$ dimensional new input induced from adding $K$ new neurons to the layer $l-1$. Denote $\Theta \in \mathbb{R}^{n_{l}\times n_{l-1}}$ the original weight matrix at layer $l$. Similarly, the perturbation on $\Theta$ is $\Delta \in \mathbb{R}^{n_{l}\times n_{l-1}}$ and the weights on $l$ layer for the newly added $K$ neurons is $\Delta_{o} \in \mathbb{R}^{K \times n_{l-1}}$. The weight that projects the previous $K$ neurons to the current layer is $\Delta_i \in \mathbb{R}^{(n_l+K) \times K}$. We further split $\Delta_i$ into $\Delta_{i1} \in \mathbb{R}^{n_l \times K}$ and $\Delta_{i2} \in \mathbb{R}^{K \times K}$. The problem can be formulated as:
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{diary/firefly.eps}
%     \caption{Illustration figure of the learnable perturbations.}
%     \label{fig:my_label}
% \end{figure}
% \begin{flalign*}
% \text{minimize: } &  \mathcal{L}(\Delta, \Delta_i, \Delta_o) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(
% \frac{1}{2}\bigg(\sigma((\Theta + \Delta)x + \Delta_{i1}x') + \sigma((\Theta - \Delta)x + \Delta_{i1}x')\bigg) + \epsilon \sigma(\Delta_ox + \Delta_{i2}x') 
% \bigg)\bigg]\\
% \text{subject to: }  & ||\Delta||^2_2 + ||\Delta_i||^2_2 + ||\Delta_o||^2_2 \leq c
% \end{flalign*}

% \begin{equation}
%     \text{contribution}(i_1) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_{i_1})\bigg) \cdot \delta_{i_1}, \quad\text{where $\delta_{i_1}$ is the $i_1$-th row of $\Delta$} 
% \end{equation}

% \begin{equation}
%     \text{contribution}(i_2) \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla \mathcal{L}(\frac{2z-1}{2N}\delta_{i_2})\bigg) \cdot \delta_{i_2}, \quad\text{where $\delta_{i_2}$ is the $i_2$-th row of $\Delta_o$} 
% \end{equation}

% \begin{equation}
%     \text{contribution}(i_1) = \nabla \mathcal{L}(\theta_{i_1} + \delta_{i_1})||_{\delta_{i_1}= 0} \cdot \delta_{i_1}
% \end{equation}
% In fact, during practice, I still find the line integral methods gives better results. This probably because it considers the change beyond the local curvature as well. In practice, $N=3$ seems enough. Also, in the extreme case, the gradient can be taken at any single point along the line the perturbation moves. If we take at the gradient at the very beginning, i.e. $\lim_{t \rightarrow 0}\nabla \mathcal{L}(\theta + t \delta)$, then this should be equivalent as the ``minimum" eigenvector in the exact case. On the other hand, if we take the gradient at $t=1$, then it estimates each neuron's contribution using it's current gradient and how much it deviates from 0. In general, if the local curvature is more convex in the larger space (as if the network has splitted), then the estimation at $t=1$ should be more conservative. Similarly, if the local curvature is more concave, which means the further we move along the perturbation, the loss decreases more on average, then the estimation is more optimistic.
% \section{Firefly (with new neurons) splitting}
% \begin{algorithm*}
%     \caption{Firefly (with new neurons) neural architecture expansion algorithm} \label{alg:main}
%     \begin{algorithmic}
%     \State For each layer, initialize $\Delta \in \mathbb{R}^{n_l \times n_{l-1}}$, $\Delta_o \in \mathbb{R}^{K \times n_{l-1}}$ and $\Delta_i = [\Delta_{i1}; \Delta_{i2}] \in \mathbb{R}^{(n_l+K) \times K}$.
    
%     \While{not converging}\Comment{Optimize the perturbations}
%         \State Calculate $L = \mathcal{L}(\Delta, \Delta_i, \Delta_o) + \lambda(||\epsilon_1 \Delta||^2_F + \epsilon_2 ||\Delta_o||^2_F)$.
%         \State Update $\Delta, \Delta_i, \Delta_o$ according to their gradient of $L$.
%         \State Clip $\Delta_i$ such that $||\Delta_i||_\infty \leq \epsilon_2$
%     \EndWhile
%     \State For each layer, initialize $w = c = \bm{0} \in \mathbb{R}^{n_l\times 1}, w_o = c_o = \bm{0} \in \mathbb{R}^{K\times 1}$.
%     \For{$z = 1 : N$}\Comment{Determine whom to split or expand}
%         \State $t = (2z - 1) / (2N)$
%         \State Let $\tilde{L} = \mathcal{L}((t\Delta + c \odot \Delta), (t\Delta_o + c_o \odot \Delta_o), \Delta_i)$
%         \State $w = w + \pdv{\tilde{L}}{c} / N$
%         \State $w_o = w_o + \pdv{\tilde{L}}{c_o} / N$
%     \EndFor
%     \State Split and expand neurons with the top-$m$ largest weights in $w \oplus w_o$
%     \end{algorithmic}
% \end{algorithm*}
% Recall that
% $$
% \mathcal{L}(\Delta, \Delta_i, \Delta_o) = \mathbb{E}_{x \sim \mathcal{D}}\bigg[\Phi\bigg(
% \frac{1}{2}\bigg(\sigma((\Theta + \epsilon_1 \Delta)x + \Delta_{i1}x') + \sigma((\Theta - \epsilon_1 \Delta)x + \Delta_{i1}x')\bigg) + \epsilon_2 \sigma(\Delta_ox + \Delta_{i2}x') 
% \bigg)\bigg]
% $$
% In practice:
% $$\lambda = 0.01, \quad \epsilon_1 = \sqrt{\epsilon_2},\quad N=3$$

% \section{preliminary results}
% \subsection{Two-Layer RBF Network}
% One of the issues that exact and Rayleigh Quotient methods have is that they are more prone to be stuck at local minimas. This is because either method determines its splitting direction (the eigenvector direction corresponding to the minimum eigenvector) based on the local curvature at the original minimum point. By contrast, Firefly methods, by gradually optimizing the perturbation direction, can see further beyond the original minimum point. We confirm our hypothesis on a simple two-layer radial-basis function neural network, which is of the form:
% \begin{equation}
%     f^*(x) = \sum_{i=1}^{20} w_i^* \sigma((\theta_i^*)^T [x, 1]), \quad \forall \theta_i^*, w_i^* \sim \mathcal{N}(0, \bm{I})
% \end{equation}
% \begin{figure}
% \begin{subfigure}[h]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{diary/rbf_loss.png}
%   \caption{Train Loss v.s. Number of Neurons}
% \end{subfigure}%
% \begin{subfigure}[h]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{diary/13.png}
%     \caption{Example of Exact method Got Stuck}
% \end{subfigure}
% \caption{(a) shows the RBF neural network training loss of different growing methods at different number of neurons, the firefly with new neuron method avoids getting stuck locally by considering growing new neurons as well as splitting. (b) gives an example of how pure splitting methods can get stuck at a local minima.}
% \end{figure}


















%with 
%provides a powerful and  then  estimates each neuron's individual  contribution to the expansion via the integrated gradient method, greedily selects out those neurons that contribute the most and expand from there on. Our method is simple to use and can be flexibly extended to include various growing operations. We derive our method for both growing wider, deeper and continuous learning. 
%
%Since FG only uses gradient estimation, it is much simpler to use and allow us to extend the framework to allow not only splitting existing neurons, but also introducing new neurons or even new layers. 
%

%Empirically, our method demonstrates better performance against existing splitting and growing methods on neural architecture search problems. Empirically, our method is demonstrated to be a useful approach for learning accurate and small neural architectures. \qred{mention some good results here} By combining with DARTS, we achieve xxx and xxx. For continuous learning tasks, we achieve xxx. and significantly outperform existing state-of-the-art approaches. 
%
%To further illustrates the potential of the FG method, we apply it to a continual learning task where it is natural to expand network capacity on the fly. 
%
%As expected, the proposed method is able to keep learning multiple tasks continually with much less parameters but higher accuracy compared to the state-of-the-art.\qred{remove? does not read exciting}To summarize, our key contribution is two-folded: \begin{enumerate}
%    \item Introducing a general and flexible  framework for growing neural network, which allows us to progressively increasingly wider and deeper networks. 
    %; the framework includes locally splitting existing neurons, growing new neurons, and introducing new layers.
 %   \item Applying our method to both neural architecture search and continual learning problems and achieve the state-of-the-art results.
%\end{enumerate}



% \iffalse 
% Learning compact but effective neural architecture is important for real-world applications that suffer from computational constraints, i.e. applications on mobile devices. 
% %
% Network pruning tackles this problem by removing less important parameters from a large pretrained network so that the remaining subnetwork can roughly preserve the original  performance. 
% %
% Unlike pruning, growing methods aim to gradually enlarge the  network's capacity only when necessary and therefore can more flexibly adapt to the task of interest in an online fashion. 
% %
% While simple heuristics like uniformly expanding the width of a feed-forward neural network can work well in certain scenarios, they are still far from being efficient and it is often hard for these methods to outperform pruning methods. 

% %
% Recently, \citet{splitting2019} first frame the network growing problem from a functional steepest descent perspective and present a practical algorithm that greedily determines which neurons are to split and in what direction. 
% %
% By doing so, their method does not require a well pretrained large network, can flexibly adapt its learning capacity, and  demonstrates comparable or improved performance over pruning methods. 
% %
% Despite good performance, the method is limited to only splitting existing neurons and therefore can oftentimes get stuck at local minimums. 
% %
% In addition, the method relies on an  accurate estimation of a local second order splitting matrix, which makes it both hard to implement and computational inefficient.


% To address these issues, we introduce a universal framework of  greedy first-order methods, the Firefly Growing (FG). 
% %
% FG uses a small amount of data to train a local perturbation, i.e. the possible expansions, within the neighborhood  functional space of the given network. 
% %
% It then efficiently estimates each neuron's individual  contribution to the expansion via the integrated gradient method, greedily selects out those neurons that contribute the most and expand from there on. 
% %
% Since FG only uses gradient estimation, it is much simpler to use and allow us to extend the framework to allow not only splitting existing neurons, but also introducing new neurons or even new layers. 
% %
% With such flexibility, FG empirically demonstrates better performance against existing splitting and growing methods on neural architecture search problems. 
% %
% To further illustrates the potential of the FG method, we apply it to a continual learning task where it is natural to expand network capacity on the fly. 
% %
% As expected, the proposed method is able to keep learning multiple tasks continually with much less parameters but higher accuracy compared to the state-of-the-art.

% To summarize, the key contributions of this work are:
% \begin{enumerate}
%     \item Introducing a universal first-order framework, the Firefly Growing, to greedily expand a neural network; the framework includes locally splitting existing neurons, growing new neurons, and introducing new layers.
%     \item Applying the Firefly Growing method to both neural architecture search and continual learning problems and achieve the state-of-the-art results.
% \end{enumerate}

 

% \fi






 %The neighorhood in \eqref{equ:masterupdate} determines the candidate size of network growing and hence places an important role. It need to be designed 
%case by case but some general rules applies. In this section, we mainly consider the general neighborhoods that allows to grow wider.  
 %Note that in this framework, the choice of 
 %Note that 
 %the neighborhood 
  %neighorhood in \eqref{equ:masterupdate} 
%  plays a crucial role of determining 
 % the possible ways in which the network can grow.
% $\neib(f_t, ~\epsilon)$ %, which we discuss in sequel,  plays a critical role. 
 %It should include functions that are $\epsilon$-close to $f_t$ but  
 %with a rich set network structures that makes growing possible (e.g., growing wider or deeper), 
 %, and also need to be constructed to make the optimization in \eqref{equ:masterupdate} (approximately) solvable in practice. 
  %, that are functionally close $f_t$. 
 %may have 
%such that the output does changes smoothly. 
%We can view $\epsilon$ as a step size parameter. 
%where we search the best neural network in a neighborhood $\neib(f_t, ~\epsilon)$ around $f_t$, subject to that its size increases at most by $\eta_t$ over $f_t$.  Here the neighborhood  $\neib(f_t, ~\epsilon)$ is defined such that 
%is no longer than 
%where $\{\eta_{t}\}$ controls the size that we want to increase over $\vv \theta_t$ and $\neib(\vv\theta_t, ~\epsilon)$ is a neighborhood of $\vv \theta_t$ in $\Omega$ with a size parameter $\epsilon$ such that $f_{\vv\theta}(x)= f_{\vv\theta_t}(x) + O(\epsilon)$, such that the output does changes smoothly. We can view $\epsilon$ as a step size parameter. 
%The idea here is similar to typical parametric gradient descent, which can be viewed as taking $\neib(\vv\theta_t, ~\epsilon)$ be the a typical L2 ball in Euclidean space, corresponding to models of the same size. To achieve architecture descent, however, we need to  extend the definition of  $\neib(\vv\theta_t, ~\epsilon)$ to include networks with larger sizes.  And also address how to solve the optimization problem.
%
% In the sequel, we address two important problems: 1) how to define the neighborhood $\neib(\vv\theta_t, ~\epsilon)$ and 2) how to solve the optimization efficiently in practice.  \qred{fix}

%and 2) how to solve the optimization efficiently in practice.  \qred{fix}

%Motivated by \citet{splitting2019},  
%In this work,we approach the problem with a general progressive local descent method, in which we incrementally update the parameter and/or structure of $f$ in $\Omega$ to greedily descent the loss in a way similar to typical gradient descent. 
%growing neural networks in a \emph{local descent} fashion. 
%In progressive growing, See Algorithm XXXX for the general framework.  Starting from a relatively small network, we alternate between typical gradient-based \emph{parametric descent phase}   with fixed model structures, and novel \emph{architecture descent phase}  that grow the network structure to decrease the loss when it is impossible with pure parameter descent, lifting the parameter optimization into a higher dimensional space to escape local optima that can not be escaped in the lower dimensional space (of the smaller models). 



%\paragraph{Definition of $\neib(\vv\theta_t, ~\epsilon)$} 


==> backup/method.tex <==
\section{Firefly Steepest Descent}
In this section, we formalize the Firefly Steepest Descent method by first providing a general framework and then discussing three specific instantiations for different growing strategies.\\\\
%

Let $\Omega$ be the space of all possible models and architectures. 
Consider, for example,  the case of one-layer neural networks, 
we have $f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$, where $\vv \theta = [\theta_i]_{i=1}^n$. Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$. This is an infinite dimensional space. In general, $\Omega$ can be much more complex than this for the case of deep neural networks. 

We consider an abstract algorithm which performs steepest descent on $\Omega$. The idea is to equip each point $\theta$ in $\Omega$ a neighorhood $N(\theta, \epsilon)$, which $\epsilon$ is the size ...


Consider at the growing iteration $t$, the current neural network is parameterized by $\theta_t$ and denote $C(\theta_t)$ as the computational cost of the network, i.e. the total flops. The general objective of the Firefly Steepest Descent is therefore to find a new $\theta$ within a neighborhood of $\theta_t$ which decreases the loss the most under the constraint that $C(\theta)$ remains low. Formally, we consider the following iterative process:
%
\begin{equation}
    \label{eq:6}
    \theta_{t+1} \gets \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~ \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) - C(\theta_t) \leq \tau_t \right\}.
\end{equation}
%
Here $\tau_t$ is a predefined computational budget for the growth and $\epsilon$ is the parameter controlling the size of the neighborhood $N(\theta_t, \epsilon)$, i.e. $\epsilon$ can be the radius of the ball centered at $\theta_t$ in the $L_p$ space \red{this should be a neighorhood in the architecture space, not $L_p$ space}. Note that here we want to abuse the notations and allow $\theta_{t+1}$ to have higher dimension than $\theta_t$. In this case, we treat those dimensions that $\theta_t$ does not have as zeros.\\\\
%
During practice, since the computational cost is mainly associated with the number of channels for each layer, we might just pick $\tau_t$ such that the number of increased channels is limited by some constant $M$. For optimization convenience, we consider a formulation equivalent to Equation \ref{eq:6} by optimizing over the perturbations around $\theta_t$. We also simply pick the $\ell_2$ norm constraint, though extensions to other norms are straightforward. Namely, let $\theta = \theta_t \oplus \delta_t$ (again, the dimensions are matched in the same way as when we compare $\theta_t$ and $\theta_{t+1}$; \red{still $\oplus$ is not defined mathematically}), then above update rule becomes:
%
\begin{equation}
    \label{eq:7}
    \delta_t \gets \arg\min_{||\delta_t||_2 \leq \epsilon} \left \{ L(\theta_t \oplus \delta_t) ~~~~s.t.~~~~ ||\theta_t \oplus \delta_t||_0 - ||\theta_t||_0\leq M \right\} \quad \text{and} \quad \theta_{t+1} &\gets \theta_t \oplus \delta_t ~.    
\end{equation}
To solve the above optimization, we consider the following two-step algorithm:\\\\
\textbf{Step 1}: transform the hard norm constraint into a norm penalty in the objective and solve $\delta_t$ without the $\ell_0$ constraint by running a small number of gradient descent steps:
\begin{equation}
    \hat{\delta}_t = \arg\min_{\delta} L(\theta_t \oplus \delta) + \lambda ||\delta||^2_2
\end{equation}
\textbf{Step 2}: project $\hat{\delta}_t$ back to satisfy the $\ell_0$ constraint, i.e. selecting the top-$M$ neurons that contribute the most to the loss decrease. Formally, let $\delta_t = z \odot \hat{\delta}_t$, where $z\in \{0, 1\}^n$ and $n$ is the dimension of $\hat{\delta}_t$. The objective can be formulated as:
\begin{equation}
    \min_z L(\theta_t \oplus (z \odot \hat{\delta_t})) ~~~~s.t.~~~~ ||z||_0 \leq M
\end{equation}
The possible choices of $z$ explode combinatorially when the dimension of $\hat{\delta}$ is large. Therefore, in practice, we estimate each neuron's contribution with the integrated gradient method. Namely,
\begin{equation}
    \Delta L = L(\theta_t \oplus \hat{\delta_t}) - L(\theta_t) = \int_{\alpha=0}^1 \nabla L(\theta_t \oplus \alpha \hat{\delta}_t) \cdot \hat{\delta_t} ~d\alpha.
\end{equation}
Expanding the gradient for individual parameter $\hat{\delta}_t^{(i)}$, we can formally define the contribution of each neuron and use monte-carlo method to approximate the integral:
\begin{equation}
\text{contribution}(\hat{\delta}_t^{(i)}) = \int_{\alpha=0}^1 \pdv{L(\theta_t \oplus \alpha \hat{\delta}_t)}{\alpha \hat{\delta}_t^{(i)}} \pdv{\alpha \hat{\delta}_t^{(i)}}{\alpha} d\alpha \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\delta}_t^{(i)})\bigg) \cdot \hat{\delta}_t^{(i)}.
\end{equation}
In practice, we find that with as small the $N$ as 3, the sampling can approximate the integral well. After the $\delta_t$ is found, FG simply expands the network according to $\delta_t$ and then resume the learning process. The whole pipeline of FG is summarized in Algorithm \ref{alg:firefly}.\\\\
Next, we will discuss three different network growing strategies: 1) splitting existing neurons, 2) growing new neurons, and 3) introducing extra layers. For each of these strategies, we present their corresponding objective formulation under the above general framework.
\paragraph{Splitting Existing Neurons:}
\paragraph{Growing New Neurons:}
\paragraph{Introducing Extra Layers:}

\begin{algorithm*}[t] % enter the algorithm environment
\caption{Firefly for Progressive Training of Neural Networks} 
\begin{algorithmic} % enter the algorithmic environment
%\begin{emumerate} 
\STATE \textbf{Input} : Search Space $S$. Initial small network $A_0$
\STATE Start from $A_0$.
%with random initialization, set the maximum neuron grow number $m^{*}_{total}$ or energy growth constraint $e^*_{total}$ each iteration and a threshold $|\lambda^*| > 0$ to stop. Repeat the following 4 steps below until the stop criterion is met:
\STATE \textbf{Repeat} Until the stop criterion is met
\STATE At step $t$
\STATE \textbf{1.} Train $A_t$ for several epochs to decrease the loss. 
    \vspace{.3\baselineskip} 
    \STATE \textbf{2.} Expand $A_t$ to a larger neighbor network $A_t'$ by adding a set of neurons $n_t$ in the search space $D$
    \vspace{.3\baselineskip} 
    \STATE \textbf{3.} Train $A_t'$ for several iterations, select the best subset of neurons in $n_t$ using our method. Keep these neurons in the network and drop the rest of the neurons in $n_t$ to get the new network $A_{t+1}$
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}


==> backup/method2.tex <==
\section{Firefly Steepest Descent}
In this section, we first provide a general functional steepest descent perspective for growing neural architectures and briefly review the existing splitting steepest descent as a special case.
%
Then we introduce the more general Firefly Growing framework that uses first-order method to approximate the steepest descent.
%
In addition, we will discuss three particular growing strategies under the general framework.


\section{Main Idea}
To illustrate the idea, 
let us consider a simple one layer neural network: 
$f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$,
where $\vv \theta = [\theta_i]_{i=1}^n$.
Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$.
This is an infinite dimensional space. The problem of learning then reduces to 
\begin{align*} 
\min_{\vv\theta\in\vv \Omega} L(\vv\theta)\overset{def}{=} \E_{x\sim \D}[\Phi(f(x; \vv\theta))] ~~~~s.t.~~~~  C(\theta) \leq \eta, 
\end{align*}
where $C(\theta)$ is some complexity cost such as the size of the network and $\eta$ is a budget constraint, and $\Phi(\cdot)$ denotes the loss function, e.g., $\Phi(f(x)) = (f(x)-f^*(x))^2$ where $f^*$ is the underlying true function. 

%In \citet{splitting2019}, a steepest descent approach is proposed. It alternates between: 

In progressive growing,
we start from a small network and gradually improve its performance by growing in a monotonic fashion. Our procedure alternates between 
parametric descent within a fixed subregion $\Omega_{m}$  and architecture descent across the regions: 

1. \emph{Parametric Descent}  
We perform typical parametric updates with a fixed model structures, 
corresponding to travel inside a subregion $\Omega_{m}.$ 
The parametric descent can continue until no further improvement can be made inside $\Omega_m$, i.e., local optima is reached.  %within the fixed region $\P$
%(corresponding )
%Fixing the structure and optimizing the parameters, this corresponds to optimizing $\vv\theta$ within a fixed subspace $\Omega_{\vv m}.$ 

2. \emph{Architecture Descent} We grow the neural network architecture by jointly updating the parameter and model architecture, 
which corresponds to jumping from one subregion to a higher region with higher complexity. 
%If $\vv\theta$ is not 
%network parameter
%In general, $\Omega$ can be much more complex for deep neural networks.
%Although $\Omega$ is an infinite dimensional space which includes neural networks with varying sizes, it still possible to perform steepest descent in the space of $\vv\Omega$. 


%Starting from an initial network $\vv\theta_0$, at each iteration $t$, we perform a decent on the loss via
Let $\vv \theta_t$ be the neural network at the $t$-th growing phase, we propose to grow the network via the following formulation: 
\begin{align} \label{equ:masterupdate}
\vv \theta_{t+1} = \argmin_{\vv\theta\in \vv \Omega_\infty} L(f(\cdot, \vv\theta)) ~~~~s.t.~~~  \vv\theta \in \neib(\vv\theta_t, ~\epsilon),~~~~~~ 
C(\vv\theta) \leq C(\vv\theta_t)+\eta_{t+1}, 
\end{align}
where $\{\eta_{t}\}$ controls the size that we want to increase over $\vv \theta_t$ and $\neib(\vv\theta_t, ~\epsilon)$ is a neighborhood of $\vv \theta_t$ in $\Omega$ with a size parameter $\epsilon$ such that $f_{\vv\theta}(x)= f_{\vv\theta_t}(x) + O(\epsilon)$, such that the output does changes smoothly. We can view $\epsilon$ as a step size parameter. 

The idea here is similar to typical parametric gradient descent, which can be viewed as taking $\neib(\vv\theta_t, ~\epsilon)$ be the a typical L2 ball in Euclidean space, corresponding to models of the same size. 
To achieve architecture descent, however, we need to  extend the definition of  $\neib(\vv\theta_t, ~\epsilon)$ to include networks with larger sizes.  And also address how to solve the optimization problem.
In the sequel, we address two important problems: 1) how to define the neighorhood $\neib(\vv\theta_t, ~\epsilon)$ and 2) how to solve the optimization efficiently in practice. 

\paragraph{Definition of $\neib(\vv\theta_t, ~\epsilon)$} 
The neighorhood in \eqref{equ:masterupdate} determines 
the candidate size of network growing and hence places an important role. It need to be designed case by case but some general rules applies. In this section, 
we mainly consider the general neighborhoods that allows to grow wider. 

It is useful to illustrate the idea with one-layer networks. 
Consider $f_\theta(x) = \sum_{i=1}^{m} w_i \sigma(x, \theta_i)$. We augmented it by two types of operators: 

\emph{Splitting Neurons (local).} 
We may consider the local updates turns a neuron into multiple similar neurons (intutively viewed as splitting). 
Splitting a neuron $w_i \sigma(x, \theta_i)$ amounts to replace it with a set of neurons $w_{i\ell} \sigma(x, \theta_{i\ell})$, 
where $|\theta_{i\ell} - \theta| \leq \epsilon$ and $\sum_{i\ell} w_{i} =1$. This ensures that the network output after splitting remains similar to the original network when $\epsilon$ is small.
 As argued in \citet{splitting2019}, it is sufficient to consider splitting to two copies $m=2$ and $w_{i1} =w_{i2} = 1/2$ and $\delta_{i1} = -\delta_{i2} = \delta_i$. In this case, it splits into two copies with equal weights, following opposite directions. 

\emph{Growing New Neurons.} 
We introduce a new neuron  $\epsilon w_i' \sigma(\theta', x)$ with a small output weight. that is, we replace $f_\theta$ with $f_\theta(x) + \epsilon w_i'\sigma(\theta_i', x)$ which introduces small change if $\epsilon$ is small. 
Because $\theta'$ can be choosen arbitrarily, this update is non-local and hence may help jump out of local optima. 
%with a small output weight. This amounts to replace $f_\theta$ with $f_\theta(x) + w_i' \sigma$
%Motivated by \citep{splitting2019}, we re
%$$f_{\vv\vartheta'}(x) =\sum_{i=1}^{m'} w_i \sigma(x,\theta'_i).$$Such that for each $j$, we need 

Overall, the augmented neural networks in $\neib(f_t, \epsilon)$
can have a form of 
$$
f(x; ~ \epsilon, \delta) = \sum_{i=1}^m \frac{1}{2}(\sigma(x, \theta_i +\epsilon_i\delta_i)  
+ \sigma(x, \theta_i - \epsilon_i \delta_i)) + \sum_{i=m+1}^{m'} \epsilon_i \sigma(x, \vartheta_i),
$$
where $\epsilon_i$ denotes a step size parameter associated with the $i$-th split or grown neuron and satisfies $\epsilon_i \in [0, \epsilon]$. If $\epsilon_i$ it means the corresponding splitting/growing is turned off,
the $\delta_i$ and $\vartheta_i$ are the splitting direction. 
Therefore, the size of each $f \in \neib(f_t, \epsilon)$  is $C(f ) \leq \norm{\epsilon}_0.$
The weights of the new neurons and satisfies $\norm{\delta_i}_2\leq 1, \norm{\vartheta_i}_2
\leq 1$. 

\paragraph{Optimization}
Now the optimization reduces to 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot; ~\vv\epsilon, \vv\delta)) ~~~s.t.~~~ \norm{\vv \epsilon}_0 \leq \eta_{t+1},~~~\epsilon_i \in [0,\epsilon],~~~
\norm{\delta_i}_2 \leq 1.
$$
This amounts to a joint optimization of the $\delta_i$ vectors, and a combinatorial optimization of which $\epsilon$ should be turned off. 

Although this yields a combinatorial optimization due to the L0 constraint on $\epsilon$, we solve it with two simple steps: 

1) Optimizing $\vv \delta$ with that the sparsity constraint, that is $[\hat{\vv\epsilon}_0, \hat{\vv\delta}]=\argmin_{\vv \epsilon, \vv \delta} L(f(\cdot; ~\vv \epsilon, \vv\delta)) ~~~s.t.~~~ \epsilon_i \in [0,\epsilon],~~~\norm{\delta_i}_2 \leq 1$.

2) Optimizing $\vv \epsilon$. To do so, note that when $\epsilon$ is small, we have by Taylor expansion: 
$$
L_{f_t}(\vv\epsilon, \hat{\vv\delta})  = L_{f_t}(0,0)
+ \sum_{i=1}^{M}\epsilon_i g_i,~~~~~~~ \text{where}~~~ 
g_i = \nabla_{\epsilon_i }L_{f_t}(\hat{\vv\epsilon}_0, \hat{\vv\delta}).
$$
Therefore, we find the optimal $\epsilon $ by 
$$
\min_{ \vv\epsilon } \sum_{i=1}^M \epsilon_i g_i ~~~~s.t.~~~ \norm{\epsilon}_0 \leq \eta_{t},
$$
whose optimal solution amounts to select the neurons with the the most negative $g_i$. Precisely, we have 
%which amounts a solution of 
$$
\hat{\epsilon}_i = \ind(g_i \leq \min(0, g_{(\eta_t)})), 
$$
where $g_{(1)} \leq g_{(2)} \leq \cdots$ is the reordering of $\{g_i\}$ \qred{switch to integral gradient.} 

\paragraph{Growing New Layers}
Our framework is highly flexible, as it just need to define the candidate set of growing operators. 
We introduce how to grow new layers. 

Assume $f$ is a deep neural network of form $f = f_T \circ \cdots \circ f_{1}$. 
We consider 
\begin{align*} 
f' = f_T \circ (I +  h_{T-1}) \cdots  (I + h_2)\circ  f_2\circ (I+  h_1) \circ f_{1}, &&\text{with}&& h_{t}(x)= \sum_{i=1}^{m'} \epsilon_{i\ell} \sigma(x, \delta_{ti}).
\end{align*}
where  we insert new residual layers of form $I+ h_{t}$, 
with $\epsilon_{it} \in [0,\epsilon]$ controlling if the $i$-th neuron is turned on. For growing layers, we may want to ensure that the increase of both new layers and new neurons are controlled. %Formally, we can define $C(f) = \max(d)$
Note that $\norm{\vv\epsilon}_{0} = \sum_{i\ell} \ind(\epsilon_{i\ell}\neq 0)$ denotes the number new neurons introduced and 
$\norm{\vv\epsilon}_{0,\infty}=\sum_{\ell} \ind(\norm{\vv\epsilon_{i}}_{\infty} \neq 0)$ the number of new layers introduced. 
The optimizatoin can be framed into 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot~;~ \vv\epsilon, \vv\delta))  ~~~s.t.~~~ \norm{\vv\epsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\epsilon}_{0,\infty} \leq \eta_{t,1},~~ \norm{\delta_{it}} \leq 1. 
$$
The optimization can be solved similar the case of going wider in Section XXX. 
Similar to that case, we can first solve the optimal $\vv\delta$, and then using Taylor expansion 
the optimal $\vv\epsilon$ can be approximately found by 
$$
\min_{\vv\epsilon} \sum_{ti} \epsilon_{ti} g_{ti}~~~~~s.t.~~~~ \norm{\vv\epsilon}_{0} \leq \eta_{t,0}, ~~  \norm{\vv\epsilon}_{0,\infty} \leq \eta_{t,1},
$$
where $\epsilon_{ti} = \nabla_{\epsilon_{ti}} L(f(\cdot ~;~\vv \epsilon, \vv \delta))$. This solution of this can be obtained by sorting $g_{ti}$ in ascending order and select the neurons until $\norm{\vv\epsilon}_{0} \leq \eta_{t,0}$ or  $\norm{\vv\epsilon}_{0,\infty}$ is satisfied, or when the gradient becomes positive. \qred{but positive is not a problem; fix}

\paragraph{Remark} In practice, we can jointly apply any combinations of the above growing strategies to enlarge the network. As illustrated in the above examples, since Firefly Growing only requires an estimation of the gradient, it can be conveniently apply to different growing scenarios.
%Therefore, the complexity function can be defined as $C(f) - C(f_t) = $
%(x)= \sum_{i=1}^{m'} \sigma(x, \delta_{ti})$. 
%Let f


\subsection{Continual Learning} 
Continual learning (CL) studies the problem of learning a sequence of different tasks (datasets) $\mathcal D_t$ that arrive in a temporal order,
%
so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks $\{\mathcal D_k\}_{k=1}^t$. 
%
The major difficulty of CL is to avoid the \emph{catastrophic forgetting} problem, which means learning the new task will severely interfere with the knowledge learned previously and make the agent ``forget'' about how to do previous tasks.
Network growing provides a natural framework to address this problem because it allows to argument the network while keeping the previous neurons from the previous tasks unchanged. 

Inspired by [XXX], 
our approach is to keep track of a master network $f_{t}$
and a mask $m_s$ for each task $s \leq t$, such that $f_{t}$ applied with mask $m_s$ works for task $s$. 
When a new task $\D_{t+1}$ arrives, 
we grow the network to address the new task. 
The new neural network includes three types of neurons: 

1. The old neurons from the existing network, which does not introduce additional storage. 

2. Neurons inherited from neurons from $f_t$, but adjust copied to fit with the new task. This creates a new neuron and hence increases the storage demand. It is similar to splitting but the original copy is kept (except kept off for the new task).

3. Newly introduced neurons with small output weights. 

%To do so, 
For $f_t(x)=\sum_{i=1}^m \sigma(x; \theta_i^t)$, the growing region is 
$$
f(x; ~ \vv\epsilon, \vv\delta) = 
\sum_{i=1}^m \sigma(x; \theta_i^t + \epsilon_i \delta_i) + 
\sum_{i=m+1}^{m'} \epsilon_i \sigma(x; \delta_i). 
%\sigma(x; \theta_i^t + \epsilon \delta) 
$$
The new neurons introduced is $\norm{\vv\epsilon}_0$, including the relaxed neurons, and the newly introduced neurons. 
Therefore, the optimization reduces to 
$$
\min_{\vv\epsilon, \vv\delta} L(f(\cdot; ~\vv\epsilon, \vv\delta)) ~~~~s.t.~~~~ \norm{\vv\epsilon}_0\leq \eta_t, ~~ \norm{\vv\epsilon}_\infty \leq \epsilon, ~~~ \norm{\vv\delta}\leq 1. 
$$
It can be solved using the same method as before. 
After $f_{t+1}$ is constructed, the masks of the previous tasks are updated accordingly. 
%complexity
%is $C(f(\cdot; ~\vv\epsilon, \vv\delta)) = C(f_t) + $

%the 
%we selectively grow the network to 
%Let $f_t$ be the network for the $t$-th task. 
%
%
%
%
%

%
The performance of CL is evaluated in the end on all the tasks the agent has seen before. So when the $t$-th task arrives, for a parameterized learner, the general objective is to find the parameter $\theta_t$ that minimize the loss over all datasets:
\begin{equation}
    \theta_t = \arg\min_{\theta} \sum_{k=1}^t \mathcal{L}(\theta, \mathcal{D}_k).
\end{equation}
However, since the agent no longer has access to previous datasets, a popular surrogate objective is:
\begin{equation}
    \theta_t = \arg\min_{\theta} \mathcal{L}(\theta, \mathcal{D}_t) + D(\theta_t || \theta_{t-1}),
\end{equation}
where $\theta_t$ denotes the best parameter learned up to task $t-1$ and $D$ is some divergence measuring the similarity between $\theta_t$ and $\theta_{t-1}$. So the ideal $\theta_t$ should minimize the loss on current task while being close to the previous $\theta_{t-1}$ to preserve the performance on old tasks. Consider all $\theta_t \in \Omega$, then a common approach is to fix $\theta_{t-1}$ while growing some new neurons $\theta_{\text{new}}$ so that $\theta_t = \theta_{t-1} \oplus \theta_{\text{new}}$. Meanwhile, we can record a binary mask $m_t$ for task $t-1$ so that $\theta_{t-1} = m_t \odot \theta_t$. Clearly, it follows that $\theta_i = m_{i+1} \odot m_{i+2} \dots \odot m_t \odot \theta_t$, for all $i < t$. As one may have noticed, the key of success for this type of methods is to efficiently grow a small group of new neurons to achieve loss decreases as most as possible, which coincides with what FSD is designed for. Hence, we also consider using FSD as a novel growing method to solve CL.

% One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.

\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}

%%CL is a natural application of the FG method. \qred{write about our own methods first before listing the baselines}%
%To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.%
%We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. 
To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}

%\subsection{}
%$\epsilon_i \in [0, \epsilon]$ and $\norm{\delta}\leq 1 $ and $\vartheta_i\in \RR^d$. 
%$$f_{\vv\vartheta'}(x) =\underbrace{\sum_{i=1}^m \sum_{\ell=1}^k w_{i\ell} \sigma(x, \theta_{i\ell})}_{splitting} + \underbrace{\sum_{j=1}^{m'- k m} w_{j} \sigma(x, \theta_j)}_{growing~~new}$$
%$$\neib(f_{t}; \epsilon) = \{ f \colon ~~ f(x) =\underbrace{\sum_{i=1}^m \sum_{\ell=1}^{k_i} w_{i\ell} \sigma(x, \theta_{i}^t + \epsilon \delta_{i\ell})}_{splitting} +  \underbrace{\epsilon \sum_{j=1}^{k_0} w_{j} \sigma(x, \theta_j)}_{growing~~new} 
%(w_i , \theta_i) \colon ~~ \}$$
%\sum_{i\ell}\ind( \epsilon_i \neq 0) + \sum_j \ind(ep=0).$ 
%$C(f ) = \sum_{i\ell}\ind( w_{i\ell}\norm{\delta_{i\ell}}\neq 0) + \sum_j \ind(w_j=0).$
%k_i + k_0$. 

%It remains to solve the problem. To do so, we first solve $\tilde f_{t+1} = \argmin_{f} L(f)~~s.t.~~ f \in \neib(f_t, \epsilon),$ and then note that we $\epsilon$ is very small, we have $$f(x) = \sum_{i=1}^m \frac{1}{2}(\sigma(x, \theta_i +\epsilon_i\delta_i)  + \sigma(x, \theta_i - \epsilon_i \delta_i)) + \sum_{i=m+1}^{m'} \epsilon_i \sigma(x, \vartheta_i),
%$$where $\epsilon_i \in \{0,\epsilon\}$ and $\norm{\delta}\leq 1 $Minimizing $f$ in $\neib(f_t, \epsilon)$

%is an increasing sequence of  budget constraints \leq \cdots \leq \eta_t \leq \cdots \leq \eta_{\infty}=\eta$ is an increasing sequence ofand 
%$\vv\theta$
%Starting from a network $\vv\theta_t$ with $n$ neurons (which has already reached parametric optimum), our question is how to optimally grow it in an optimal, incremental way. 
%We consider growing wider first. 
%We want to grow the network with continous changes of the neuron. 
%There are two essential ways to grow the network. 
%1. Splitting neurons, in which we replace an existing neural $w_i\sigma(\theta_i, x)$  into $\sum_{k} w_i \sigma(\theta_{i}+\delta_{ik}, x).$2. Growing new neurons, in which we introduce new neurons with $w_{i,new}\sigma(\theta_{i,new}, x)$. 

%This is framed as augmenting the network to 
%$$f(x; \vv \theta, [\delta,\epsilon]) = \sum_{i=1}^m\sum_{i=1}^n w_{ik}\sigma(\theta_i + \delta_{ik}, x)  + \sum_{j=1}^{m'} w_{i}'\sigma(\theta_{i}', x)$$And then we want to optimize it 
%$$\min_{\delta, \epsilon \in N } L(\theta, [\delta], \epsilon).$$The idea is that when $\epsilon$ is sufficiently small, we can approximate it by first growing a lot and then prune?

%$$\min_{\theta'} L(\theta, \theta') s.t.~~~ \norm{\theta}_0\leq \eta, ~~~~ \norm{\theta'} \in N(0).  $$
%We solve this problem bycan approximate it by first growing a lot and then prune?

%$$\tilde \theta'=\argmin_{\theta'} L(\theta, \theta') s.t.~~~ \norm{\theta}_0\leq \eta, ~~~~ \norm{\theta'} \in N(0).  $$
%and then 
%$$\theta' = \arg\min L(\theta, \theta') + \lambda \norm{\theta'}_0\leq \eta. $$

%To formulate the problem of progressively growing a neural network, we can first equip each point $\theta_0 \in \Omega$ with a neighborhood $N(\theta_0, \epsilon)$, where $\epsilon$ describes the size of this neighborhood, and then look within this neighborhood for a new parameter $\theta$ such that the training loss mostly decreases. As a result, this procedure corresponds well to the idea of functional gradient descent. %\bo{I will try to add more to this part, but the transition to next section is still difficult.}


%
\subsection{Growing as Functional Steepest Descent}
Let $\Omega$ be the space of all possible models, i.e. models that have different parameters and architectures.
%
Consider, for example, the case of one-layer neural networks, 
we have $f(x; \vv \theta) = \sum_{i=1}^n \sigma(\theta_i, x)$, where $\vv \theta = [\theta_i]_{i=1}^n$.
%
Then we have $\Omega = \cup_{n=1}^\infty \mathbb R^d$. This is an infinite dimensional space. In general, $\Omega$ can be much more complex for deep neural networks. To formulate the problem of progressively growing a neural network, we can first equip each point $\theta_0 \in \Omega$ with a neighborhood $N(\theta_0, \epsilon)$, where $\epsilon$ describes the size of this neighborhood, and then look within this neighborhood for a new parameter $\theta$ such that the training loss mostly decreases. As a result, this procedure corresponds well to the idea of functional gradient descent. \bo{I will try to add more to this part, but the transition to next section is still difficult.}
%
\subsection{Firefly Growing Framework}
Consider at the growing iteration $t$, the current neural network is parameterized by $\theta_t$ and denote $C(\theta_t)$ as the computational cost of the network, i.e. the total flops. The general objective of the Firefly Steepest Descent is therefore to find a new $\theta$ within a neighborhood of $\theta_t$ which decreases the loss the most under the constraint that $C(\theta)$ remains low. Formally, we consider the following iterative process:
%
\begin{equation}
    \label{eq:6}
    \theta_{t+1} \gets \arg\min_{\theta} \left \{ L(\theta) ~~~~s.t.~~~~ \theta \in N(\theta_t; \epsilon), ~~~ C(\theta) - C(\theta_t) \leq \tau_t \right\}.
\end{equation}
%
Here $\tau_t$ is a predefined computational budget for the growth and $\epsilon$ is the parameter controlling the size of the neighborhood $N(\theta_t, \epsilon)$, i.e. $\epsilon$ can be the radius of the ball centered at $\theta_t$ in $\Omega$. Note that $\theta_{t+1}$ can have higher dimension than $\theta_t$. During practice, since the computational cost is mainly associated with the number of channels for each layer, we might just pick $\tau_t$ such that the number of increased channels is limited by a certain constant $M$. For optimization convenience, we consider a formulation equivalent to Equation \ref{eq:6} by optimizing over the perturbations around $\theta_t$. We also simply pick the $\ell_2$ norm constraint, though extensions to other norms are straightforward. Namely, let $\theta = \theta_t \oplus \delta_t$ (again, the dimensions are matched in the same way as when we compare $\theta_t$ and $\theta_{t+1}$; \red{still $\oplus$ is not defined mathematically}), then above update rule becomes:
%
\begin{equation}
    \label{eq:7}
    \delta_t \gets \arg\min_{||\delta_t||_2 \leq \epsilon} \left \{ L(\theta_t \oplus \delta_t) ~~~~s.t.~~~~ ||\theta_t \oplus \delta_t||_0 - ||\theta_t||_0\leq M \right\} \quad \text{and} \quad \theta_{t+1} &\gets \theta_t \oplus \delta_t ~.    
\end{equation}
To solve the above optimization, we consider the following two-step algorithm:\\\\
\textbf{Step 1}: transform the hard norm constraint into a norm penalty in the objective and solve $\delta_t$ without the $\ell_0$ constraint by running a small number of gradient descent steps:
\begin{equation}
    \hat{\delta}_t = \arg\min_{\delta} L(\theta_t \oplus \delta) + \lambda ||\delta||^2_2
\end{equation}
\textbf{Step 2}: project $\hat{\delta}_t$ back to satisfy the $\ell_0$ constraint, i.e. selecting the top-$M$ neurons that contribute the most to the loss decrease. Formally, let $\delta_t = z \odot \hat{\delta}_t$, where $z\in \{0, 1\}^n$ and $n$ is the dimension of $\hat{\delta}_t$. The objective can be formulated as:
\begin{equation}
    \min_z L(\theta_t \oplus (z \odot \hat{\delta_t})) ~~~~s.t.~~~~ ||z||_0 \leq M
\end{equation}
The possible choices of $z$ explode combinatorially when the dimension of $\hat{\delta}$ is large. Therefore, in practice, we estimate each neuron's contribution with the integrated gradient method. Namely,
\begin{equation}
    \Delta L = L(\theta_t \oplus \hat{\delta_t}) - L(\theta_t) = \int_{\alpha=0}^1 \nabla L(\theta_t \oplus \alpha \hat{\delta}_t) \cdot \hat{\delta_t} ~d\alpha.
\end{equation}
Expanding the gradient for individual parameter $\hat{\delta}_t^{(i)}$, we can formally define the contribution of each neuron and use monte-carlo method to approximate the integral:
\begin{equation}
\ref{eq:score}
\text{contribution}(\hat{\delta}_t^{(i)}) = \int_{\alpha=0}^1 \pdv{L(\theta_t \oplus \alpha \hat{\delta}_t)}{\alpha \hat{\delta}_t^{(i)}} \pdv{\alpha \hat{\delta}_t^{(i)}}{\alpha} d\alpha \approx \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\delta}_t^{(i)})\bigg) \cdot \hat{\delta}_t^{(i)}.
\end{equation}
In practice, we find that with as small the $N$ as 3, the sampling can approximate the integral well. After the $\delta_t$ is found, FG simply expands the network according to $\delta_t$ and then resume the learning process. The whole pipeline of FG is summarized in Algorithm \ref{alg:firefly}.
\subsection{Three Growing Strategies}
\label{sec:str}
Next, we will discuss three different network growing strategies: 1) splitting existing neurons, 2) growing new neurons, and 3) introducing extra layers. For each of these strategies, we present its specific objective function as in step 1 of the FG framework. For illustration purpose, we will consider a neural network like $\Phi(\sigma(\theta, x))$, where $\theta$ is the neuron, $x$ is the input, $\sigma$ is the activation function, and $\Phi$ the mapping that maps the output of the neuron to the final output.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/firefly.pdf}
    \caption{Visual illustration of the three splitting methods. In all cases, FSD first expands the network as illustrated in the visualization and then train the corresponding $\delta$/$\bm{\Delta}$.}
    \label{fig:firefly_method}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Splitting Existing Neurons:} From Theorem 2.3 of \cite{splitting2019}, the optimal solution of greedily splitting existing neurons is to split them into two copies that have the opposite local updates. Formally, if a neuron $\theta$ were to be splitted, the optimal way is to split it into
$\Phi(\frac{1}{2}\sigma(\theta+\delta, x) + \frac{1}{2}\sigma(\theta-\delta, x))$,
where $\delta$ ideally should be along the direction of the mininum eigenvector of the splitting matrix, and the loss decrease are estimated by the corresponding minimum eigenvalue. Instead of solving the eigenvalues/eigenvectors exactly, FG trains the local perturbation $\delta$ with data to approximate the steepest descent direction, and then select the neurons based on the integrated gradient estimation. To summarize, for each neuron $\theta$ in the network, FG creates a corresponding $\delta$ that shares the same size as $\theta$, and then minimize the following:
\begin{equation}
\label{eq:split}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\frac{1}{2}\sigma(\theta+\delta, x) + \frac{1}{2}\sigma(\theta-\delta, x)\bigg) \bigg] + \lambda ||\delta||^2_2.
\end{equation}
After a few gradient steps, FG uses Equation \ref{eq:6} to select the $M$ neurons with the most contribution and only split these neurons according to their learned $\hat{\delta}$.
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/continual-learning.pdf}
    \caption{Illustration of how FSD performs continual learning. When the $t$-th task comes, FSD will iteratively grow the network until it solves the task and then record the corresponding network mask to reproduce the performance on task $t$ in the future.}
    \label{fig:my_label}
\end{figure}
\paragraph{Growing New Neurons:} As we will show in the experiment section, adding new neurons can be essential for FG to escape local minimums compared to pure splitting methods. Since we constrain the computation growth, we limit the algorithm to grow at most $M$ neurons. To make the functional gradient descent update continuous at the current architecture, when introducing these neurons, we initialize them around $0$ and give them a very small weight $\epsilon$. Formally, denote a new neuron as $\theta_{\text{new}} = \bm{0} + \delta$, we consider the following objective:
\begin{equation}
\label{eq:new}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta, x)  + \epsilon \cdot \sigma(\delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.
\end{equation}


\paragraph{Introducing Extra Layers:}
Denote the output of a layer as $\bm{h} = \sigma(\bm{W}\bm{x})$, where $\bm{W}$ is the weight matrix of the layer of interest. To introduce an extra layer, we can insert an identity mapping~\citep{chen2015net2net} layer on top of the current layer, i.e. $\bm{h} = \sigma(\bm{I}\sigma(\bm{W}\bm{x}))$\footnote{Note that this requires $\sigma$ satisfying $\sigma(\bm{I}\sigma(\bm{v})) = \sigma(\bm{v}),\forall \bm{v}$. ReLU is one example of this type of activations.}. Then the objective of finding new layers becomes:
\begin{equation}
    \hat{\bm{\Delta}} = \min_{\bm{\Delta}} \mathbb{E}_{\bm{x} \in \mathcal{D}} \bigg[
        \Phi \bigg(
            \sigma\big((\bm{I} + \bm{\Delta})\sigma(\bm{W}\bm{x})\big)
            \bigg)
    \bigg] + \lambda ||\bm{\Delta}||_F.
\end{equation}
After $\hat{\bm{\Delta}}$ is determined, we can similarly apply Equation~\ref{eq:6} to calculate the contribution of the entire layer by replacing every $\hat{\delta}$ with $\hat{\bm{\Delta}}$. On the other hand, since the contribution of the entire layer is just the sum of the contributions of each neuron, we could alternatively use that summation to approximate the contribution of the layer. Denote the $k$-th row of $\hat{\bm{\Delta}}$ as $\delta_k$ and assume $\hat{\bm{\Delta}}$ has $K$ rows in total ($K$ neurons at this layer), we then have:
\begin{equation}
\label{eq:score}
    \text{contribution}(\hat{\bm{\Delta}}) \approx  \frac{1}{N}\bigg(\sum_{z=1}^N \nabla L(\frac{2z-1}{2N}\hat{\bm{\Delta}}) \bigg) \cdot \hat{\bm{\Delta}} = \frac{1}{N}\bigg(\sum_{z=1}^N \sum_{k=1}^K \nabla L(\frac{2z-1}{2N}\delta_k) \bigg) \cdot \delta_k.
\end{equation}

\paragraph{Remark} In practice, we can jointly apply any combinations of the above growing strategies to enlarge the network. As illustrated in the above examples, since Firefly Growing only requires an estimation of the gradient, it can be conveniently apply to different growing scenarios.

\begin{algorithm*}[t] % enter the algorithm environment
\label{alg:main}
\caption{Firefly for Progressive Training of Neural Networks} 
\begin{algorithmic} % enter the algorithmic environment
%\begin{emumerate} 
\STATE \textbf{Input} : Search Space $S$. Initial small network $A_0$
\STATE Start from $A_0$.
%with random initialization, set the maximum neuron grow number $m^{*}_{total}$ or energy growth constraint $e^*_{total}$ each iteration and a threshold $|\lambda^*| > 0$ to stop. Repeat the following 4 steps below until the stop criterion is met:
\STATE \textbf{Repeat} Until the stop criterion is met
\STATE At step $t$
\STATE \textbf{1.} Train $A_t$ for several epochs to decrease the loss. 
    \vspace{.3\baselineskip} 
    \STATE \textbf{2.} Expand $A_t$ to a larger neighbor network $A_t'$ by adding a set of neurons $n_t$ in the search space $D$
    \vspace{.3\baselineskip} 
    \STATE \textbf{3.} Train $A_t'$ for several iterations, select the best subset of neurons in $n_t$ using our method. Keep these neurons in the network and drop the rest of the neurons in $n_t$ to get the new network $A_{t+1}$
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}

\begin{algorithm*}[t] % enter the algorithm environment
\caption{Firefly Steepest Descent for Continual Learning} 
\begin{algorithmic} % enter the algorithmic environment
    \STATE \textbf{Input} : a stream of datasets $\{\mathcal{D}_1, \mathcal{D}_2, \dots, \mathcal{D}_K\}$, an initial network $A_0$.
    \FOR{task $k=1:K$}
        \STATE Denote $A_k = A_{k-1}$.
        \IF{$k = 1$}
            \STATE Train $A_1$ for several epochs until convergence.
        \ENDIF
        \WHILE{$A_k$ cannot solve task $k$}
            \IF{$k = 1$}
                \STATE Grow $A_k$ with the \textbf{split}-existing-neuron and grow-new-neuron strategies.
            \ELSE
                \STATE Grow $A_k$ with the \textbf{duplicate}-existing-neuron and grow-new-neuron strategies.
            \ENDIF 
            \STATE minimize $L(\mathcal{D}_k, A_k)$ for several epochs until convergence.
        \ENDWHILE
        \STATE Record the network mask $m_k$ for $A_k$.
    \ENDFOR
\end{algorithmic}
\label{alg:firefly}  
\end{algorithm*}

\subsection{Continual Learning} 
Continual learning (CL) studies the problem of learning a sequence of different tasks (datasets) $\mathcal D_t$ that arrive in a temporal order,
%
so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks $\{\mathcal D_k\}_{k=1}^t$. 
%
The major difficulty of CL is to avoid the \emph{catastrophic forgetting} problem, which means learning the new task will severely interfere with the knowledge learned previously and make the agent ``forget'' about how to do previous tasks.
%
The performance of CL is evaluated in the end on all the tasks the agent has seen before. So when the $t$-th task arrives, for a parameterized learner, the general objective is to find the parameter $\theta_t$ that minimize the loss over all datasets:
\begin{equation}
    \theta_t = \arg\min_{\theta} \sum_{k=1}^t \mathcal{L}(\theta, \mathcal{D}_k).
\end{equation}
However, since the agent no longer has access to previous datasets, a popular surrogate objective is:
\begin{equation}
    \theta_t = \arg\min_{\theta} \mathcal{L}(\theta, \mathcal{D}_t) + D(\theta_t || \theta_{t-1}),
\end{equation}
where $\theta_t$ denotes the best parameter learned up to task $t-1$ and $D$ is some divergence measuring the similarity between $\theta_t$ and $\theta_{t-1}$. So the ideal $\theta_t$ should minimize the loss on current task while being close to the previous $\theta_{t-1}$ to preserve the performance on old tasks. Consider all $\theta_t \in \Omega$, then a common approach is to fix $\theta_{t-1}$ while growing some new neurons $\theta_{\text{new}}$ so that $\theta_t = \theta_{t-1} \oplus \theta_{\text{new}}$. Meanwhile, we can record a binary mask $m_t$ for task $t-1$ so that $\theta_{t-1} = m_t \odot \theta_t$. Clearly, it follows that $\theta_i = m_{i+1} \odot m_{i+2} \dots \odot m_t \odot \theta_t$, for all $i < t$. As one may have noticed, the key of success for this type of methods is to efficiently grow a small group of new neurons to achieve loss decreases as most as possible, which coincides with what FSD is designed for. Hence, we also consider using FSD as a novel growing method to solve CL.

% One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.

\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}

%%CL is a natural application of the FG method. \qred{write about our own methods first before listing the baselines}%
%To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.%
%We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. 
To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}


==> content/experiment.tex <==
\section{Experiment}\label{sec:experiments}
In this section, we present three sets of experiments to showcase the power of FG for both neural architecture optimization and continuous learning. 
Across various tasks, we find our method tends to much smaller and computationally efficient architecture with higher performance than existing methods. 
In particular, we find method singificantly outperforms the state-of-the-art m continuous learning methods, including xXX and XXX, all of which also progressively grow neural networks to adapt to new tasks.  

We start with a toy RBF network experiment  in Section XXX 
to demonstrate the advantage of FG over the splitting steepest descent \citep{splitting2019, wu2020signed}, 
%, compared with the second-order splitting method, is less likely to get stuck at local minimums. 
%
and then evaluate our 
FG on neural architecture search (NAS) for 
image classification, in terms of both growing wider and deeper.  
We apply our method to continual learning (CL) 
and compare it against the state-of-the-art method \qred{(name some methods?)} that also continuously grow a network. 

\subsection{Toy RBF Network} \label{sec:toy}
%One problem with the second-order splitting method is that it is more likely to get stuck at local minimums. Because the method considers only the local curvature around the origininal minimum, and more importantly, it can only split existing neurons. To illustrate this problem, 
For the purpose of illustration, 
we start with testing our methods on growing an one-dimensional two-layer radial-basis function (RBF) neural network with one-dimensional inputs, %which is of the form: 
\begin{equation} 
\label{equ:rbf}
f(x) = \sum_{i=1}^{m} w_i \sigma(\theta_{i1} x + \theta_{i2}), \quad \text{where } ~~\sigma(t) = \exp (-\frac{t^2}{2}), ~~~~~x \in \RR, 
\end{equation}
\qred{how do you generate the parameters?}
where $w_i \in \mathbb R$ and $\theta_i = [\theta_{1i},\theta_{2i}]$ are the input and output weights of the $i$-th neuron, respectively. We generate our true function by drawing $m = 15$ neurons with $w_i$ and $\theta_i$ i.i.d. from  $\normal(0,3)$. 
For dataset $\{x^{(\ell)}, y^{(\ell)}\}_{\ell=1}^{1000}$, we generate them
with $x^{(\ell)}$ drawing from $\mathrm{Uniform}([-5,5])$ and let $y^{(\ell)} = f(x^{(\ell)})$.
We apply various growing methods to grow the network from one single neuron all the way up to 12 neurons. 

\emph{Random Splitting} ({\tt Random (Splitting)}): When growing the network, we randomly select one of the existing neurons from the network, split it into two copies, set the output weight to be half value of the original one and give each of them a small random perturbation.

\emph{Random Splitting+New} ({\tt Random (Splitting+New)}): \red{Should not also have as baseline as well?} We introduce 5 newly initialized neurons drawn from $\mathcal{N}(0, 0.1)$ with a small output weights and list them as well as the existing neurons in the network as the candidate set. We randomly choose one neuron from the candidate set, if we choose the newly initialized neuron, we directly add them in the network. And if we select the existing neurons, we split it using the same operation as the {\tt Random Splitting} case.

\emph{Splitting steepest descent} ({\tt Steepest Splitting}):  We following the algorithm of \cite{splitting2019}. We choose one neuron to split and set the perturbation step size $\epsilon = 0.01$.

\emph{Firefly steepest descent} ({\tt Firefly (Splitting only)}): 
\qred{Some key parameters are missing, such as how many neurons we split and add before pruning. We need to do an ablation study on it...} We only apply splitting existing neurons operation described in Section \ref{sec:str} here. After expand the network, we train for 5 iterations and choose the neuron with the highest contribution score defined in \ref{eq:score}. 


\emph{Firefly steepest descent} ({\tt Firefly (Splitting+New)}): 
We apply our algorithm \ref{alg:main}, and deploy 
the splitting and introducing-new-neuron strategies defined in \ref{eq:split} and \ref{eq:new}.   
We add 5 new neurons which are initialized from $\mathcal{N}(0, 0.1)$ and split the existing neurons in the network into two copies. After expanding the network, we will select the neuron with best score after training for 5 iterations.

\emph{Training from scratch} ({\tt Scratch)}): We also train networks of different sizes directly, without progressive growing. 

All the growing methods above add one neuron at each step. We update 10,000 iterations between two consecutive growing. Furthermore, to make sure the results are consistent, we generate one fixed true function, run the experiments 20 times with different generated datasets and report the averaged training loss of the network at each stage of growing in Figure~\ref{fig:toy} \qred{are models randomized everytime as well?}.

Figure \ref{fig:toy}a shows the \red{training loss} as we grow the network size. We can see that 
%w.r.t. the size of the learned network 
{\tt Firefly (Splitting+New)} tends to achieve nearly-zero loss, suggesting that it can efficiently escape local optimum via growing. 
\red{{\tt Random (Splitting+New)}  considers the same space of growing operations, but is clearly less efficient.}
In contrast, methods that only include splitting operators are more likely to get stuck, domenstrating the benefit of adding \red{new random neurons (need fix the name)}. 
%tends to find minimize the training loss 
\red{all splitting methods can get stuck} (never make such absolute claim, and it is your own method.......) at a local minimum and the training loss will no longer decrease from there on. By contrast, FG can more easily escape local minimums and achieve near zero training loss with as few as 6 neurons.



 To study the contribution scores and the integral approximation method described in \ref{eq:score}, we choose one case when the network has $m = 3$ neurons. We expand the network by applying {\tt Firefly (Splitting+New)}, which will split the three existing neurons and introduce 5 new neurons in. After training the expanded network for 5 iterations, we sort the neurons using contribution score, select one of them adding into the network and fintune the network for 10,000 iterations.  Figrue \ref{fig:toy}b shows the relationship between the score rank and the loss after fintuneing when applying different integral steps. We can see from the figure that adding the neuron with a high contribution score will help the network converge better. In addition, more integral steps will lead a better approximation, and as a result, the score rank will 
have a better correlation with the loss after finetune.

%which randomly chooses a neuron to split, and the train from scratch (scratch) method which trains a network of the same size from sctach. For all of the growing methods, we apply them to grow the RBF network from $1$ neuron all the way up to $12$ neurons and draw the corresponding loss curves. 


%In this section, we present three sets of experiments to showcase the strength of FG. Firstly, we adopt a toy RBF network experiment to demonstrate that FG, compared with the second-order splitting method, is less likely to get stuck at local minimums. Then we evaluate FG's performance on Neural Architecture Search (NAS) problems with standard image classification datasets. To further illustrate potential usage of the FG method, we apply it to a continual learning problem and compare it against the state-of-the-art method that also iteratively grow a network. As we will show, FG can learn a much smaller architecture with less computation resource and achieve even higher performance.

%\subsection{Toy RBF Network}
%One problem with the second-order splitting method is that it is more likely to get stuck at local minimums. Because the method considers only the local curvature around the origininal minimum, and more importantly, it can only split existing neurons. To illustrate this problem, we consider growing a two-layer radial-basis function (RBF) neural network with one-dimensional inputs, which is of the form:
%\begin{equation} 
%\label{equ:rbf}
%f(x) = \sum_{i=1}^{m} w_i \sigma(\theta_{i1} x + \theta_{i2}), \quad \text{where } ~~\sigma(t) = \exp (-\frac{t^2}{2}).
%\end{equation}
%Here, $w_i \in \mathbb R$ are the weights of each neuron, and $\theta_{i1}$ and $\theta_{i2}$ are the first layer weights and biases. Specifically, we consider baselines including the steepest descent splitting method (splitting), the random splitting method (random splitting) which randomly chooses a neuron to split, and the train from scratch (scratch) method which trains a network of the same size from sctach. For all of the growing methods, we apply them to grow the RBF network from $1$ neuron all the way up to $12$ neurons and draw the corresponding loss curves. For FG, we apply the splitting and introducing-new-neuron strategies. When introducing new neurons, the neurons are initialized from $\mathcal{N}(0, 0.1)$. At each growing iteration, FG uses one epoch of training to estimate the steepest descent gradient as well as determining which neurons to expand. For all methods, we update 10,000 iterations between two consecutive growing. Furthermore, to make sure the results are consistent, we run the experiments 20 times and report the averaged training loss of the network at each stage of growing in Figure~\ref{fig:toy}.

\begin{figure}[ht!]
    \centering
    \begin{tabular}{cc}
    \raisebox{3.0em}{\rotatebox{90}{{ Loss}}}~\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png} &
    \raisebox{3.0em}{\rotatebox{90}{{ Loss after training}}}~\includegraphics[width=0.45\textwidth]{figures/rbf/score.png}\\
         Number of neurons & Score Rank
         \\
         (a) & (b)\\
    \end{tabular}
    
    \caption{
    \qred{[shorter]}
    \red{TODO: Add random splitting + new baseline here}
    (a) Average loss under 20 runs. 
    (b) The relationship between the contribution score and loss after finetuning when applying different $N$ when $m = 3$.
    }
    \label{fig:toy}
\end{figure}



\subsection{Growing Wider and Deeper Networks}\label{sec:expwider}
We test the effectiveness of our method for growing network width and growing depth, respectively. We use standard image classification tasks on MINST and CIFAR10 as benchmark.  
%of networks for standard image classification tasks. 
\paragraph{Growing width} \qred{result feels not strong with a single figure?}
We compare our method with Splitting Steepest Descent \citep{splitting2019} and Net2Net uniform grow baselines on CIFAR-10 using VGG19 to test FG's performance on widening a deep network. \qred{use bullet like earlier}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{1\baselineskip}
    
    \begin{tabular}{c}
     %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
     \hspace{-1.5em}\raisebox{3.0em}{\rotatebox{90}{{ Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/VGG/percent.pdf}\\
         %Number of neurons & 
         Parameter size ratio
    \end{tabular}
    
    \caption{Widening \qred{wider? more information} VGG19 on CIFAR10 \qred{turn to a wrapfigure}
    }
    \label{fig:cifar}
\end{wrapfigure}

For Net2Net, which uniform grow network by randomly choose the existing neurons to split in each layer. \qred{better to have an independent sentence explain "we compare with Net2Net, which uniform grow network by xx and xx (do they have both splitting and new?) " } Start with a small VGG19 network with a $0.125\times$ multiplier applies on each layer, we grow $30\%$ of the neurons in each layers each time.

For Splitting Steepest Descent and our method, we start with a small VGG19 network with 16 channels in each layer. When applying Splitting Steepest Descent, we follow the setting in \citep{splitting2019} and split $30\%$ neurons in the network each time.

For Firefly steepest descent, we apply splitting and introducting new neurons together. When expanding the network we split all the neurons in the network and additionally add $50$ new neurons in each layer. In the selecting phase, we train the network with new neurons for 1 epoch and select the top $30\%$ of the new neurons based on the contribution score. 

In addition, between two grow steps using the methods above, the network will be finetuned with 160 epochs.

From Figure \ref{fig:cifar}, we can see our Firefly performance outperform the other two growing method and outperform the Full size VGG19's performance using less than 10\% parameters. 


\paragraph{Growing depth} To evaluate FG's performance on deepening a network, we compare against AutoGrow \cite{wen2019autogrow} and Uniform Network Morphsim \citep{wei2016network} that can also introduce new layers. We follow the AutoGrow's experiment setting and choose the same MNIST and CIFAR-10 dataset. For AutoGrow, we build 3 blocks with 1 layer in each block as the initial network. The first layer in each block are set with stride = 2 to decrease the feature map's resolution. For Network Morphsim and FG, we start with a network having one layer with 16 channels in each blocks. Each step, for Network Morphsim, we randomly add one layer in a block.  For AutoGrow, we follow the setting in the paper and grow the layer with pre-defined layer width. And for FG, we pre-define 10 identity layers in each blocks and grow the depths.


\begin{table}[ht!]
\centering
\begin{tabular}{c|c|ccc}

\hline
  \multicolumn{2}{c|}{ }&Structure& Param (M) & Accuracy\\
\hline

\multirow{3}*{MNIST} & AutoGrow & 20-20-20 & 212 & 99.66 \\

& Firefly & 16-15-16 & \textbf{154} &99.66 \\
& Network Morphsim & 23-22-18 & 253 &99.64 \\

\hline
\multirow{2}*{CIFAR10} & AutoGrow & 23-22-22 & 342 & 90.84 \\

& Firefly & - & - &- \\

\hline

\end{tabular}
\caption{Growing Depth }
\end{table}






\subsection{Application on Neural Architecture Search}
\label{sec:expDarts}
We apply our method to improve cell-based Neural Architecture Search (NAS)\citep[e.g.][]{ zoph2018learning, liu2018progressive, real2019regularized}. The idea of cell-based NAS is to learn an optimal neural network module (called cell), from a predefined search space, such that networks constructed from multiple cells can achieve good performance. A cell is a directed graph with $N$ nodes as $N$ latent space. There are several edges between the nodes that can be assigned with the operations in the predefined search space. 



%\qred{improve. need a full course explaination of cell-based. "The idea of cell-based NAS is to learn an optimal neural network module (called cell), from a predefined search space, such that networks constructed from the cell can achieve good performance. The search space of the cells consists of xxxx."}


Following the cell's setting in DARTS \citep{liu2018darts}, we search the structure on the cell with 7 nodes. Our targets is to search the best choice of the operations between each node pairs. We specially modify the operations choice into SepConv$3 \times 3$, SepConv$5 \times 5$, DilConv $3 \times 3$, DilConv $5 \times 5$ and Identity to better formulate our growing strategy. When build up the cell, SepConv$3 \times 3$, SepConv$5 \times 5$, DilConv $3 \times 3$, Dil Conv $5 \times 5$ will be add as operations between each Nodes in the cell and their output result will be sum up as the state of the Node on the output direction.


% \qred{without setting up what we want to do with NAS, i do not know what is going on here.}
% Comparing with other growing method, FG is capable of determining the importance of each layer \qred{(of what?)} globally \qred{what do you mean?}. In addition, FG can more efficiently determine the layer type in each cells by jointly growing all the layer types in the search space and keep only the layer with the most contribution. As a result, FG also achieves very good search efficiency, which is a major bottleneck of contemporary splitting methods. \qred{tell me what you do before saying that FG is good.}

 
To apply our method to cell-based NAS, we first build our search network with 5 stacked cell at the beginning. Among these 5 cells, the second and the fourth one is placed with a special cell called the reduction cell, which contains the operation with stride two to decrease the resolution of the feature map. At beginning, the operations' channels are set to be ${4, 8, 8, 16, 16}$ in each cells. We then progressively train and grow the network. Between every 10 epochs' training on the whole network, we choose one cel and grow all the operations using our Firefly splitting and adding new neurons strategy. Each time when expand the network, we introduce 16 new neurons and split all the existing neurons. In the selection phase, we keep $25\%$ new neurons with the highest contribution score. We totally train the network for 100 epochs with the cell grow order 1-2-3-4-5-1-2-3-4-5 which means each cell will be grow for twice. The overall training setting keep the same as DARTS.

After we finish the search, We select the widest layer as the final search result between each nodes. In addition, if all the layers between two nodes are grow less than $50\%$ comparing with the initial width, we select the identity operation as the search result.


\begin{table}[ht!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c|ccc}
    \hline
        Method & Search Time (GPU Days) & Param (M) & Error  \\
        \hline
        DenseNet-BC \citep{huang2018condensenet} & - & 25.6 & $3.46$
         \\
         \hline
         PNAS \citep{liu2018progressive}& 225 & 3.2 & $3.41$
         \\
         ENAS \citep{pham2018efficient} & 4 & 4.2 & $2.91$
         \\
         Random Search & 4 & 3.2 & $3.29 \pm 0.15$
         \\
      
          DARTS (first order) \citep{liu2018darts} & 1.5 & 3.3 & $3.00 \pm 0.14 $ \\

          DARTS (second order) \citep{liu2018darts}  & 4 & 3.3 & $ 2.76 \pm 0.09$ \\

          Firefly & 1.5 & 3.3 & $ 2.78 \pm 0.05 $  \\
          \hline
    \end{tabular}
    }
    \caption{Performance compared with several NAS baseline}
    \label{tab:nas}
\end{table}

\subsection{Continual Learning}\label{sec:expCL}
%Continual learning (CL) studies the problem of learning a sequence of different tasks in an online fashion so that whenever the agent reaches to a new task, it no longer has any access to the previous tasks. The performance of CL is evaluated in the end on all the tasks the agent has seen before. As a result, the major difficulty of CL is to avoid the catastrophic forgetting problem, which is prominent on rich function approximators like the neural networks. One particular method in CL involves progressively growing a network for new tasks. Importantly, the learning of new tasks can also benefit from the architecture learned from the old tasks since the prediction result comes from the combined architecture learned up to the current task. In short, for task $k$, the network adopts all modules grown up to task $k$ for prediction. While switching to task $k+1$, the network fixes all the parameters learned previously to avoid forgetting.
%\qred{Write about how we apply FG to CL in algorithmic steps. And move it to main text.}
We test our method for continuous learning.  
%CL is a natural application of the FG method.
\qred{write about our own methods first before listing the baselines} 
%
To verify its effectiveness, we choose two state-of-the-art methods that also grow networks for CL, the Compact-Pick-Grow (CPG) \cite{hung2019compacting} and the Learn-to-grow~\cite{li2019learn} methods, as the baseline.
%
We adopt the same training and growing procedure as in CPG and Learn-to-grow when comparing against them. To continually adapt to new tasks while fixing the  old weights, we extend the proposed FG framework to a new operation called \emph{copying existing neurons} \qred{I feel this should goes into the main text }. Essentially, we make copies of existing neurons and apply the grow-new-neuron strategy on those copies (so the main difference is that those new neurons are no longer initialized around zeros). Formally, for a neuron $\theta$ in the network, the objective becomes:
%
\begin{equation}
    \hat{\delta} = \min_\delta \mathbb{E}_{x \in \mathcal{D}} \bigg[ \Phi \bigg(\sigma(\theta_{\text{copy}} + \delta, x) \bigg) \bigg] + \lambda ||\delta||^2_2.\red{what \theta_{copy}+\delta mean mathematically?}
\end{equation}

During implementation, we apply both the copy-exist-neuron and grow-new-neuron strategies to tackle the CL problem. During each growing iteration, we add $15$ new neurons for each layer as candidates for growing. During the selection phase, we select out the top 256 neurons among all the copied neurons and new neurons, for learning the new task. Following the setup in CPG, we finetune 50 epochs for each sub-task.
% Continual learning is another task that perfectly suitable for a growing network. When the new data stream comes, the original network may lack the capacity to remember the new knowledge. Using a large network or separately use several individual model to learn the task may solve the question, however it will be super expensive when we face a large number of tasks situation. So we want to gradually grow the network to meet the growing demand of the network capacity when the new task comes. Moreover, we can better select and use the knowledge from the previous 
% task to support the newly grow network to fit the new task.


% When the training start, the tasks will come one by one as a data stream, the previous task's training data can not be retrieved after it is passed. To prevent the previous task from forgetting when training the new task data, we train the network start from a small network and gradually grow the network while keeping the previous learned neurons' weight fixed. 

% \bo{maybe we can introduce copying as another growing strategy.}
% Specifically saying, suppose we are training the network with task i. When task i is finished and task i + 1 comes, we first use a mask i to fix the weight for task i and prevent it from further update and grow the network using our firefly method. While growing, we keep the original output weight unchanged to prevent the forgetting on the original data. Each time, we add 15 new neurons as well as the splitting neurons copy from the original network at the expansion phase in each layer. Note that to keep the performance of the original network, we set the output weight of the splitting neurons to 1 instead of 0.5. In the selection phase, we train the expanded network for 50 epochs to better fit the new tasks and keep the top 256 neurons as the candidate neurons for the new task.
% After the Firefly operation is done for task i + 1, we together finetune these newly added neurons for task i + 1 with the previous fixed neurons as the parameter for task i + 1. 

Start from a small VGG16 with 32 channels in each layer, we repeat the procedure above and gradually grow our network capacity to adapt the new tasks while keep the old task's performance unchanged. After the training, we can retrieve the task i's model according to the corresponding mask i.

We randomly split CIFAR-100 into 10 and 20 random tasks and compare with some recent baselines including learn-to-grow \citep{li2019learn} and CPG \citep{hung2019compacting} which is the state of the art method on continuous learning tasks. Figure \ref{fig:cl}, Table \ref{tab:cl10} and Tabel \ref{tab:cl20} shows the result.

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|ccc}
    \hline
        Method &  Param (M) & Accuracy  \\
        \hline
          EWC & 6.55  & 74.23
         \\
           HAT & 6.83 & 74.52
         \\
          Learn-to-grow  & 6.86 & 76.21
         \\
          Firefly & 5.63 & \textbf{82.43} \\

          \hline
    \end{tabular}
    \caption{\red{TODO: Add param vs accuracy plot here} 10 random split CIFAR-100}
    \label{tab:cl10}
\end{table}

% \begin{table}[ht!]
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \scalebox{0.8}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%         Method&1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 &  9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 &  19&  20 & avg  \\
%         \hline
%          Individual & 86.8 &	83.2 &	91.6&	93.6 &	89.0&	94.0&	92.4&	79.6&	89.6&	88.6&	94.6&	80.6&	90.6&	88.2&	87.4&	90.8&	88.6&	93.8&	91.6&	82.6&  88.85 \\
%         \hline
%          CPG& 87.0 &	84.0 &	91.4&	95.6 &	91.2&	96.6&	93.0&	80.0&	90.0&	90.8&	95.6&	85.8&	92.4&	89.8&	89.4&	91.8&	89.6&	93.8&	92.8&	83.2&  90.19 \\
%          \hline
%          Firefly & 87.8 & 90.8 & 94.6 & 89.2 & 94.2 & 96.2 & 91.4 & 92.8 & 92.8 & 90.4 & 93.4 & 88.0 & 90.0 & 91.0 & 90.4 & 86.4 & 89.8 & 94.2 & 84.6 & 82.8 &  \textbf{90.53}


\begin{figure}
    \centering
    \begin{tabular}{c}
     %\includegraphics[width=0.4\textwidth]{figures/rbf/rbf_loss.png}&
     \raisebox{3.0em}{\rotatebox{90}{{ Average Accuracy}}}~\includegraphics[width=0.4\textwidth]{figures/cl/cl_20.png}\\
         %Number of neurons & 
         Task ID
    \end{tabular}
    
    \caption{Average accuracy on 20 random split CIFAR-100 dataset over 3 runs. Individual means train each task from scratch using the Full VGG16.
    }
    \label{fig:cl}
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|ccccc}
    \hline
        Method &  Model Size (M) & Avg. Training epochs & Avg. Selecting epochs & Avg. Accuracy  \\
        \hline
          Individual &2565 & 100 & 0& 88.85
         \\
           CPG & 289 & 100 & 420 &90.75
         \\
           CPG w/o FC & 28 & 100 & 420 &90.58
         \\
          Firefly & 26 & 100 & 50 & \textbf{91.03} \\

          \hline
    \end{tabular}
    \caption{Cost of time and space on different method. CPG w/o FC means remove the fully connection layers before the classification layers in CPG to align the model size with Firefly. The average training epoch represents the average epochs taken in fitting the new tasks. The selecting epoch means iteratively pruning and training piggymasks for CPG, means expansion and selection phase for Firefly.   }
    \label{tab:cl20}
\end{table}










==> content/impact.tex <==
\section*{Broader Impact}
This work develops a new framework that can grow neural networks simply and efficiently, which can be generally used in various applications that using neural networks and positively enhance their capacity and performance. In particular, we anticipate it can be applied on devices which have hard memory/computation constraint, i.e. mobile devices or robots. Our work does not have any negative societal impacts.
